Geometric Pricing: How Low Dimensionality Helps in Approximability

Consider the following toy problem. There are $m$ rectangles and $n$ points on the plane. Each rectangle $R$ is a consumer with budget $B_R$, who is interested in purchasing the cheapest item (point) inside R, given that she has enough budget. Our job is to price the items to maximize the revenue. This problem can also be defined on higher dimensions. We call this problem the geometric pricing problem. In this paper, we study a new class of problems arising from a geometric aspect of the pricing problem. It intuitively captures typical real-world assumptions that have been widely studied in marketing research, healthcare economics, etc. It also helps classify other well-known pricing problems, such as the highway pricing problem and the graph vertex pricing problem on planar and bipartite graphs. Moreover, this problem turns out to have close connections to other natural geometric problems such as the geometric versions of the unique coverage and maximum feasible subsystem problems. We show that the low dimensionality arising in this pricing problem does lead to improved approximation ratios, by presenting sublinear-approximation algorithms for two central versions of the problem: unit-demand uniform-budget min-buying and single-minded pricing problems. Our algorithm is obtained by combining algorithmic pricing and geometric techniques. These results suggest that considering geometric aspect might be a promising research direction in obtaining improved approximation algorithms for such pricing problems. To the best of our knowledge, this is one of very few problems in the intersection between geometry and algorithmic pricing areas. Thus its study may lead to new algorithmic techniques that could benefit both areas.

==> arxiv 7.24.2012/abstract_soda13.tex <==

\begin{abstract}
Consider the following toy problem. There are $m$ rectangles and $n$ points on the plane. Each rectangle $R$ is a consumer with budget $B_R$, who is interested in purchasing the cheapest item (point) inside R, given that she has enough budget. Our job is to price the items to maximize the revenue. This problem can also be defined on higher dimensions. We call this problem the {\em geometric pricing} problem.

In high dimensions, the above problem is equivalent to the {\em unlimited-supply profit-maximizing pricing} problem, which has been studied extensively in approximation algorithms and algorithmic game theory communities. Previous studies suggest that the latter problem is too general to obtain a sub-linear approximation ratio (in terms of the number of items) even when the consumers are restricted to have very simple purchase strategies.

In this paper, we study a new class of problems arising from a geometric aspect of the pricing problem. It intuitively captures typical real-world assumptions that have been widely studied in marketing research, healthcare economics, etc. It also helps classify other well-known pricing problems, such as the {\em highway pricing} problem and the {\em graph vertex pricing} problem on planar and bipartite graphs. Moreover, this problem turns out to have close connections to other natural geometric problems such as the geometric versions of the {\em unique coverage} and {\em maximum feasible subsystem} problems.

We show that the low dimensionality arising in this pricing problem does lead to improved approximation ratios, by presenting sublinear-approximation algorithms for two central versions of the problem:  {\em unit-demand uniform-budget min-buying} and {\em single-minded} pricing problems. Our algorithm is obtained by combining algorithmic pricing and geometric techniques. These results suggest that considering geometric aspect might be a promising research direction in obtaining improved approximation algorithms for such pricing problems. To the best of our knowledge, this is one of very few problems in the intersection between geometry and algorithmic pricing areas. Thus its study may lead to new algorithmic techniques that could benefit both areas.
\end{abstract}


==> arxiv 7.24.2012/conclusion_ec.tex <==
\section{Open Problems}\label{sec:conclusion}

%We present a new model for algorithmic pricing problems based on consumers' criteria and items' attributes, and show some evidence that the problem has more desirable approximation factors in many cases, especially when the number of attributes is very low. This model opens up a new direction of tackling the problem and might be extendable to other closely related topics. Our results also reveal a number of low-dimensional geometric structures that can be exploited in designing approximation algorithms.


%We consider the approximation and hardness results for geometric pricing problems. Several interesting problems are open.  

Several interesting problems are open. The most important problem is whether we can obtain better approximation factors for $d$-{\sf UUDP-MIN} and $d$-{\sf SMP}.
%
%For simplicity, let us pay attention to simple purchase strategies such as $d$-{\sf UDP-MIN} and $d$-{\sf SMP}.
%
We tend to believe that there is an $f(d)$-approximation algorithm for $d$-{\sf UUDP-MIN} and $d$-{\sf SMP} where $f(d)$ is a function that depends on $d$ only. However,
it seems to be a very challenging task to obtain approximation ratio like $\log^{O(d)} n$ or $O_d(\log^{1-\epsilon(d)} m)$, for some constant $\epsilon(d)>0$ depending on $d$.

\fullonly{
\begin{openproblem}
\label{conjecture: main one}
For any integer $d >0$, are there $\log^{O(d)} n$-approximation algorithms for $d$-{\sf UUDP-MIN} and $d$-{\sf SMP}?
\end{openproblem}
%
\begin{openproblem}
\label{conjecture: main two}
For any integer $d >0$, are there $O_d(\log^{1-\epsilon_d} m)$-approximation algorithms for $d$-{\sf UUDP-MIN} and $d$-{\sf SMP}?
\end{openproblem}
}



One promising direction in attacking the above problems is to improve Theorem~\ref{thm: dimension reduction for UDP}, e.g., getting $O_d(\rho\cdot\mathrm{polylog}(n))$ for $d$-{\sf UUDP-MIN} using a $\rho$-approximation algorithm of $(d-1)$-{\sf UUDP-MIN} as a blackbox.
\fullonly{
\begin{openproblem}
For any constant $d >0$, given a $\rho$-approximation algorithm for $(d-1)$-{\sf UUDP-MIN} (and $(d-1)$-{\sf SMP}), is it possible to get an $O_d(\rho\cdot\polylog n)$ approximation algorithm for $d$-{\sf UUDP-MIN} (and $d$-{\sf SMP})?
\end{openproblem}
}
%
A positive resolution to this problem would imply $(\log^{O(d)} n)$-approximation algorithm for $d$-{\sf UUDP-MIN}. We believe that, even resolving this problem would require some new insights on geometric and poset structures.

%So we propose the following set of problems (in no particular order) as intermediate steps towards a better understanding of this model.

%In this paper, we show that breaking the barrier of $n$ is possible. A possible next step is to try to get an  $O(\log^{1-\epsilon_d} m)$-approximation for some constant $\epsilon_d >0$ that depends on $d$. For $d=2$, we show that this is possible due to our {\sf QPTAS}.


%A particularly interesting direction to attack this problem is to improve the approximation factor obtained from our dimension reduction theorem; here our reduction transforms an $n^{\rho}$-approximation for $(d-1)$-\pricing to $n^{(3+\rho)/4}$-approximation for $d$-\pricing. Can we do better? For instance, can we turn $\rho$-approximation for $(d-1)$-\pricing to $\rho g(d)$-approximation for $d$-\pricing for some function $g$? One can start by tackling the following weaker statement:



There are two special cases that can be thought of as barriers in dealing with standard versions of {\sf SMP} and {\sf UUDP-MIN}, and we believe that these two special cases serve as good starting points in attacking our problems. The first problem is the geometric version of the Maximum Expanding Subsequence ({\sc Mes}) problem which is the key problem to show the hardness of {\sf UUDP-MIN}~\cite{BriestK11}. The second problem is the Unique Coverage problem \cite{DemaineFHS08} when the sets have constant VC-dimension. Another interesting problem is to obtain {\sf PTAS}s for $2$-{\sf UUDP-MIN} and $2$-{\sf SMP} (e.g., by extending the techniques in \cite{GrandoniR10}). 

\fullonly{

There are two special cases that can be thought of as barriers in dealing with standard versions of {\sf SMP} and {\sf UUDP-MIN}, and we believe that these two special cases serve as good starting points in attacking our problems. First, in order to get an $O_d(\polylog n)$-approximation algorithm for $d$-{\sf UUDP-MIN}, we need to deal with the Maximum Expanding Subsequence ({\sc Mes}) problem which is the key problem to show the hardness of {\sf UUDP-MIN}~\cite{Briest08}.

\fullonly{
\begin{definition}[Maximum Expanding Sub-sequence ({\sc Mes})]
We are given a set of $n$ ground elements $U$ and a set system $S_1,\ldots, S_m$ where $S_i \subseteq U$ for all $i$. We say that $S_{\phi(1)},\dots, S_{\phi(\ell)}$ is {\em expanding sequence} if for all $j$, we have $S_{\phi(j)} \not\subseteq \bigcup_{j' < j} S_{\phi(j')}$. The objective is to find an expanding sequence of maximum length.
\end{definition}

Briest \cite{Briest08} introduces this problem as an intermediate problem to prove hardness of approximation results for {\sf UUDP-MIN} and {\sf SMP}. Roughly speaking, Briest used $n^{\epsilon}$-hardness for this problem to show $n^{\delta}$-hardness of approximating {\sf UUDP-MIN}. His results showed a very strong evidence that {\sc Mes} is very closely related to {\sf UUDP-MIN} and {\sf SMP}. Now we ask the following question.

\begin{openproblem}
Suppose that the underlying set system of {\sc Mes} is defined by our framework in $\R^d$. That is, ground elements are points in $\R^d$, and each set is defined by an unbounded rectangle in $\R^d$. Can we get, says, an $O(\poly \log n)$ approximation algorithm for {\sc Mes}?
\end{openproblem}
}
%
\sodaonly{This motivates us to propose the following open problem, called $d$-{\sc Mes}: Suppose that the underlying set system of {\sc Mes} is defined by our framework in $\R^d$. That is, ground elements are points in $\R^d$, and each set is defined by an unbounded rectangle in $\R^d$. Can we get, says, $O(\poly \log n)$ approximation algorithm for {\sc Mes}?} It can be observed that our algorithm implies an $\tilde O_d(n^{1-\epsilon(d)})$-approximation for $d$-{\sc Mes}. Solving this problem can be considered the first step in getting $\log^{O(d)} n$ approximation.

Getting $O_d(\log^{1-\epsilon(d)} m)$ approximation for $d$-{\sf SMP} also has the following barrier.  Previous results suggest that {\sf SMP} has inherited its intractibility from the problem called {\sf Unique Coverage} \cite{DemaineFHS08}. Roughly speaking, {\sf Unique Coverage} is equivalent to {\sf SMP} in which all consumers have budget one. An $O(\log n)$ approximation is known for this problem \cite{DemaineFHS08}. The question is whether we can improve this ratio in the case of $d$-{\sf SMP}.
\fullonly{
\begin{openproblem}
Is there a sub-logarithmic approximation algorithm for $d$-{\sf SMP} with unit budgets.
\end{openproblem}
}
Solving this problem is a first step in breaking another barrier of $O(\log m)$ for $d$-{\sf SMP}. Moreover, it would give a convincing evidence that our model may not inherit intractibility from {\sf Unique Coverage} problem. In fact, this problem itself can be seen as {\sf Unique Coverage} when the sets have {\em constant VC-dimension} and may be of independent interest.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another interesting direction is to further investigate $2$-{\sf UUDP-MIN} and $2$-{\sf SMP}. We know that {\sf PTAS}s are likely to exist but do not even have an $O(\log n)$-approximation algorithm running in polynomial time. Getting {\sf PTAS} would be very interesting, and we believe that it will require novel ideas and structural properties. Even weaker approximation guarantees, such as $n^{\epsilon}$-approximation in time $n^{O(1/\epsilon)}$, would still be interesting.
%
\fullonly{
\begin{openproblem}
Can we construct $O(\log n)$ approximation algorithms for $2$-{\sf UUDP-MIN} or $2$-{\sf SMP}?
\end{openproblem}
}
}
%
%It is also interesting to extend the technique of the {\sf QPTAS} for $2$-{\sf SMP} to solve more general problems when there are two attributes such as the multidimensional pricing and the case of symmetric valuation and subadditive revenue.\danupon{I added this paragraph. Please check!}

%\begin{enumerate}
%\squishlisttwo
%  \item {\bf Two Attributes:} Can we construct $O(\log n)$ approximation algorithms for $2$-{\sf UDP-MIN} or $2$-{\sf SMP}? Note that we know that {\sf PTAS} is likely to exist but we do not even have an $O(\log n)$-approximation algorithm. Getting {\sf PTAS} would be very interesting and we believe that it will require novel techniques and structural properties. Even weaker approximation guarantees, such as $n^{\epsilon}$-approximation in time $n^{O(1/\epsilon)}$, would still be interesting.

%  \item {\bf Three Attributes:} We have shown that $4$-{\sf UDP-MIN} is {\sf APX}-hard, and $3$-{\sf UDP-MIN} is \NP-hard. Is $3$-{\sf UDP-MIN} {\sf APX}-hard? Or it is possible to get a {\sf QPTAS}. Currently we only have $O(n^{7/8})$-approximation.

%\item {\bf When is $d$-{\sf SMP} {\sf APX}-hard?} We show that $d$-{\sf SMP} is \NP-hard for $d=2$ and {\sf APX}-hard for $d=O(\log n)$. From our {\sf QPTAS}, $2$-{\sf SMP} is not {\sf APX}-hard unless $\NP \subseteq {\sf DTIME}(n^{\poly \log n})$. Nothing is known otherwise.
%\squishendtwo
%\end{enumerate}




%Another very interesting problem is the case where there are some items already priced by other sellers (i.e., Stackelberg problem). This case is still not much explored although it is usually the case in reality.





\iffalse
\squishlist

\item Are there polylogarithmic approximation algorithms for $d$-{\sf UUDP} and $d$-{\sf SMP}, for any constant $d$? We note that, no explicit $O(\log n)$-approximation algorithms are known even for the case of $d=2$, although constant approximation factors are the real hope for a constant $d$ and we know that a {\sf PTAS} is likely to exist for the case of $d=2$.

\item In this paper, a {\sf PTAS} is shown to likely to exist in many cases but it is interesting to have explicit algorithms.\danupon{I'm not sure if we should list this problem.} (A {\sf PTAS} for $2$-{\sf SMP} is especially interesting since it will generalize the recent {\sf PTAS} result for the highway problem.)

\item
Another very interesting problem is the case where there are some items already priced by other sellers (i.e., Stackelberg problem). This case is still not much explored although it is usually the case in reality.



\squishend
\fi


==> arxiv 7.24.2012/hardness.tex <==
\section{Hardness}\label{sec:hardness}

%\sodaonly{We sketch our results here. More details can be found in the full version.}
We provide hardness results in both  scenarios when the number of attributes $d$ is small and when $d$ is large. We sketch our results here. More details can be found in Appendix~\ref{sec:omitted_hardness}.


\paragraph{Few attributes} First we discuss the \NP-hardness of $3$-{\sf UUDP-MIN} and \APX-hardness of $4$-{\sf UUDP-MIN}. These hardness results hold even when the consumer budgets are either 1 or 2. We perform a reduction from Vertex Cover~\cite{DBLP:journals/tcs/GareyJS76,DBLP:conf/ciac/AlimontiK97}, essentially using the same ideas as in~\cite{GuruswamiHKKKM05}, except for the fact that we use Schnyder's result~\cite{Schnyder89,DBLP:conf/soda/Schnyder90} to ``embed'' the instance into posets of low order dimensions.

%These results are proved by a reduction from Vertex Cover~\cite{DBLP:journals/tcs/GareyJS76,DBLP:conf/ciac/AlimontiK97}, which
%uses essentially the same idea as the {\sf APX}-hardness proof of
%{\sf UUDP-MIN}~\cite{GuruswamiHKKKM05}, except for one part in which
%we use Schnyder's result~\cite{Schnyder89,DBLP:conf/soda/Schnyder90} about the {\em order dimensions} of
%planar graphs and cubic graphs.
%We sketch the ideas below and defer the formal proof to \sodaonly{the full version.}\fullonly{Appendix~\ref{sec:omitted_hardness}.}


%states that any planar graph have a adjacency poset of dimension $3$
%and any $4$-colorable graphs (including cubic graphs) have adjacency
%posets of dimension $4$. Moreover, embedding a planar graph to
%Euclidean space can be done in polynomial
%time~\cite{DBLP:conf/soda/Schnyder90}. We now sketch the idea,
%leaving the details in Appendix.


First, let us recall the reduction in \cite{GuruswamiHKKKM05}. We start
from a graph $G=(V,E)$, which is an input instance of Vertex Cover. We create two types of consumers: (i) poor
consumer ${\bf C}_e$ for each edge $e$ with budget $1$ and (ii) rich
consumer ${\bf C}_v$ for each vertex $v$ with budget $2$. The items
are $\iset = \set{{\bf I}_v: v\in V}$. Each poor consumer ${\bf C}_e$ has  a
consideration set containing two items ${\bf I}_u$ and ${\bf I}_v$
where $e=(u,v)$ and each rich consumer ${\bf C}_v$ considers only
one item ${\bf I}_v$. Using the analysis essentially the same as
\cite{GuruswamiHKKKM05}, one can show that the problem is {\sf NP}-hard
if we start from Vertex Cover on planar graphs and {\sf APX}-hard if
we start from Vertex Cover on cubic graphs.
%


Therefore, it only remains to map consumers and items to points in $\reals_{\geq 0}^d$ (where $d=3,4$) such that for each consumer
${\bf C}$, the set of items that pass her criteria (i.e., $\{\Item\in \iset \mid\Item[i]\geq \Consumer[i]~~\mbox{for all $1\leq i\leq d$}\}$) is exactly her consideration set.
The main idea is to first embed the problem into an {\em adjacency poset} of the input graph. Then, we  invoke Schnyder's theorem~\cite{Schnyder89,DBLP:conf/soda/Schnyder90} to again embed this poset into a Euclidean space.

An adjacency poset of a graph can be constructed as follows. First we construct a $2$-layer poset with minimal elements in the first layer and maximal elements in the second layer. For each edge $e \in E$, we have a minimal element in the poset corresponding to $e$ (for convenience, we also denote the poset element by $e$). For each vertex $v \in V$, we have a maximal poset element corresponding to $v$. There is a relation $e\preceq v$ if and only if vertex $v$ is an endpoint of $e$. \fullonly{This is called an {\em adjacency poset} of the graph.}

%Now we define the mapping $\psi$ from consumers and items to poset elements. Mapping $\psi$ maps consumers $\Consumer_e$ and $\Consumer_v$ to the corresponding poset elements $e$ and $v$ respectively. Similarly, mapping $\psi$ maps each item $\Item_v$ to the corresponding poset element $v$.

The last task is to ``embed'' poset elements into points in the Euclidean space in such a way that, for any poset elements $e_1$ and $e_2$, $e_1\preceq e_2$ if and only if $q_{e_1}[i]\geq q_{e_2}[i]$ for all $i$ where $q_{e_1}$ and $q_{e_2}$ are points that $e_1$ and $e_2$ are mapped to, respectively. If we can do this, we would be done, simply by defining the coordinates of each consumer $\Consumer_e$ to be $q_{e}$, and the coordinates of each consumer $\Consumer_v$ to be $q_v$. Similarly, we define the coordinates of each item $\Item_v$ as $q_v$. In order to obtain such an embedding, we use part of Schnyder's theorem~\cite{Schnyder89} which states that any planar graph has an adjacency poset of dimension three, and any $4$-colorable graph (including cubic graphs) has an adjacency poset of dimension four. Moreover, embedding these graphs into Euclidean spaces can be done in polynomial time~\cite{DBLP:conf/soda/Schnyder90}.



%Now we put items and consumers on this poset. We simply put consumers ${\bf C}_e$ and ${\bf C}_v$ on the corresponding poset elements $e$ and $v$, respectively. Similarly we put each item ${\bf I}_v$ on the corresponding poset element $v$. The last task is to map poset elements into points in the Euclidean space in such a way that, for any poset elements $e_1$ and $e_2$, $e_1\preceq e_2$ if and only if $q_{e_1}[i]\geq q_{e_2}[i]$ for all $i$ where $q_{e_1}$ and $q_{e_2}$ are points that $e_1$ and $e_2$ are mapped to, respectively.
%
%Now we think of the poset relation $\preceq$ as the relation ``is dominated by'' between points. Each consumer ${\bf C}_e$ where $e=(u,v)$ considers items ${\bf I}_u$ and ${\bf I}_v$ because $e \preceq u$ and $e \preceq v$; moreover, each consumer ${\bf C}_v$ only considers item ${\bf I}_v$. Therefore, if we can somehow ``embed'' this poset into Euclidean space, preserving the relation $\preceq$, we would be done.
%
%To get this, we use part of Schnyder's theorem~\cite{Schnyder89} which states that any planar graph has an adjacency poset of dimension three, and any $4$-colorable graph (including cubic graphs) has an adjacency poset of dimension four. Moreover, embedding these graphs into Euclidean spaces can be done in polynomial time~\cite{DBLP:conf/soda/Schnyder90}.


Finally we note that $2$-{\sf SMP} is strongly $\NP$-hard and $4$-{\sf SMP} is $\APX$-hard. The proof follows from the fact that these problems generalize Highway pricing and graph vertex pricing on bipartite graphs, respectively, and can be found in \sodaonly{the full version}\fullonly{Appendix~\ref{sec:omitted_hardness}}.\danupon{TO DO: Write the proof for $4$-{\sf SMP}}

%More details can be found in Appendix~\ref{sec:omitted_hardness}.

%
%The latter two results follow simply from the fact that the
%considered problems generalize previous problems. In particular,
%$(k, c)$-$1$-{\sf SMP} generalizes {\sf SMP} with $k$ items and the
%consideration set size is at most $c$. It is shown that this case is
%hard to approximate within a factor of $\Omega(c^\epsilon)$ for some
%$\epsilon>0$, under some complexity assumption~\cite{Briest08,
%BriestThesis}. Additionally, {\sf NC-$2$-SMP} generalizes the
%highway problem, which is recently proved to by strongly {\sf
%NP-hard}~\cite{DBLP:conf/sagt/ElbassioniRRS09}.

\paragraph{Many attributes}
We establish a connection between the {\sf UUDP-MIN} with bounded-size consideration sets and our problem. This connection immediately implies hardness results for $d$-{\sf UUDP-MIN} when $d$ is at least poly-logarithmic in $n$. Our main result in this section is the following:

\begin{theorem}(Informal)
\label{theorem: higher dimension}
Let $A =(\cset, \iset, \{S_\Consumer\}_{ \Consumer \in \cset} )$ be an instance of {\sf UUDP-MIN} where $B=\max_{\Consumer \in \cset} \size{S_\Consumer}$. We can (with high probability of success) create an instance $A'=(\cset', \iset')$ of $d$-{\sf UUDP-MIN}, where $d= O(B^2 \log n)$, that is ``equivalent'' to $A$.
\end{theorem}

In other words, the above theorem shows that any {\sf UUDP-MIN} instance with consideration sets of size bounded by $B$, can be realized by a $d$-{\sf UUDP-MIN} instance for $d= O(B^2 \log n)$.
\sodaonly{
Combining this with the result in \cite{ChalermsookPricing}, we have a hardness of $\Omega(d^{1/4-\epsilon)}$ for any $\epsilon>0$. 
%, assuming the hardness of the balanced bipartite independent set problem in constant degree graphs or refuting random 3{\sf CNF} formulas.
}
\fullonly{
This implies that $d$-{\sf UUDP-MIN} is at least as hard
as the original problem when consideration sets have size at most $B$.
When
$B$ is at least logarithmic in the number of items, our
reduction yields the following corollary, assuming the hardness of the balanced bipartite independent set problem in constant degree graphs or refuting random 3{\sf CNF} formulas \cite{BriestThesis}. \danupon{I shortened the last sentence.}
%assuming some reasonable complexity assumptions (the hardness of the balanced bipartite independent set problem in constant degree graphs or refuting random 3{\sf CNF} formulas) stated formally in \cite{BriestThesis}.\danupon{To do: State the assumption formally in the corollary statement}
%our reduction yields the following result.
\begin{corollary}
There is a constant $\epsilon$ such that for every $d \geq \log^2
n$, it is hard to approximate $d$-{\sf UUDP-MIN} to
within a factor of $d^{\epsilon}$.
\end{corollary}
}

We remark that our reduction here in fact works independently of the decision model, so this result works for {\sf SMP} and {\sf UDP-Util} as well.

%In particular for $B=2$, our result shows that $O(\log n)$-{\sf SMP} is at least as hard as the Graph Vertex pricing problem considered in \cite{BalcanB05}. This implies that $O(\log n)$-{\sf SMP} is \APX-hard.


==> arxiv 7.24.2012/higherdimension.tex <==
\subsection{Hardness Results in Higher Dimensions}\label{sec:higher
dimensions}

In this section, we present the proof of Theorem~\ref{theorem: higher dimension}. Let $A = (\iset, \cset)$ be an instance of {\sf UUDP-MIN} where every consumer ${\bf C}$ has its consideration set $S_\Consumer$ of size at most $B$. Let $\iset = \set{{\bf I}_1,\ldots, {\bf I}_n}$. For each $i \in [d]$, we pick a random permutation $\pi_i: [n] \rightarrow [n]$, so we have $d$ permutations $\pi_1,\ldots, \pi_d$. The function $\phi$ on items $\iset$ can be defined as $\phi({\bf I}_j)[i] = \pi_i(j)$, and we extend the function to the set of consumers as follows: $\phi({\bf C})[i] = \min_{j \in S_C} \pi_i(j)$. Now we have a well-defined function $\phi$.

\begin{lemma}
With probability at least $1- 1/n$, for all consumer ${\bf C} \in \cset$, the consideration set $S'_\Consumer$ defined by $S'_\Consumer = \set{{\bf I}_j: \phi({\bf I}_j) \mbox{ dominates } \phi({\bf C})}$ is exactly $S_\Consumer$.
\end{lemma}
\begin{proof}
Since we define $\phi({\bf C})$ to be the minimum of $\phi({\bf I}_j)$ over all items in $S_\Consumer$, we have $S_\Consumer \sse S'_\Consumer$. Let $k$ be the index of an item that does not belong to $S_\Consumer$. We show the following claim.


\begin{claim}
\label{claim: tiny prob}
The probability that $\phi({\bf I}_k)$ dominates $\phi({\bf C})$ is at most $1/n^{B+2}$.
\end{claim}
\begin{proof}%[Proof of Claim~\ref{claim: tiny prob}]
Fix some $i \in [d]$. The bad event that $\pi_i(k)\geq \min_{j \in
S_C} \pi_i(j)$ happens only if $\pi_i$ does not put $k$ in the last
position among $S_C \cup \set{k}$. This probability is exactly
$(1-1/(B+1))$. Therefore, the bad event happens for all values of
$i$ with probability at most $(1-1/(B+1))^d \leq 1/n^{B+2}$ for $d=
O(B^2 \log n)$.
\end{proof}

This claim immediately implies the lemma: By the union bound, the
probability that $\phi({\bf I}_k)$ dominates $\phi({\bf C})$ is at
most $1/n^{B+1}$. So we have that $\pr{}{S_\Consumer \neq S'_\Consumer} \leq
1/n^{B+2}$. There are at most $n^B$ possible consideration sets of
size at most $B$, so by union bounds, the probability that a bad
event $S_C \neq S'_\Consumer$ happens for some consumer ${\bf C}$ is at most
$1/n$.
%
\end{proof}

\paragraph{$n$ attributes capture general problem} Finally, we end this section with the proof that $n$-{\sf UUDP-MIN} captures the whole generality of {\sf UUDP-MIN}: Consider an instance $(\cset, \iset, \set{S_\Consumer}_{\Consumer\in \cset})$ of {\sf UUDP-MIN}. Denote the set of items by $\iset = \set{\Item_1,\ldots, \Item_n}$. Notice that we can define the coordinates of each consumer by $\Consumer[i] = 0$ if $\Item_i \in  S_\Consumer$, and $\Consumer[i] = 1$ otherwise. We define the coordinates of each item as $\Item_i[i] = 0$ and $\Item_i[j] =1$ for all $j \neq i$. It is easy to check that the consideration sets are preserved by this reduction.




==> arxiv 7.24.2012/intro_soda2013.tex <==
\section{Introduction}

This paper studies a geometric version of two central {\em unlimited-supply pricing} problems. We are given a set $\iset$ of $n$ consumers and a set $\cset$ of $m$ items.
Every item ${\bf I}\in\iset$ is represented by a point ${\bf I} = ({\bf I}[1],\ldots, {\bf I}[d]) \in \R^d_{\geq 0}$, where $\R_{\geq 0}$ denotes the set of non-negative reals and ${\bf I}[j]$ expresses the quality of item ${\bf I}$ in the $j$-th attribute. Every consumer ${\bf C}\in\cset$ is represented by a point ${\bf C}= ({\bf C}[1],\ldots, {\bf C}[d]) \in \R^d_{\geq 0}$, where ${\bf C}[j]$ is the criterion of consumer ${\bf C}\in\mathcal{C}$ in the $j$-th attribute. Each consumer $\Consumer$ is additionally equipped with budget $B_{\Consumer}\in\mathbb{R}_{\geq 0}$ and a consideration set
%
\begin{equation}\label{eq:SC for UDP-MIN}
S_\Consumer=\set{{\bf I}: {\bf I}[j] \geq {\bf C}[j], \mbox{for all } 1\leq j \leq d}.
\end{equation}
\begin{wrapfigure}{r}{0.3\textwidth}
\center
  % Requires \usepackage{graphicx}
  %\includegraphics[width=0.3\linewidth]{problem_visualization.pdf}\\
  \vspace{-.9 cm}
  \includegraphics[width=1.1\linewidth, clip=true, trim= 0.5cm 1cm 1cm 0.8cm]{problem_visualization.pdf}\\
  \caption{Problem visualization}\label{fig:visualization}\vspace{-.3cm}
\end{wrapfigure}
%
In the {\em $d$-dimensional uniform-budget unit-demand min-buying pricing problem} ($d$-{\sf UUDP-MIN}), once we assign prices to items, each consumer ${\bf C}$ will buy the cheapest item ${\bf I}$ in $S_{\Consumer}$ if the price of item  ${\bf I}$ is at most $B_{\Consumer}$. In the {\em $d$-dimensional single-minded pricing problem} ($d$-{\sf SMP}), consumer ${\bf C}$ will buy the {\em all} items in $S_{\Consumer}$ if the total price of those items  is at most $B_{\Consumer}$.
%
The objective is to set the price of items in $\iset$ in order to maximize the revenue. That is, we want to find $p: \iset\rightarrow \reals_{\geq 0}$ that maximizes $\sum_{{\bf C}\in \cset, \min_{\Item\in S_\Consumer} p(\Item)\leq B_\Consumer} \min_{\Item\in S_\Consumer} p(\Item)$ in the case of $d$-{\sf UUDP-MIN} and $\sum_{{\bf C}\in \cset, \sum_{\Item\in S_\Consumer} p(\Item)\leq B_\Consumer} \sum_{\Item\in S_\Consumer} p(\Item)$ in the case of $d$-{\sf SMP}.
%
Fig.~\ref{fig:visualization} illustrates the problem: Each item corresponds to a point in the plane. The consideration set of each consumer $\Consumer$ is represented by an (unbounded) axis-parallel rectangle with point ${\bf C}$ as a lower-left corner.

% and interested in buying items inside its interior.

%Each consumer $\Consumer$ is an (unbounded) axis-parallel rectangle with point ${\bf C}$ as a lower-left corner and interested in buying items inside its interior.



The above problems when $d$ is unbounded (called {\sf UUDP-MIN} and {\sf SMP}) have been widely studied recently
(e.g.,
\cite{Rusmevichientong03,GuruswamiHKKKM05,RusmevichientongRG06,BriestK11,ChalermsookPricing,AggarwalFMZ04,BalcanB07})
%
and are known to be $O(\log m)$-approximable~\cite{AggarwalFMZ04}; so we have a reasonable approximation guarantee when there are not many consumers.
However, in many cases, one would expect the number of consumers to be much larger than the number of items~$n$. In this case, we are still stuck at the trivial $O(n)$ approximation ratio, and there are evidences that suggest that getting a sub-linear approximation ratios might be impossible: Unless $\NP \subseteq \DTIME(n^{\poly  \log n})$, these problem are hard to approximate within a $2^{\log^{1-\epsilon} n}$ for any constant $\epsilon>0$~\cite{ChalermsookPricing}. Moreover, assuming a stronger (but still plausible) assumption, these problems are hard to approximate to within a factor of $n^{\epsilon}$ for some $\epsilon >0$ \cite{BriestK11}.


%This calls for more insights from real-world scenarios to help overcome this barrier. Two previous research directions along this line are to exploit either input distributions or special structures. This paper focuses on making a step further in the second direction. In this direction, we have seen some progress in recent years (e.g., when there is a {\em price-ladder constraint}~\cite{Rusmevichientong03,AggarwalFMZ04,RusmevichientongRG06,RusmevichientongRG06-2,BriestK07}, consideration sets are small~\cite{BalcanB07,BriestK07} or consideration sets correspond to paths on graphs~\cite{BalcanB07,ElbassioniSZ07,GrandoniR10,ElbassioniRRS09,DBLP:conf/icalp/GamzuS10}). However,  the previously studied structures are very specific to special scenarios, and thus it has been a challenging task to find simplified problem structures that capture various real-world settings while allowing us to break the previous barrier.

Motivated by various types of assumptions, the pricing problems with special structures have been studied (e.g., when there is a {\em price-ladder constraint}~\cite{Rusmevichientong03,AggarwalFMZ04,RusmevichientongRG06,RusmevichientongRG06-2,BriestK11}, consideration sets are small~\cite{BalcanB07,BriestK11} or consideration sets correspond to paths on graphs~\cite{BalcanB07,ElbassioniSZ07,GrandoniR10,ElbassioniRRS09,DBLP:conf/icalp/GamzuS10}). In these cases, better approximation ratios are usually possible.

In this paper we consider the geometric structure of pricing problems arising naturally from real-world scenarios, which turns out to be quite general. Our motivation is two-fold: We hope that the geometric structures will lead to better approximation algorithms, and we found these problems interesting on their own as they have connections to other pricing and geometric problems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is the longer version of the intro. - Danupon
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%This calls for more insights from real-world scenarios to help getting through this barrier. Previous research along this line can be categorized into the following two types, depending on simplification assumptions made. This paper makes a step forward in the second direction.

%The first direction is when we assume that consumer valuations are drawn from some known distributions. Previous research in this direction shows that if we assume that each consumer's valuations on different items are drawn independently, then approximation algorithms with better factors exist in some cases~\cite{CaiD11,ChawlaHK07,ChawlaHMS10}. Thus, this is one promising direction although it is still open how to deal with this problem when there are correlations.\danupon{Removed: However, if this is not the case then the problem could be equally hard~\cite{BriestThesis,Briest08}.}


%The second direction, which complements the first approach when input distribution cannot be assumed, is to exploit more problem structures. For instance, one might consider the case where the size of each consideration set is bounded above by some number $k$ (e.g., \cite{BalcanB07,BriestK07}) or assume that considerations sets are {\em paths} in a graph (e.g., \cite{BalcanB07,ElbassioniSZ07,GrandoniR10,DBLP:conf/sagt/ElbassioniRRS09,DBLP:conf/icalp/GamzuS10}).
%
%However, the previously studied structures are very specific to some special scenarios, and thus it has been a challenging task to find simplified problem structures that capture various real-world settings. \danupon{Let's explain more detail in related work section instead.}

%%%%However, these ways of classifying the problem clearly have limitations. The first type of classification cannot deal with consumers who, say, would be willing to buy any car as long as it is cheap enough (i.e., the size of the consideration set is as  large as $n$). The second way clearly cannot deal with problems that do not possess graph structures, e.g., the case of cars. This motivates us to search for a new way to classify the problem, while the problem remains tractable.

%\subsection{Our Approach \& Results}

%To break through the approximation barrier of the {\sf UUDP-MIN} problem and at the same time capture a broad class of real-world settings, we propose a natural structure based on the following simple observation on the consumers' behavior.

Our problems are motivated by the following simple observation on the consumers' behavior.
%
Consider a setting where we sell cars. If a consumer has car $A$ with horse power $130$HP in her consideration set, she would not mind buying car $B$ with horse power $150$HP. Maybe she does not want $B$ because it is less energy-efficient or has lower reputation. But, if we list {\em all} attributes of the cars that people care about and it happens that $B$ is not worse than $A$ in all other aspects, then $B$ should also be in the list.

%\paragraph{Our approach: attribute-based consideration sets.} In this paper we propose a natural structure that captures a broad class of real-world scenarios. This approach is based on the following simple observation on  the consumers' behavior.  Consider a setting where we sell cars. If a consumer has Honda Civic with horse power $130$HP in her consideration set, she would not mind buying Ford Fusion with horse power $150$HP. Maybe she does not want Ford Fusion because it is less energy-efficient or has lower reputation. But, if we list {\em all} attributes of the cars that people will look at and it happens that Ford Fusion is not worse than Honda Civic in all other aspects, then Ford Fusion should also be in the list.

In particular, instead of looking at a full generality where each consumer $\Consumer$ considers any set of items $S_\Consumer$, it is reasonable to assume that each consumer has some criterion in mind for each attribute of the cars, and her consideration set consists of any car that passes all her criteria, i.e.  consumers judge items according to their attributes.
This natural assumption  has been a model of study in other fields such as marketing research, healthcare economics and urban planning. It is referred to as the {\em attribute-based screening process}. In particular, using criteria to define consideration sets as in Eq.~\eqref{eq:SC for UDP-MIN} is called {\em conjunctive screening rule}. Besides being natural, this assumption has been supported by a number of studies where it is concluded that consumers typically use a conjunctive screening rule in obtaining their consideration sets (see further detail in Section~\ref{sec:relatedwork}).

It is also interesting that $d$-{\sf SMP} captures many previously studied problems as special cases. For example, $2$-{\sf SMP} generalizes the highway pricing problem~\cite{GuruswamiHKKKM05,BalcanB07,ElbassioniSZ07,GrandoniR10} and thus our algorithmic results on $2$-{\sf SMP} can immediately be applied to this problem. Moreover, $3$-{\sf SMP} generalizes the upward case of the tollbooth pricing problem \cite{ElbassioniRRS09,KortsarzRR11} as well as the graph vertex pricing problem on planar graphs \cite{BalcanB07,ChalermsookKLN11}. $4$-{\sf SMP} generalizes the unlimited-supply version of the {\em exhibition} problem \cite{ChristodoulouEF10}, the graph vertex pricing problem on bipartite graphs \cite{BalcanB07,KhandekarKMS09}, and the ``rectangle version'' of the {\em unique coverage problem} ({\sc UC}) \cite{DemaineFHS08}, which are the geometric variants of {\sc UC} studied recently in~\cite{ErlebachL08,ItoNOOUUU12}.


%Another problem that specializes {\sf SMP} is the {\em unique coverage problem} \cite{DemaineFHS08}. Geometric versions of this problem have received attention recently~\cite{ErlebachL08,ItoNOOUUU12}, including the ``rectangle version'' which is a special case of $4$-{\sf SMP}.

%Until very recently, unique coverage problem serves as the main ``source of hardness'' for {\sf SMP}, since it is a special case of {\sf SMP} and the only hardness proof of {\sf SMP} was through unique coverage. Geometric versions of unique coverage have received attention recently~\cite{ErlebachL08,ItoNOOUUU12}. Our $4$-{\sf SMP} problem can be thought of as a generalized variant of geometric unique coverage where sets are rectangles.


Moreover, {\sf SMP} is a special case of the {\em maximum feasible subsystem with 0/1 coefficients} problem ({\sc Mrfs}) \cite{ElbassioniRRS09}. Elbassioni et~al. \cite{ElbassioniRRS09} showed that a very special geometric version of {\sc Mrfs} (the ``interval version'') admits much better approximation ratios than the general one. A geometric {\sc Mrfs} can be seen as a special case of ``$2$-{\sc Mrfs}'' in our terminologies, and it is thus interesting whether ``$d$-{\sc Mrfs}'' is easier than general {\sc Mrfs} for other values of $d$. Our geometric {\sf SMP} is a special case of $d$-{\sc Mrfs}. Thus, solving $d$-{\sf SMP} serves as the first step towards solving  $d$-{\sc Mrfs}.



%
%TO BE FINISHED
%Moreover, $d$-{\sf SMP} is also closely related to the maximum feasible subsystem with 0/1 coefficients ({\sc Mrfs}), studied in, e.g.,\cite{XXX}. Elbassioni et~al~\cite{ElbassioniRRS09} shows that the general case of {\sc Mrfs} is $m^{1/3-\epsilon}$ hard to approximate (even in a bi-criteria setting), and this was recently improved by Chalermsook~et~al~\cite{XXX} to $m^{1-\epsilon}$. Interestingly, as shown in~\cite{ElbassioniRRS09}, {\sc Mrfs} generalizes {\sf SMP}. Besides the general {\sc Mrfs}, Elbassioni et~al also discussed a ``geometric variant'' of the problem where constraints are defined by intervals and variables correspond to points on the line, and they showed that improvements are possible in this geometric setting, e.g. one can even gets a {\sf QPTAS} in a bi-criteria setting.
%TO BE FINISHED


%Besides, a number of studies have concluded that consumers typically use a conjunctive screening rule in obtaining a consideration set.

\subsection{Our Results and Techniques}

We show that geometric structures lead to breaking the linear-approximation barrier: While the pricing problems are likely to be hard to approximate within a factor of $n^{1-\epsilon}$ in the general cases, we obtain an $o(n)$-approximation algorithms in the geometric setting, as follows.

\begin{theorem}\label{thm:intro thm udp smp}
For any $d>0$, there is an $\tilde O_d\left(n^{1-\epsilon(d)}\right)$-approximation algorithm for $d$-{\sf UUDP-MIN} and $d$-{\sf SMP} where function $\epsilon(d): = \frac{1}{4^{d-1}}$ and $\tilde O_d$ treats $d$ as a constant and hides a $\mathrm{polylog}(n)$ factor.
\end{theorem}
%
%

The essential idea behind our algorithm is to partition the problem instance into sub-instances without decreasing the optimal revenue (we call this {\em consideration-preserving decomposition}). This is done by using Dilworth's Theorem (partitioning items into chains and anti-chains) and epsilon-nets to find subsets of items satisfying certain structural properties. Subsequently, we show that the dimensions of these sub-instances can be reduced through the notion of {\em consideration-preserving embedding}. In the end of our algorithm, we are left with a sub-linear number of sub-instances, each of which can be solved almost optimally in polynomial time. Returning the best solution among the solutions of these sub-instances guarantees a sub-linear approximation ratio.

The spirit of our technique is in some sense in a similar flavor to Chan's algorithm \cite{Chan12} which computes a {\em conflict-free} coloring of $d$-dimensional points (w.r.t. rectangle ranges) using $O(n^{1-0.632/(2^{d-3}-0.368)})$ colors. In particular, in the 2-dimensional cases of both our geometric pricing and Chan's conflict-free coloring problems, the upper bounds of $O(\sqrt{n})$ can be obtained by a simple application of Dilworth's theorem (Ajwani et al. \cite{AjwaniEGR12} obtained a better bound in this case for the latter problem). However, the techniques of the two results are different in higher dimensions.

\paragraph{QPTASs} We also obtain {\sf QPTAS}s for $2$-{\sf UUDP-MIN} and $2$-{\sf SMP}. We present this in Appendix~\ref{sec: qptas 2 udp} and \ref{sec:2-SMP}. These results, together with a widely-believed assumption that the existence of a {\sf QPTAS} for any problem implies that {\sf PTAS} exists for the same problem (e.g., \cite{BansalCES06,ElbassioniSZ07}), imply that the value of $\epsilon(d)$ in Theorem~\ref{thm:intro thm udp smp} could be improved slightly to $1/4^{d-2}$.
%
As a by-product of these results, we show a {\sf QPTAS} for $2$-{\sf SMP} which subsumes the previous {\sf QPTAS} for highway pricing \cite{ElbassioniSZ07}.

\begin{comment}

\paragraph{Further results} We note that the notion of attribute and our techniques are useful not only for attacking {\sf UUDP-MIN} but also for several other models.
%
%We present several results on other models in this paper.
%
For instance we consider another well-known setting called {\em single-minded pricing} ({\sf SMP})~\cite{GuruswamiHKKKM05}, in which each consumer buys the entire bundle $S_{\Consumer}$ if she can afford to and buys nothing otherwise.
We prove that the $d$-attribute version of {\sf SMP}, called $d$-{\sf SMP}, admits the same approximation ratio as in Theorem~\ref{thm:intro thm udp smp}.
%
%As an example of $d$-{\sf SMP}, consider when a hotel is renting out its rooms (for simplicity, we assume that the hotel has unlimited number of rooms) and each customer wants to get a room for some consecutive nights. This can be captured by $2$-{\sf SMP}.
%
%
%We note that the {\em exhibition} problem in \cite{ChristodoulouEF10} can be seen as a special case of the limited-supply $4$-{\sf SMP} problem as well..






More importantly, we obtain {\sf QPTAS}s for important subroutines which are crucial building blocks in our main theorem. These results, together with a widely-believed assumption that the existence of a {\sf QPTAS} for any problem implies that {\sf PTAS} exists for the same problem (e.g., \cite{BansalCES06,ElbassioniSZ07}), imply that the approximation ratios of the aforementioned problems can be improved.  (We emphasize that this claim relies on the fact that the subroutines that we obtain {\sf QPTAS}s have {\sf PTAS}s.) They also imply that obtaining sublinear-approximation algorithms is possible even for more general problems. Here, we consider two broader models of the pricing problem. \fullonly{(see their full definitions in Section~\ref{sec: algorithms for small d})}\sodaonly{Due to the page limitation, most of the proof details are omitted in this extended abstract and can be found in the full version of our paper \cite{Fullversion}}.

%\todo{Khaled suggested writing ``{\bf we believe} the approximation ratios of the aforementioned problems...''. This sounds weird so we should talk to Khaled.}



%
%More importantly, with a widely-believed assumption that the existence of a {\sf QPTAS} for any problem implies that {\sf PTAS} exists for the same problem (e.g., \cite{BansalCES06,ElbassioniSZ07}), the approximation ratios of the aforementioned problems can be improved, and obtaining sublinear-approximation algorithms is possible even for more general problems. Here, we consider two broader models of the pricing problem. \fullonly{(see their full definitions in Section~\ref{sec: algorithms for small d})}\sodaonly{Due to the page limitation, most of the proof details are omitted in this extended abstract and can be found in the full version of our paper \cite{Fullversion}}.\todo{Khaled suggested writing ``{\bf we believe} the approximation ratios of the aforementioned problems...''. This sounds weird so we should talk to Khaled.}
\squishlist
\item The {\em unit-demand utility-maximizing pricing problem} ({\sf UDP-Util}) is a model that generalizes {\sf UUDP-MIN} in that the consumers may have different {\em valuations} on different items and want to maximize the difference between the valuations and the price of the purchased items. (This problem is sometimes called {\em envy-free pricing problem} \cite{BriestK07} and {\em max-gain-buying pricing problem} \cite{AggarwalFMZ04}. We name this problem {\sf UDP-Util} to distinguish it from other general pricing problems studied in this paper.) We show that there is an $\tilde O_d\left(n^{1-1/4^{d-1}}\right)$-approximation algorithm for a naturally defined $d$-attribute version of {\sf UDP-Util} when valuations are monotone functions of $d$ attributes (i.e., each consumer values an item not less than the inferior ones). This result also holds for the $d$-attribute version of the (non-uniform) unit-demand min-buying pricing problem ({\sf UDP-MIN}) where consumers can have different budgets on different items.

%\item The {\em multidimensional pricing problem} is a model that generalizes {\sf UUDP-MIN} in that the consumers may have different {\em valuations} on different items. Recent results show that this problem can be well-approximated in some Bayesian settings  \cite{CaiD11,ChawlaHK07}\danupon{Maybe we should cite ``Yang Cai, Constantinos Daskalakis and Matt Weinberg: An Algorithmic Characterization of Multi-Dimensional Mechanisms. ECCC Report, 2011.'' and ``Constantinos Daskalakis and Matt Weinberg: On Optimal Multi-Dimensional Mechanism Design. ECCC Report, 2011.'' Also, one of the reviewers commented that some of the previously cited papers are on mechanism design so we shouldn't cite them.}. We present  a positive result in the non-Baysian setting: there is an $\tilde O_d\left(n^{1-1/4^{d-1}}\right)$-approximation algorithm for a natural $d$-attribute version of this problem when valuations are monotone functions of $d$ attributes (i.e., each consumer values an item not less than the inferior ones).
%
\item The pricing problem with {\em symmetric valuations} and {\em subadditive revenues} is a model that includes both {\sf UUDP-MIN} and {\sf SMP} as well as many other natural problems. Informally, symmetric valuation means that each consumer's valuation only depends on the number of items she gets, and subadditive revenue implies that the amount that each consumer pays to get an item bundle $X$ is at most the amount she pays to get the items in $X$ separately. We show that there is an $\tilde O_d\left(n^{1-1/4^{d-1}}\right)$-approximation algorithm for the $d$-attribute version of this problem.
\squishend

%
%\squishlist
%\item The multidimensional pricing problem~\cite{CaiD11,ChawlaHK07,ChawlaHMS10} \danupon{Have to say ``unit-demand''?} is the problem where each consumer $\Consumer$ wants to buy an item $\Item$ that maximizes $v_\Consumer(\Item)-p(\Item)$ where $v_\Consumer(\Item)$ is the valuation of $\Consumer$ on $\Item$ and $p(\Item)$ is the price of $\Item$. This problem generalize the {\sf UDP-MIN} problem. Positive results were shown recently in \cite{CaiD11,ChawlaHK07,ChawlaHMS10}. We show one more positive result for this problem in the case where there are attributes.
%\squishend


\fullonly{
We summarize our results in the following theorem.

\begin{theorem}\label{thm:intro all}
Unless there is a problem that admits {\sf QPTAS} but no {\sf PTAS}, there exist $\tilde O_d(n^{1-1/4^{d-1}})$-approximation algorithms for (1) {\em unit-demand utility-maximizing} $d$-attribute pricing problem where valuations depend only on attributes and (2) $d$-attribute pricing problem with {\em symmetric valuations} and {\em subadditive revenues}. Moreover, there exist $\tilde O_d(n^{1-1/4^{d-2}})$-approximation algorithms for $d$-{\sf UUDP-MIN} and $d$-{\sf SMP}.
\end{theorem}
}


As a by-product of our proof, we show a {\sf QPTAS} for $2$-{\sf SMP} which subsumes the previous {\sf QPTAS} for the highway pricing problem \cite{ElbassioniSZ07}. \fullonly{We discuss this in the next subsection.}

\end{comment}

\paragraph{Hardness} We also study the hardness of approximation of our problems. We show that $3$-{\sf UUDP-MIN} and $2$-{\sf SMP} are {\sf NP}-hard, and $4$-{\sf UUDP-MIN} and $4$-{\sf SMP} are {\sf APX}-hard. Hence, our problem is already non-trivial for small $d$.
%
Our hardness proofs establish a cute connection between our problem and the vertex cover problem on graphs of low {\em order dimensions}~\cite{Schnyder89,DBLP:conf/soda/Schnyder90}.
%
%Interestingly, our proofs rely on embedding graphs of low {\em order dimensions} into Euclidean space~\cite{Schnyder89, DBLP:conf/soda/Schnyder90}.
%
%Our proofs rely on the hardness of Vertex Cover in graphs with low {\em order dimensions} (e.g. planar graphs and cubic graphs) which allow ``embedding'' into Euclidean space (through Schnyder's theorem~\cite{Schnyder89, DBLP:conf/soda/Schnyder90}).
%
Moreover, we show that the hardness of our problem tends to increase as we increase $d$, and the whole generality is captured when $d=n$. In particular, we show that when the dimension is sufficiently high (i.e. $d \geq \log^2 n$), the problems are hard to approximate to within a factor of $d^{1/4-\epsilon}$ for any $\epsilon>0$. %The result holds for both problems.
%
Table~\ref{table:current status} concludes our results for $d$-{\sf UUDP-MIN} and $d$-{\sf SMP}.


%\sodaonly{
%\begin{table}
%{
%\footnotesize
%\begin{tabular}{|c|c|c|c|c|c|c|}
%  \hline
%  {\bf Problem} & & $\mathbf{d=1}$ & $\mathbf{d=2}$ & $\mathbf{d=3}$ & $\mathbf{d=4}$ & {\bf large $\mathbf{d}$  \{range \} }\\
%  \hline
%  \multirow{2}{*}{$d$-{\sf UUDP-MIN}} & Upper bound & Polytime & {\sf QPTAS} &  & & $n^{1-\frac{1}{4^{d-1}}}$ \{constant $d$\}\\
%  & Lower bound & & & {\sf NP}-hard &  {\sf APX}-hard & $d^\epsilon$ \{$d=\omega(\log n)$\} \\
%  \hline
%  \multirow{2}{*}{$d$-{\sf SMP}} & Upper bound & Polytime & {\sf QPTAS} &  & & $n^{1-\frac{1}{4^{d-1}}}$ \{constant $d$\}\\
%  & Lower bound & & {\sf NP}-hard &  & {\sf APX}-hard & $d^\epsilon$ \{$d=\omega(\log n)$\} \\
%  \hline
%\end{tabular}
%}
%\caption{Results of $d$-{\sf UUDP-MIN} and $d$-{\sf SMP} for small values of $d$.}
%%\end{center}
%\label{table:current status}
%\end{table}
%}

\begin{table}
\begin{center}
%  \scriptsize
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|}
  \hline
  {\bf Problem} & & $\mathbf{d=1}$ & $\mathbf{d=2}$ & $\mathbf{d=3}$ & $\mathbf{d=4}$ & {\bf large $\mathbf{d}$  \{range \} }\\
  \hline
  \multirow{2}{*}{$d$-{\sf UUDP-MIN}} & Upper bound & Polytime & {\sf QPTAS} &  & & $n^{1-\frac{1}{4^{d-1}}}$ \{constant $d$\}\\
  & Lower bound & & & {\sf NP}-hard &  {\sf APX}-hard & $d^{\frac{1}{4}-\epsilon}$ \{$d=\omega(\log n)$\} \\
  \hline
  \multirow{2}{*}{$d$-{\sf SMP}} & Upper bound & Polytime & {\sf QPTAS} &  & & $n^{1-\frac{1}{4^{d-1}}}$ \{constant $d$\}\\
  & Lower bound & & {\sf NP}-hard & & {\sf APX}-hard & $d^{\frac{1}{4}-\epsilon}$ \{$d=\omega(\log n)$\} \\
  \hline
\end{tabular}
\end{center}
\vspace{-.5cm}
\caption{Results of $d$-{\sf UUDP-MIN} and $d$-{\sf SMP} for small values of $d$.}
\label{table:current status}
\vspace{-.3cm}
\end{table}


\fullonly{

\subsection{General Framework}\label{sec:framework}

We explain the general framework of the proofs in this subsection, and we will solve $d$-{\sf UUDP-MIN} to give the key ideas of our techniques in Section~\ref{sec:d udp min}. The proofs of our results can be divided into two parts.

In the first part, we essentially show that a large class of $d$-attribute pricing problems is sublinear-approximable {\em if} it is sublinear-approximable for some small $d$. This class is the class of pricing problems with {\em subadditive revenue} (informally described in the previous subsection), which includes all the aforementioned problems. Thus, in one shot we reduce our task to solving the pricing problems on a very simple input! The following informal theorem shows the essence of the first part (detail in Section~\ref{sec:dim reduction statement} and \ref{sec:dim reduction proof}).

%We call this {\em Dimension Reduction Theorem}. Since this theorem requires many formal definitions to state, we defer its formal statement to Section~\ref{sec:dim reduction proof}. The following informal statement shows the essence of this theorem.

\begin{theorem}[Dimension Reduction Theorem (Informal)] Let $\cP$ be any pricing problem with subadditive revenue. For any $d$ and $d'<d$, if there is an $\tilde O_d(1)$ approximation algorithm for the $d'$-attribute version of $\cP$ then there is an $\tilde O_d(n^{1-\varepsilon(d,d')})$-approximation algorithm for its $d$-attribute version, where $\varepsilon(\cdot)$ is a function defined as $\varepsilon(t,t') = 1/4^{t-t'}$.
\end{theorem}

In the second part we show that the aforementioned problems can be solved in the case of one and two attributes. First, the cases of  $1$-{\sf UUDP-MIN} and $1$-{\sf SMP} can be solved optimally by simple dynamic programs and sublinear-approximation algorithms of both problems thus follow. Furthermore, we show quasi-polynomial time approximation schemes ({\sf QPTAS}s) for $2$-{\sf UUDP-MIN} and $2$-{\sf SMP} as well as (1) {\em unit-demand utility-maximizing} $1$-attribute pricing problem where valuations depend only on attributes and (2) $1$-attribute pricing problem with {\em symmetric valuations} and {\em subadditive revenues}. These results rule out the possibility of these problems being {\sf APX}-hard unless $\NP \subseteq \DTIME(n^{\poly \log n})$. Thus {\sf PTAS}s for these problems are likely to exist. This, along with the Dimension Reduction Theorem, implies Theorem~\ref{thm:intro all}.


On a technical side, we note that our {\sf QPTAS} for $2$-{\sf SMP} generalizes the {\sf QPTAS} result in \cite{ElbassioniSZ07} for the Highway pricing problem as the Highway pricing problem is a special case of $2$-{\sf SMP}. However, $2$-{\sf SMP} seems to have a more complicated structure and is harder to handle. A good evidence of this is that while the Highway problem has a very simple $O(\log n)$-approximation algorithm \cite{BalcanB07}, getting a polynomial-time algorithm with $o(\sqrt{n})$ approximation guarantee for $2$-{\sf SMP} without assuming anything is already a challenging task. Obtaining $O(\log n)$-approximation algorithm or extending the {\sf PTAS} technique in \cite{GrandoniR10} to $2$-{\sf SMP} (or $2$-{\sf UUDP-MIN}) is an interesting open problem.
}

%\paragraph{Organization} %After the end of introduction, the rest of the paper is organized as follows.
%In Section \ref{sec:d udp min} we prove Theorem~\ref{thm:intro thm udp smp} by showing how to reduce the dimension by one while ensuring that the sublinear approximation ratio is preserved (see Theorem~\ref{thm: dimension reduction for UDP} below). In Section~\ref{sec:hardness}, we sketch the key ideas used in proving our hardness results. %We conclude with some open problems in Section \ref{sec:conclusion}. %Other results we mention here can be found in the full version \cite{Fullversion}.


\subsection{Related Work}\label{sec:relatedwork}

Rusmevichientong et al.~\cite{Rusmevichientong03,RusmevichientongRG06,RusmevichientongRG06-2} defined the {\em non-parametric multi-product
pricing problem}, motivated by the possibility that the data about consumers' preferences and budgets can be predicted based on previous data, which can be gathered and mined by web sites designed for this purpose, e.g., \cite{HaublTrifts00,RusmevichientongRG06-2}. This problem is what we call uniform-budget unit-demand pricing problem ({\sf UUDP}). Rusmevichientong et al. proposed many decision rules such as min-buying, max-buying and rank-buying and showed that {\sf UUDP-MIN} allows a polynomial-time algorithm, assuming the {\em price-ladder constraint}, i.e., a predefined total order on the prices of all products. Aggarwal et al.~\cite{AggarwalFMZ04} later showed that the price ladder constraint also leads to a $4$-approximation algorithm for the max-buying case, even in the case of limited supply.
%

We note that the price ladder constraint is closely related to our notion of attributes in the following sense. It can be shown that $1$-{\sf UUDP-MIN} satisfies the price ladder constraint (this is the reason we can solve it in polynomial time). Moreover, although $2$-{\sf UUDP-MIN} does not satisfy this constraint, it {\em partially} satisfies the constraint in the sense that if one item is better than another item in all attributes then we can assume that it has a higher price. This property plays an important role in obtaining {\sf QPTAS} for $2$-{\sf UUDP-MIN} and also holds for general $d$.

Other variants defined later include non-uniform and utility-maximizing unit-demand, single-minded ({\sf SMP}), tollbooth and highway models~\cite{AggarwalFMZ04,GuruswamiHKKKM05}.
%
%
These problems were later found to have important connections to
algorithmic mechanism design~\cite{AggarwalH06,BalcanB05,GuruswamiHKKKM05} and online pricing
problems~\cite{BalcanB07,BlumH05}.
%
As we mentioned in the introduction, many problems can be approximated within the factor of $O(\log m + \log n)$ and $O(n)$, and these seem to be tight.


The observation that consumers make decisions based on attributes has been used in  other areas outside computer science. For example, most pricing models are captured by the {\em two-stage consider-then-choose} model (e.g., \cite{Gensch87,Payne82,PayneBJ88,GilbrideAllenby,HaublTrifts00,JedidiK05,HauserTEBS10,LiuArora2011}) in marketing research: Each consumer first screens out some undesirable items ({\em screening process}) and is left with the consideration set which is used to make a final decision. Pricing problems such as {\sf UUDP-MIN} are the case where consideration sets are arbitrary (as defined in, e.g. \cite{Shocker91,HauserW90}) while the final decision is simplified to, e.g., buying the cheapest item.



The idea of using the consideration sets defined from attributes is called {\em attribute-based screening process}~\cite{GilbrideAllenby} in marketing research where it was shown to be a rational choice for trading off between accuracy and cognitive effort~\cite{Bettman79,BettmanJP90,BettmanPark80,Shugan80}. Our model is equivalent to the attribute-based screening process  with {\em conjunctive screening rules} (e.g., \cite{GilbrideAllenby,LiuArora2011}). This type of rules was justified by many studies that it is what consumers typically use when making decisions (e.g., \cite{Bettman79,GilbrideAllenby,HauserTEBS10}).


==> arxiv 7.24.2012/omitted_hardness.tex <==
\section{Omitted hardness results}\label{sec:omitted_hardness}



\subsection{Hardness of 3-{\sf UUDP-MIN} and 4-{\sf UUDP-MIN}}

In this section we show that $3$-{\sf UUDP-MIN} is \NP-hard, and
$4$-{\sf UUDP-MIN} is \APX-hard by a reduction from {\sf Vertex Cover}. Our
reduction relies on the concepts of adjacency poset and its
embedding into Euclidean space. We describe basic terminologies
here. Given a graph $G=(V,E)$, an adjacency poset $(V \cup E,
\preceq_G)$ of graph $G$ can be constructed as follows: First we
define a poset with its maximal elements corresponding to vertices in $V$ and its minimal
elements corresponding to edges $E$. For each vertex $v$ and each edge $e$, we
have the relation $e \preceq_G v$ if and only if vertex $v$ is an endpoint of
$e$. We say that a map $\phi: V \cup E \rightarrow \R^d$ is an {\em
embedding} of adjacency poset $(V \cup E, \preceq_G)$ into $\R^d$
if and only if it preserves the relations $\preceq_G$, i.e., for any two
elements $a,b \in V \cup E$, we have that $a \preceq_G b$ iff $\phi(a)[i] \leq \phi(b)[i]$ for all coordinates $i \in [d]$.

Now we describe our reductions. Since two reductions are essentially the same, we give a general procedure which will imply both results. Given an instance $G=(V,E)$ of {\sf Vertex Cover}, we first construct an adjacency poset $(V \cup E, \preceq_G)$ for $G$,
and then we compute the embedding $\phi$ of this poset into Euclidean space $\R^d$. We will use the graph $G$, as well as the embedding $\phi$, to define the instance of $d$-{\sf UUDP-MIN} as follows:

\begin{itemize}
\item {\bf Consumers:} We have two types of consumers, i.e. the rich consumers and the poor ones. For each vertex $v \in V$, we create a {\em rich} consumer $C_v$ with budget $2$ at coordinates $\phi(v)$. For each edge $e \in E$, we create a {\em poor} consumer $C_e$ with budget $1$ at coordinates $\phi(e)$.

\item {\bf Items:} For each vertex $v \in V$, we create item ${\bf I_v}$ at coordinates $\phi(v)$.
\end{itemize}
%
Note that for each $e=(u,v)$, each poor consumer $C_e$ has $S_{C_{e}} = \set{\Item_v, \Item_u}$, while each rich consumer $C_v$ has $S_{C_v} = \set{\Item_v}$. We denote the resulting instance by $(\cset, \iset)$.

The following lemma gives a characterization of the optimal solution for $(\cset, \iset)$. It says that we may assume without loss of generality that every poor consumer gets some item.

\begin{lemma}
For any price $p$ that is a solution for $(\cset, \iset)$ constructed above, we can transform $p$ to $p'$ such that every poor consumer buys some item with respect to $p'$, and the revenue of $p'$ is at least as much as the revenue of $p$.
\end{lemma}

\begin{proof}
Consider edge $e=(u,v)$. Suppose poor consumer $C_e$ does not get
any item, so it implies that both items ${\bf I}_u$ and ${\bf I}_v$
have price $p({\bf I}_u)= p({\bf I}_v) =2$ (recall that, since budgets are $1$ or $2$, the optimal prices would never set prices that are not in $\set{1,2}$). We define the price function $p'$ by setting
$p'({\bf I}_u) = 1$ while $p'({\bf I}_w) = p({\bf I}_w)$ for all
other vertices $w \in V \setminus \set{u}$. The only rich consumer that gets affected is $C_u$, whose payment may decrease by one. However, we earn the revenue of one back from poor consumer $C_e$. For $e' \in E: e'\neq e$, poor consumer $C_{e'}$ is never affected because his budget is one. Overall, changing the price from $p$ to $p'$ never decreases revenue.
\end{proof}

Let $p^*$ be the optimal price for $(\cset, \iset)$ and ${\sf VC}(G)$ denote the size of
minimum vertex cover of $G$. We show the following connection
between the size of minimum vertex cover and the optimal revenue
collected by $p^*$.

\begin{theorem}
The optimal revenue collected by $p^*$ is exactly $2n-{\sf VC}(G)
+m$.
\end{theorem}
\begin{proof}
From the previous lemma, we can assume that the pricing $p^*$ sells
items to every poor consumer. In other words, if $V' = \set{v:
p^*({\bf I}_v)=1}$, it must be the case that $V'$ is a vertex cover:
otherwise, let $e=(u,w)$ be an edge which is not covered by any
vertex in $V'$, so $C_e$ is only interested in items with price $2$,
which he cannot afford. This contradicts the assumption that $p^*$
sells items to every poor consumer.

The revenue collected from poor consumers is exactly $m$. Each rich
consumer $C_v$ in the vertex cover gets the item with price $1$ while
others get the items with price $2$, so the total revenue is $m + {\sf
VC}(G) + 2(n - {\sf VC}(G))$.
\end{proof}

This theorem immediately implies the gap between {\sc Yes-Instance} and {\sc No-Instance} for $d$-{\sf UUDP-MIN}. The only detail we left out is the computation of the embedding $\phi$, and this is where the hardness proofs
of $3$-{\sf UUDP-MIN} and $4$-{\sf UUDP-MIN} depart (other steps are
exactly the same). For $3$-dimensional case, we start from planar
graphs whose adjacency poset can be embedded into $\R^3$. Since
planar vertex cover has a polynomial-time approximation scheme, we
only get \NP-hardness here. For $4$-dimensional case, we start from
vertex cover in cubic graphs, which is known to be \APX-hard, but
unfortunately we can only embed its adjacency poset into $\R^4$,
thus obtaining the hardness of $4$-{\sf UUDP-MIN}.

\paragraph{\NP-Hardness of $3$-{\sf UUDP-MIN}}

To show the \NP-hardness, we start from {\sf Vertex Cover} in planar graphs, which is known to be \NP-complete~\cite{DBLP:journals/tcs/GareyJS76}. We will use the following theorem,
due to Schnyder~\cite{Schnyder89}.

\begin{theorem}
Let $(V \cup E, \preceq_G)$ be an incident poset of planar graph
$G$. Then there exists an embedding $\phi$ from the poset into
$\R^3$.
\end{theorem}

Schnyder shows later that the crucial step in the theorem
can be computed in polynomial time \cite{DBLP:conf/soda/Schnyder90}, which
immediately implies the following theorem.

\begin{theorem}
$3$-{\sf UUDP-MIN} is \NP-hard even when the consumer budgets are
either $1$ or $2$.
\end{theorem}



\paragraph{\APX-Hardness of $4$-{\sf UUDP-MIN}}

We will be using the fact that {\sf Vertex Cover} in cubic graphs
is \APX-hard \cite{DBLP:conf/ciac/AlimontiK97}, stated in the
language convenient for our use below.

\begin{theorem}
For some $0 < \alpha < \beta < 1$, it is \NP-hard to distinguish
between (i) the graph that has a vertex cover of size at most
$\alpha n$, and (ii) the graph whose minimum vertex cover is at
least $\beta n$.
\end{theorem}

Now we assume that our input graph $G$ is a cubic graph and use the
following theorem to embed the adjacency poset of $G$ into $\R^4$.

\begin{theorem}[Schnyder]
An adjacency poset of any $4$-colorable graph can be embedded into
$\R^4$. Moreover, the embedding is computable in polynomial time.
\end{theorem}

It only requires a straightforward computation to prove the
following theorem.
\begin{theorem}
$4$-{\sf UUDP-MIN} is \APX-hard even when the consumer budgets are
either $1$ or $2$.
\end{theorem}
\begin{proof}
In the \yi, we can collect the revenue of $(2-\alpha) n +m$.
However, in the \ni, the revenue is at most $(2-\beta)n +m$. Since
the graph is cubic, we may assume that $m =\gamma n$ for some $1\leq
\gamma <2$. Hence we have a gap of
$(2-\alpha+\gamma)/(2-\beta+\gamma)$.
\end{proof}

\subsection{\NP-hardness of $2$-{\sf SMP}}

Highway problem can be defined as follows: We are given a line $P = (v_0,\ldots, v_n)$ consisting of $n$ edges and $n+1$ vertices and a set of consumers $\cset$ where each consumer $\Consumer$ corresponds to a subpath $P_{\Consumer}$ of $P$ and is equipped with budget $B_\Consumer$. Our goal is to set price to edges so as to maximize the revenue, where each consumer $\Consumer$ buys a path $P_{\Consumer}$ if she can afford the whole path; otherwise she buys nothing.

\begin{lemma}
There is a polynomial-time algorithm that transforms an instance of Highway problem to an instance of $2$-{\sf SMP}.
\end{lemma}

\begin{proof}
For each $i=1,\ldots, n$, each edge $(v_{i-1}, v_i)$, we create an item $\Item_i$ at coordinates $(i, n+1-i)$. Then for each consumer $\Consumer$ whose path is $P_\Consumer = (v_s,\ldots, v_t)$, we create a consumer point at $(s+1, n+1-t)$. It is easy to see that the consideration set remains unchanged.
\end{proof}

\subsection{\APX-hardness of $4$-{\sf SMP}}

We perform a reduction from {\sf Graph Vertex Pricing} on bipartite graphs. In this problem, we are given a graph $G=(V,E)$, where each vertex corresponds to item and each edge $e \in E$ corresponds to a consumer, additionally equipped with budget $B_e$. Each consumer edge is interested in items that correspond to her incident vertices. Our goal is to set a price $p: V \rightarrow \R$ so as to maximize our revenue.

Given an instance $(G, \set{B_e}_{e \in E})$ of {\sf Graph Vertex Pricing} where graph $G$ is a bipartite graph $(U \cup W, E)$, we create an instance of $4$-{\sf SMP} as follows. Suppose we have $U = \set{u_1,\ldots, u_{|U|}}$ and $W = \set{w_1,\ldots, w_{|W|}}$. For each vertex $u_i \in U$, we have a corresponding item $\Item^u_{i}$ with coordinates $(i, |U|+1-i, \infty,\infty)$. Similarly, for each vertex $w_j \in W$, we have a corresponding item $\Item^w_{j}$ with coordinates $(\infty,\infty,j, |W|+1-j)$. Finally, for each edge $(u_i, w_j) \in E$, we have a consumer $\Consumer_{ij} = (i, |U|+1-i, j, |W|+1-j)$, whose budget is the same as the budget of edge $(u_i,w_j)$. The following claim is almost immediate.

\begin{claim}
For each consumer $\Consumer_{ij}$, we have that $S_{\Consumer_{ij}} = \set{\Item^u_i, \Item^w_j}$
\end{claim}

\begin{proof}
It is easy to see that $\set{\Item^u_i, \Item^w_j} \subseteq S_{\Consumer_{ij}}$. Notice that for $i'<i$, we have $\Consumer_{ij}[1] > \Item^u_{i'}[1]$, so any such item $\Item^u_{i'}$ cannot belong to $S_{\Consumer_{ij}}$. Similarly for $i' >i$, we have $\Consumer_{ij}[2] > \Item^u_{i'}[2]$, so such an item cannot belong to $S_{\Consumer_{ij}}$. By using similar arguments for items of the form $\Item^w_{j'}$ for $j' \neq j$, we reach the conclusion that $S_{\Consumer_{ij}} = \set{\Item^u_i, \Item^w_j}$.
\end{proof}

Since the $4$-{\sf SMP} instance is equivalent to the instance of {\sf Graph Vertex Pricing}, the maximum revenue is preserved. Using the \APX-hardness result of {\sf Graph Vertex Pricing} on bipartite graphs~\cite{KhandekarKMS09}, we conclude that $4$-{\sf SMP} is \APX-hard.





%\input{higherdimension}



==> arxiv 7.24.2012/overviewH_ec.tex <==
\section{Sub-linear Approximation Algorithm (Proof of Theorem~\ref{thm:intro thm udp smp})}\label{sec:d udp min}

To simplify the presentation, we present the algorithm for $d$-{\sf UUDP-MIN} in this section. The algorithm for $d$-{\sf SMP} is almost identical. Let $\cset$ and $\iset$ be the set  of points in $\mathbb{R}^d$, where every consumer $\Consumer\in{\cal C}$ has budget $B_{\Consumer}$ and consideration set $S_{\Consumer}$ which is specified by coordinates of the input point. For any subset $\mathcal{C}'\subseteq\cset$ and ${\cal I}'\subseteq \iset$, let
$\mathcal{P}(\cset',\iset')$ be the $d$-{\sf UUDP-MIN} problem with input $\cset'$ and $\iset'$. Moreover, for any $\cset'$ and $\iset'$, we use $\opt(\cset', \iset')$ to express the optimal revenue of the instance $(\cset', \iset')$. At a high level, our algorithm proceeds in an inductive manner and obtains a solution of $d$-{\sf UUDP-MIN} problem by invoking the algorithms for $(d-1)$-{\sf UUDP-MIN} and $1$-{\sf UUDP-MIN} as a subroutine. Our result is summarized in the following theorem.

\begin{theorem}
\label{thm: dimension reduction for UDP}
For any $\epsilon \in (0,1]$, if there is an $\tilde O_d(n^{1-\epsilon})$-approximation algorithm for $(d-1)$-{\sf UUDP-MIN} then there is an $\tilde O_d(n^{1-\epsilon/4})$-approximation algorithm for $d$-{\sf UUDP-MIN} as well.
\end{theorem}

Theorem~\ref{thm:intro thm udp smp} then follows from the fact that $1$-{\sf UUDP-MIN} can be solved optimally in polynomial time (see Appendix~\ref{sec:one udp min}\fullonly{ and its generalization in Section~\ref{sec: algorithms for small d}}). As we noted earlier, it can be improved slightly since $2$-{\sf UUDP-MIN} admits {\sf QPTAS} \sodaonly{(see Appendix~\ref{sec: qptas 2 udp})}\fullonly{(see Section~\ref{subsection: qptas minbuying})}.
%
%\begin{corollary}
%For any constant $d$, there is an approximation algorithm that gives a sub-linear approximation guarantee for $d$-{\sf UDP-MIN}.
%\end{corollary}


\subsection{Consideration-preserving Decomposition}

Our algorithm partitions the input instance into many subinstances and tries to collect the profit from some of them. The notion of consideration-preserving decomposition, defined below, allows us to do so without losing revenue.

\begin{definition}\label{def:decomposition} We call a collection $\set{(\cset'_1,\iset'_1),\ldots, (\cset'_k, \iset'_k)}$  a {\em consideration-preserving decomposition} of the problem $(\cC, \cI)$ if and only if for any $\Consumer \in \cset$ and $\Item \in S_{\Consumer}$, there exists (not necessarily unique) $i$ such that $\Consumer \in \cset'_i$ and $\Item \in \iset'_i$.
%and (2) for any $\Consumer \in \cset$ and $\Item \notin S_{\Consumer}$, there is no $i$ such that $\Consumer \in \cset'_i$ and $\Item \in \iset'_i$.
\end{definition}
%


By definition, for any consumer $\Consumer$ and item $\Item$ the fact that consumer $\Consumer$ considers item $\Item$ is preserved by at least one instance $(\cset'_i, \iset'_i)$. The following lemma says that this decomposition preserves the total revenue.


\begin{lemma}
\label{lemma: UDP decomposition}
For any consideration-preserving decomposition $\left\{(\cset'_1,\iset'_1), \ldots, (\cset'_k, \iset'_k)\right\}$ of $(\cset, \iset)$, it holds that
$\sum_{i=1}^k \opt(\cset'_i, \iset'_i)\geq \opt(\cset, \iset)
\,.$
Moreover, any price function for $\pset(\cset'_i, \iset'_i)$ can be extended to a price function for the original problem $\pset(\cset, \iset)$ that gives revenue at least $\opt(\cset'_i, \iset'_i)$.
\end{lemma}


\iffalse
\sodaonly{\begin{proof}[Proof Idea]}
\fullonly{\begin{proof}[Proof idea]}
(See Appendix~\ref{sec: proof of UDP decomposition lemma} for the full proof.)
Let $p^{\star}:\iset\rightarrow\mathbb{R}$ be the optimal price function for  $\pset(\cset, \iset)$. It is straightforward to see that, for any consumer $\Consumer$, the optimal revenue that $\Consumer$ gets from any subset of $\iset$ is at least the optimal revenue $\Consumer$ gets when considering the set $\iset$. This proves the first statement.

For the second one, let $p$ be a price function for $\pset(\cset_i, \iset_i)$. We extend $p$ to $p':\iset\rightarrow\R$ defined by $p'(\Item)=p(\Item)$ if $\Item\in\iset_i$, and $p'(\Item)=\infty $ otherwise.
\end{proof}
\fi


This is simply by applying the optimal price function of one problem to the other (see Appendix~\ref{sec: proof of UDP decomposition lemma} for the full proof). In the rest of our discussion, we mainly use two different types of consideration-preservation decomposition, as explained in the following observation.


\begin{observation}\label{observation: conseration preserving decomposition}
Given an input instance $(\cset',\iset')$, let $\cset' = \bigcup_{i=1}^k \cset'_i$. Then $\{(\cset'_1,\iset')$, $\ldots$, $(\cset'_k, \iset')\}$ is a consideration-preserving decomposition of $(\cset', \iset')$. Similarly, if $\iset' = \bigcup_{i=1}^k \iset'_i$, then we have that $\set{(\cset',\iset'_1), \ldots, (\cset', \iset'_k)}$ is a consideration-preserving decomposition of $(\cset', \iset')$.
\end{observation}



\subsection{Algorithm}


%
%\begin{figure}[tb]
%  % Requires \usepackage{graphicx}
%  \center\includegraphics[width=3in]{overview.pdf}
%  \vspace{-0.3cm}
%  \caption{Decomposition overview}\label{fig:overview}
%\end{figure}

%\begin{figure}[tb]
\begin{wrapfigure}{r}{0.5\textwidth}
  % Requires \usepackage{graphicx}
  \vspace{-1.5cm}
  \center\includegraphics[width=\linewidth]{overview.pdf}
  \vspace{-.5cm}
  \caption{Decomposition overview}\label{fig:overview}
  \vspace{-.5cm}
%\end{figure}
\end{wrapfigure}
%
At a high level, the algorithm proceeds in four steps where each step involves consideration-preserving decomposition (see Fig.~\ref{fig:overview} for an overview). In Step 1, we partition $\iset$ into different subsets where
 every subset satisfies certain properties, i.e. the elements in each subset either form a chain or an antichain. The problem on those subsets
  in which elements form a chain can be solved easily, and we deal with the antichains in later steps. In Step 2, we partition consumers in $\cset$ into two types, those with large and small consideration sets. We use the algorithm of \cite{BalcanB07,BriestK11} to deal with consumers with small consideration sets and handle the rest consumers in later steps. In Step 3, we find a subset of items, i.e. a ``hitting set'',  and partition consumers further into several sets. Each set of consumers has the following property: There is some item desired by all consumers in the set. Using this property, we show in Step 4 that the problem can be further partitioned into a few problems where each of them can be viewed as a $(d-1)$-{\sf UUDP-MIN} problem. (We call this a ``consideration-preserving embedding''.)



%Consider any $\cset'_1, \ldots, \cset'_k\subseteq \cset$ and $\iset'_1, \ldots, \iset'_k$ such that, for any $\Consumer$ and $\Item\in S_\Consumer$, there exists $i\leq k$ such that $\Consumer\in \cset'_i$ and $\Item\in \iset'$. Observe that $\sum_{i=1}^k \opt(\cset_i, \iset_i)\geq \opt(\cset, \iset)$. Moreover, we can achieve the revenue of $\opt(\cset_i, \iset_i)$ by pricing all $\iset\setminus \iset_i$ to infinity and all items in $\iset$ to the price we use to achieve $\opt(\cset_i, \iset_i)$ when the input consists of $\cset_i$ and $\iset_i$.

%Secondly, we note that $1$-{\sf UDP-MIN} can be solved optimally by a simple dynamic program.

%Our main goal is to find $\cset'\subseteq \cset$ and $\iset'\subseteq \iset$ such that $\opt(\cset', \iset')=\Omega(\opt(\cset, \iset)/n^{3/4})$ and the $2$-{\sf UDP-MIN} problem on input $(\cset', \iset')$ can be solved optimally by reducing to a $1$-{\sf UDP-MIN} problem. We do this in several steps as follows.

\paragraph{\underline{Step 1:} Partitioning items into chains and antichains}
%\subsection{Step 1: Partitioning items into chains and antichains}\label{sec:step 1}

Let $(\cset, \iset)$ be an input of $d$-{\sf UUDP-MIN}. First we define a partially ordered set $(\iset, \leq)$ on the item set as follows. We say that $\Item_1 \leq \Item_2$ if and only if $\Item_1$ has a lower quality than $\Item_2$ in every attribute, i.e. $\Item_1[d'] \leq \Item_2[d']$ for all $d' \in [d]$.
%
We say that a subset $\iset' \subseteq \iset$ is a chain if $\iset'$ can be written as $\iset'= \set{\Item_1,\ldots, \Item_z}$ such that $\Item_j \leq \Item_{j+1}$ for all $j\in[z-1]$. We say that $\iset' \subseteq \iset$ is an antichain if and only if for any pair of items $\Item, \Item' \in \iset'$, neither $\Item \leq \Item'$ nor $\Item' \leq \Item$.



\begin{lemma}
\label{lemma: chain decomposition}
For any $\epsilon >0$ and any $s = n^{\epsilon/4}, t= n^{1-\epsilon/4}$, we can partition $\iset$ into $A_1, \ldots, A_s$ and $B_1, \ldots, B_t$ in polynomial-time. Moreover, each $A_i$ is an antichain and each $B_j$ is a chain.
\end{lemma}
\sodaonly{\begin{proof}[Proof Idea]}
\fullonly{\begin{proof}[Proof idea]}
(See Section~\ref{sec:detail one} for detailed definitions and proofs.)
By Dilworth's theorem \cite{Dilworth,Fulkerson-Dilworth}, the minimum chain decomposition equals to the maximum antichain size. We will use the fact that both minimum chain decomposition and maximum-size antichain can be computed in polynomial time as follows:
As long as the maximum-size antichain is bigger than $n^{\epsilon/4}$, we repeatedly extract such an antichain out of the input; otherwise, we would have the decomposition into at most $n^{\epsilon/4}$ chains, so we stop.
\end{proof}

By Observation~\ref{observation: conseration preserving decomposition}, the collection
%\[
$\{(\cset, A_1), \ldots, (\cset, A_s), (\cset, B_1), \ldots, (\cset, B_t)\}$
%\]
 is a consideration-preserving decomposition of $(\cset, \iset)$. It follows by Lemma~\ref{lemma: UDP decomposition} that
%\[
$\sum_{i=1}^s\opt(\cset, A_i)+\sum_{j=1}^t \opt(\cset, B_j) \geq \opt(\cset, \iset).$
%\]
Further, observe that if there exists $j$ such that $\opt(\cset, B_j)\geq\opt(\cset, \iset)/(2n^{1-\epsilon/4})$, then we would be done: the $d$-{\sf UUDP-MIN} problem $\pset(\cset, B_j)$ can be seen as a $1$-{\sf UUDP-MIN} problem (since $B_j$ is a chain) and hence can be solved optimally! (See  Lemma~\ref{lem:chain to one dim} for detailed analysis)
 Otherwise $\opt(\cset, B_j)\leq \opt(\cset, \iset)/ (2n^{1-\epsilon/4})$ for every $j$. Therefore
% \[
$\sum_{j=1}^t \opt(\cset, B_j) \leq n^{1-\varepsilon/4}\cdot\opt(\cset,\iset)/ (2n^{1-\varepsilon/4})< \opt(\cset,\iset)/2.$
% \]
 If this is not the case then we know that there must be an antichain $A_i$ such that
%\begin{equation*}
$\opt(\cset, A_i)\geq \opt(\cset,\iset)/2n^{\epsilon/4}\,.$
%\end{equation*}
%
%We now proceed to the next step.

%Our goal now is to $O(n^{1/2})$-approximate the problem on such $A_i$.

%\begin{figure}
\begin{wrapfigure}{r}{.5\textwidth}
  % Requires \usepackage{graphicx}
  \vspace{-.9cm}
  \center\includegraphics[width=\linewidth]{step1.pdf}\\
  \vspace{-.3cm}\caption{Example of Step 1}\label{fig:step1}\vspace{-.2cm}
%\end{figure}
\end{wrapfigure}


%\paragraph{Step 2: Dealing with small consideration sets.}
\paragraph{\underline{Step 2:} Dealing with small consideration sets}
For simplicity, let us assume that we know $i$ such that $\opt(\cset, A_i)\geq \opt(\cset, \iset)/(2n^{\epsilon/4})$. Now we focus on collecting revenue from the subproblem $\pset(\cset, A_i)$. Let $\cset_1 \subseteq \cset$ be the set of consumers who are interested in at most $n^{1-2\epsilon/4}$ items in $A_i$, i.e. $\cset_1=\left\{\Consumer\in \cset: |S_\Consumer\cap A_{i}|\leq n^{1-2\epsilon/4}\right\}$, and define $\cset_2=\cset\setminus \cset_1$.
Since $\{(\cset_1, A_i), (\cset_2, A_i)\}$ is a consideration-preserving decomposition of $(\cset, A_i)$, we have
%\[
$\opt(\cset_1, A_i)+\opt(\cset_2, A_i) \geq \opt(\cset, A_i) \geq \frac{\opt(\cset, \iset)}{2n^{\epsilon/4}}.$
%\]
%
%$\opt(\cset_1, A_i)+\opt(\cset_2, A_i)\geq \opt(\cset, A_i)\geq \opt(\cset, \iset)/2n^{\epsilon/4}$ because $\{(\cset_1, A_i), (\cset_2, A_i)\}$ is a decomposition of $(\cset, A_i)$.
%
Now we need an algorithm of \cite{BalcanB07,BriestK11}. Balcan and Blum give an approximation algorithm for {\sf SMP} whose approximation guarantee depends on the sizes of consideration sets. Briest and Krysta, by using a slight modification of this algorithm, give an approximation algorithm with the same guarantee for {\sf UDP-MIN}. Their result, stated in terms of {\sf UUDP-MIN}, is summarized in the following theorem. (For completeness, we provide the proof in Appendix~\ref{sec:balcanblum for udp min}.)


\begin{theorem}\label{theorem:BalcanBlum}\cite{BalcanB07,BriestK11}
Given a {\sf UUDP-MIN} instance $(\cset, \iset, \set{S_{\Consumer}}_{\Consumer \in \cset})$, there is a deterministic $O(k)$-approximation algorithm of {\sf UUDP-MIN}, where  $k: = \max_{\Consumer \in \cset} \size{S_{\Consumer}}$.
\end{theorem}

%\danupon{I removed the following sentence ``We note that in fact the algorithm in~\cite{BalcanB07} is for {\sf SMP}, but it is possible to generalize their algorithm to give the same guarantee for {\sf UDP-MIN} (and, in fact, any pricing problem with subadditive revenue; see the full version for detail) For completeness, we provide the proof in Appendix~XXX.'' since this was already observed in \cite{BriestK07} (also mentioned in the journal version of \cite{balcanB07}).}

We remark that we extend this technique to deal with any pricing problem with subadditive revenue in the full version of this paper.


If $\opt(\cset_1, A_i)\geq \opt(\cset, \iset)/(4n^{\epsilon/4})$, then we could invoke the algorithm in Theorem~\ref{theorem:BalcanBlum} on $(\cset_1, A_i)$ to get a solution with approximation ratio
%\[
$O\left(\max_{\Consumer \in \cset_1} \size{S_{\Consumer}\cap A_i}\right)=O(n^{1-2\epsilon/4}).$
%\]
 This yields a solution that gives a desired revenue of
$\Omega\left(\opt(\cset_1, A_i)/n^{1-2\epsilon/4}\right)=\Omega\left(\opt(\cset, \iset)/n^{1-\epsilon/4}\right)\,.$
 Otherwise we have $\opt(\cset_1, A_i)< \opt(\cset, \iset)/4n^{\epsilon/4}$. Then
%\begin{align*}
$\opt(\cset_2, A_i)=\Omega\left(\opt(\cset, \iset)/n^{\epsilon/4}\right).$
%\end{align*}
We will deal with this case in the next steps.

%... Note that $|A_i|$ could be as large as $\Omega(n)$....


%\paragraph{Step 3: Partitioning consumers using a small hitting set obtained from the epsilon net.}
\paragraph{\underline{Step 3:} Partitioning consumers using a small hitting set}
%From now on, we only focus on the instance $(\cset_2, A_i)$ which corresponds to the consideration set system $\{S_{\Consumer}\}_{\Consumer\in \cC_2}$ where $S_{\Consumer}=\{\Item\in A_i\mid \Item\geq \Consumer\}$.
%We claim that we can, in randomized polynomial time, find a set $H\subseteq A_i$ of size $\tilde O(n^{2\epsilon})$ that is a {\em hitting set} of $\cC_2$, i.e., $S_\Consumer\cap H\neq \emptyset$ for all $\Consumer\in \cset_2$.
%
%We claim the following.% lemma (detail in Section~\ref{sec:detail three}).
First, we apply the epsilon net theorem~\cite{Chazelle-book,Epsilon-net} to derive the following lemma.
%
\begin{lemma}\label{lem:hitting set}
We can find a set $H\subseteq A_i$ of size $\tilde O(n^{2\epsilon})$ in randomized polynomial time such that for any $\Consumer\in \cset_2$, there exists $\Item\in H$ such that $\Item\geq \Consumer$.
%$S_\Consumer\cap H\neq \emptyset$ for all $\Consumer\in \cset_2$.
\end{lemma}
%
%
%This lemma follows from the epsilon net theorem~\cite{Chazelle-book,Epsilon-net} which roughly states that, for any $\delta>0$, if the set system has low VC dimension and all sets have size at least $n^\delta$ then there is a hitting set of size $\tilde O(n^{1-\delta})$; here, we use $\delta=1-2\epsilon$, and our sets $S_\Consumer$ have $O(1)$ VC dimension because they can be seen as {\em $d$-dimensional boxes}.\danupon{If we are not using ``box'' anymore. We should change here as well.} (See Section~\ref{sec:detail three} for detail.)
%
\begin{proof}
%As noted before,
%$\{S_{\Consumer}\}_{\Consumer\in \cC_2}$ where $S_{\Consumer}=\{\Item\in A_i\mid \Item\geq \Consumer\}$.
%
\danupon{We should consider providing a bit more detail (``a primer'') in the Appendix.}
%
The instance $(\cC_2, A_i)$ defines a set system $\{S_\Consumer\}_{\Consumer\in \cC_2}$ over $A_i$, where $S_\Consumer=\{\Item\in A_i\mid \Item\geq \Consumer\}$. We note that each set $S_{\Consumer}$ has {\em descriptive complexity} at most $d$,  i.e. set $S_{\Consumer}$ can be described by $d$ linear inequalities of the form $S_{\Consumer} = \bigcap_{d'=1}^d \set{\Item \in \iset: \Item[d'] \geq \Consumer[d']}$. In this case, this set system has VC dimension $O(d)$, c.f. \cite{Sharir-book}. More specifically, it is well known (e.g., \cite{AronovES10}) that any collection of $d$-dimensional axis-parallel boxes has VC dimension $O(d)$. We will not formally define VC-dimension here. The following theorem is all we need.

\begin{theorem}(\cite{Chazelle-book,Epsilon-net}; Epsilon net theorem)
Let $\xset$ be a set system of VC-dimension at most $d'$ over $N$. Then for any $\delta \in (0,1)$, we can find a set $H \subseteq N$ with $\size{H} = O(\frac{d'}{\delta}\log \frac{d'}{\delta})$ in randomized polynomial time such that, for all $X_i \in \xset$ with $\size{X_i} \geq \delta \size{N}$, it holds that  $H \cap X_i \neq \emptyset$.
\end{theorem}
%
%
Using the theorem with $\delta = n^{-2\epsilon/4}$, we can find a set $H \subseteq A_i$ of size at most $\tilde{O}(n^{2\epsilon/4})$, and since we have $|S_{\Consumer} \cap A_i| \geq \delta n$ for all $\Consumer \in \cset_2$, we are guaranteed that $H \cap S_{\Consumer} \neq \emptyset$ for all $\Consumer \in \cset_2$.
\end{proof}


We call $H$ a {\em hitting set} of $\cC_2$ since $H$ intersects $S_\Consumer$ for all $\Consumer\in \cC_2$. We use $H$ to decompose $(\cC_2, A_i)$ into a small number of subproblems and show in Step 4 that each of these problems can be viewed as a $(d-1)$-{\sf UUDP-MIN} problem.

For each $\Item\in H$, let $\cset_\Item=\{\Consumer\in \cset_2\mid \Item \in S_\Consumer\}$, i.e., $\cset_\Item$ consists of all consumers in $\cset_2$ that consider item $\Item$. Observe that $\bigcup_{\Item \in H} \cset_{\Item} = \cset_2$, and therefore by Lemma~\ref{lemma: UDP decomposition}, we have
%\[
$\sum_{\Item \in H} \opt(\cset_\Item, A_i)\geq \opt(\cset_2, A_i)
\geq \Omega\left(\opt(\cset, \iset)/n^{\epsilon/4}\right).$
%\]
%
Since $\size{H}=O(n^{2\epsilon/4})$, there exists $\Item^*\in H$ such that
\begin{align*}
\opt(\cset_{\Item^*}, A_i) &=\tilde\Omega\left(\opt(\cC, \cI)\cdot n^{-\epsilon/4}/|H|\right)
=\tilde\Omega\left(\opt(\cC, \cI)/n^{3\epsilon/4}\right).
\end{align*}
%
Now we, again, assume that we know $\Item^*$ and turn our focus to the subproblem $\pset(\cset_{\Item^*}, A_i)$.

%For notational convenience, we abbreviate $\cset_{\Item^*}$ by $\tilde{\cset}$ and $A_i$ by $\tilde{\iset}$.\danupon{I think there is no need to change to notation.}




%\paragraph{Step 4: Reducing the dimension.} We have now reached the most crucial step.
\paragraph{\underline{Step 4:} Reducing the dimension} We have now reached the most crucial step.
%
%Recall that we now have the problem $(\cC_2, A_i)$ that satisfies Eq.\eqref{eq:C2Ai} and its hitting set $H$ of size $O(n^{2\epsilon/4})$.
%
We will (crucially) rely on the fact that all consumers in $\cset_{\Item^*}$ consider item $\Item^*$, and that $A_i$ is an antichain.
%
%We now decompose the problem on $C_{\Item^*}$ and $A_i$ into two problems that are equivalent to {\sf $1$-UDP-MIN}.
%
For each $j \leq d$,  define $A_i^j$ as the set of items in $A_i$ that are at least as good as $\Item^*$ in the $j$-th coordinate, i.e., $A_i^j=\{\Item\in A_i \mid \Item[j]\geq \Item^*[j]\}$. See Fig.~\ref{fig:step4_1} for an example in the case of $2$-{\sf UUDP-MIN}.

%
%That is, for $j=1, 2$, let $\cset_{\Item^*}^j=\{\Consumer\in \cset_{\Item^*} \mid \Consumer[j]\leq \Item^*[j]\}$ and $A_i^j=\{\Item\in A_i \mid \Item[j]\geq \Item^*[j]\}$.
%
%Observe that
%\begin{equation}
%A_i = \bigcup_{j=1}^d A_i^j\label{eq:union of d dimensions}
%\end{equation}
\begin{lemma}\label{lem:union of d dimensions}
$A_i = \bigcup_{j=1}^d A_i^j$.
\end{lemma}
%
%\begin{wrapfigure}{r}{.5\textwidth}
%%\begin{figure}
%  % Requires \usepackage{graphicx}
%  \vspace{-2cm}%\hspace{-1cm}
%  \center\includegraphics[width=\linewidth, clip=true, trim=1.5cm .3cm 1cm .3cm]{step3.pdf}
%  \vspace{-.9cm}\caption{Example of Step 4}\label{fig:step4_1}\vspace{-.4cm}
%%\end{figure}
%\end{wrapfigure}
%%
%\begin{wrapfigure}{r}{0.35\textwidth}
%%\begin{figure}
%  % Requires \usepackage{graphicx}
%  \vspace{-.8cm}
%  \center\includegraphics[width=\linewidth, clip=true, trim=3cm .75cm 7cm 1cm]{step4.pdf}\\
%  \vspace{-.4cm}\caption{Example of Step 4 when we view the instance $\cC_{\Item^*}, A_i^j$ as a $(d-1)$-{\sf UUDP-MIN} instance.}\label{fig:step4}\vspace{-.7cm}
%%\end{figure}
%\end{wrapfigure}

\begin{figure}
\begin{center}
\subfigure[]{
\includegraphics[height=0.12\textheight, clip=true, trim=1.5cm .3cm 1cm .3cm]{step3.pdf}
\label{fig:step4_1}
}
\subfigure[]{
\includegraphics[height=0.12\textheight, clip=true, trim=3cm .75cm 7cm 1cm]{step4.pdf}
\label{fig:step4}
}
\end{center}
\vspace{-.5cm}
\caption{\subref{fig:step4_1} Example of Step 4. \subref{fig:step4} Example of Step 4 when we view the instance $\cC_{\Item^*}, A_i^j$ as a $(d-1)$-{\sf UUDP-MIN} instance.}
\vspace{-.5cm}
\end{figure}

%
This lemma holds simply because $A_i$ is an antichain (in any antichain, no item can completely dominate the others, so at least one coordinate of any $\Item\in \cI_{\Item^*}$ has to be at least as good as $\Item^*$; see detailed proof in Appendix~\ref{proof:union of d dimensions}). Then $\{(\cC_{\Item^*}, A_i^1), \ldots, (\cC_{\Item^*}, A_i^d)\}$ is a consideration-preserving decomposition of $(\cC_{\Item^*}, A_i)$ and thus there exists $j$ such that
%\begin{align*}
$\opt(\cC_{\Item^*}, A_i^j) \geq \opt(\cset_{\Item^*}, A_i)/d = \tilde\Omega_d(\opt(\cC, \cI)/n^{3\epsilon/4}).$
%\end{align*}
%
%
Observe that, for all $\Consumer\in \cset_{\Item^*}$ and $\Item \in A_i^j$, $\Consumer[j]\leq \Item^*[j]\leq \Item[j]$. This implies that we can ignore the $j$-th coordinate when we solve $\pset(\cset_{\Item^*}, A_i^j)$. (In particular, for any $\Consumer\in\cC_{\Item^*}$, the consideration set $S_\Consumer=\left\{\Item\geq \Consumer\mid \Item\in A_i^j\right\}$ remains the same even when we drop the $j$-th coordinate of all points.) In other words, the problem can be viewed as a $(d-1)$-{\sf UUDP-MIN} problem (see Fig.~\ref{fig:step4} for an idea).
We defer the formal statement and proof of this claim to Section~\ref{sec:detail four}.
%
%
Finally, we can invoke the $\tilde O_d(n^{1-\epsilon})$-approximation algorithm for $(d-1)$-{\sf UUDP-MIN} to collect the revenue of
%
%\begin{align*}
%&\max\set{\opt(\cset_{\Item^*}, A_i^1), \ldots, \opt(\cset_{\Item^*}, A_i^d)}/n^{1-\epsilon}\\
$\tilde\Omega_d\left(\opt(\cset, \iset) n^{-3\epsilon/4}/n^{1-\epsilon}\right)$ $=\tilde\Omega_d\left(\opt(\cset, \iset)/n^{1-\epsilon/4}\right).$ Therefore we obtain an approximation ratio of $\tilde O_d(n^{1-\epsilon/4})$ in all cases. Algorithm~\ref{algo:udp} summaries our algorithm for solving $d$-{\sf UUDP-MIN}.


\begin{algorithm}
\caption{\footnotesize {\sf UUDP-MIN-APPROX}($d$)}\label{algo:udp}
\begin{algorithmic}[1]
\footnotesize
\IF{$d=1$}

\STATE Solve the problem $\cP(\cC, \cI)$ optimally using an algorithm for $1$-{\sf UUDP-MIN} (cf. Appendix~\ref{sec:one udp min})


\ELSE

\STATE Partition $\cI$ into antichains $A_1, \ldots, A_s$ and chains $B_1, \ldots, B_t$ where $s\leq n^{\epsilon/4}$ and $t\leq n^{1-\epsilon/4}$ as in Step 1.

\STATE We claim that the problems $\cP(\cC, B_1), \ldots, \cP(\cC, B_t)$ are equivalent to $1$-{\sf UUDP-MIN} problems (cf. Section~\ref{sec:detail one}). Solve them optimally using an algorithm for $1$-{\sf UUDP-MIN} (cf. Appendix~\ref{sec:one udp min}).
%Remember the solution with highest revenue.

\FOR{$i=1, \ldots, s$}


\STATE Partition $\cC$ into $\cC_1$ and $\cC_2$ as in Step 2. Find an $O(\max_{\Consumer \in \cset_1} \size{S_{\Consumer}\cap A_i})$=$O(n^{1-2\epsilon/4})$ approximate solution of problem $\cP(\cC_1, A_i)$.

%Remember the solution with hight

\STATE Find a hitting set $H$ of $(\cC_2, A_i)$ as in Step 3

\FOR{each $\Item\in H$}

\STATE Define $\cC_\Item$ as in Step 3

\STATE Define $A_i^1, \ldots, A_i^d$ as in Step 4 %(using $\Item^*=\Item$)

\STATE Solve problem $\cP(\cC_\Item, A_i^1), \ldots, \cP(\cC_\Item, A_i^d)$ using an $O(n^{1-\epsilon})$-approximation algorithm for $(d-1)$-{\sf UUDP-MIN}

\ENDFOR

\ENDFOR

\ENDIF

\RETURN the solution with highest revenue among the solutions of all solved problems

\end{algorithmic}
\end{algorithm}



%
%\subsection{Detail of Step 1}\label{sec:detail one}
%
%We give formal definitions needed for Step 1 here. Let $(\cset, \iset)$ be an input of $d$-{\sf UDP-MIN}. First we can define a partially ordered set $(\iset, \leq)$ on the set of items as follows. We say that $\Item_1 \leq \Item_2$ if and only if $\Item_1$ has a lower quality than $\Item_2$ in every attribute, i.e. $\Item_1[d'] \leq \Item_2[d']$ for all $d' \in [d]$.
%
%We say that a subset $\iset' \subseteq \iset$ is a chain if $\iset'$ can be written as $\iset'= \set{\Item_1,\ldots, \Item_z}$ such that $\Item_j \leq \Item_{j+1}$ for all $j: 1\leq j \leq z-1$. We say that $\iset' \subseteq \iset$ is an antichain if and only if for any pair $\Item, \Item' \in \iset'$, neither $\Item \leq \Item'$ nor $\Item' \leq \Item$ (i.e. they are incomparable).
%
%Given a partial order $P=(S,\leq)$, we can define the chain number of $P$ as ${\sf chain}(P)$ which denotes the minimum positive integer $w$ such that $S$ can be partitioned into disjoint sets $S_1,\ldots, S_w$ where each $S_j$ is a chain. We will use the following theorem, first proved by Dilworth \cite{Dilworth}, and its polynomial computability follows from the equivalence between Dilworth's theorem and Konig's theorem~\cite{Fulkerson-Dilworth}.
%
%\begin{theorem}
%Let $(S, \leq)$ be a partially ordered set, and $Z$ be the maximum number of elements in any antichain of $S$. Then there is a polynomial time algorithm that produces a partition of $S$ into $Z$ chains $S_1,\ldots, S_Z$.
%\end{theorem}
%
%We now use the theorem to prove Lemma~\ref{lemma: chain decomposition}.
%
%\begin{proof}[Proof of Lemma~\ref{lemma: chain decomposition}]
%In each iteration, we check if the size of maximum antichain in $\iset$ is at least $t=n^{1-\epsilon/4}$. If so, we find the maximum antichain and remove the items in it from $\iset$. This maximum antichain becomes a set $A_i$. Notice that there can be at most $s=n^{\epsilon/4}$ such antichains. Once the size of maximum-size antichain in $\iset$ is smaller than $t$, we apply the above theorem to compute a decomposition of $\iset$ into $B_1,\ldots, B_t$. This concludes the proof of Lemma~\ref{lemma: chain decomposition}.
%\end{proof}



%
%
%\subsection{Detail of Step 3}\label{sec:detail three}
%
%%\danupon{I think this section should be changed as follows. 1) We have to define the notion of $d$-dimensional box. 2) I don't think we have to define the notion of VC dimension but instead we should cite some theorem that says that $d$-dimensional box has $O(d)$ VC dimension. Or, if we really want to define it, the definition and the full proof that $d$-dimensional box has $O(d)$ VC dimension should be in Appendix~XXX (for completeness).}
%%Let $N$ be a set of ground elements, and $\xset= \{X_1,\ldots, X_m \}$ where $X_i \subseteq N$, be a collection of sets. We say that $\xset$ {\em shatters} a subset $N' \subseteq N$ if and only if $\size{\set{N' \cap X_i: X_i \in \xset}} = 2^{\size{N'}}$. The VC-dimension of set system $(N,\xset)$ is the size of maximum-size subset $N' \subseteq N$ that is shattered by $\xset$.
%
%As noted before, the instance $(\cC_2, A_i)$ to define a set system $\{S_\Consumer\}_{\Consumer\in \cC_2}$ over $A_i$, where $S_\Consumer=\{\Item\in A_i\mid \Item\geq \Consumer\}$. We note that each set $S_{\Consumer}$ has {\em descriptive complexity} at most $d$ (i.e. set $S_{\Consumer}$ can be described by $d$ linear inequalities\danupon{Could be better if we can write 2-3 sentences here}), this set system has VC-dimension $O(d)$ (see textbooks such as \cite{Sharir-book} for detail). \danupon{If this is all we will provide, we should write this as a proof.}
%
%%We will be working with the set system $(A_i, \set{S_{\Consumer}}_{\Consumer \in \cset_2})$. Since each set $S_{\Consumer}$ has descriptive complexity at most $d$ (i.e. set $S_{\Consumer}$ can be described by $d$ linear inequalities), this set system has VC-dimension at most $O(d)$ (see, e.g., \cite{Sharir-book}).
%
%\begin{theorem}[Epsilon net theorem]
%Let $(N, \xset)$ be a set system of VC-dimension at most $d'$. Then for any $\delta \in (0,1)$, we can, in randomized polynomial time, find a ``hitting set'' $H \subseteq N$ with $\size{H} = O(\frac{d'}{\delta}\log \frac{d'}{\delta})$ such that, for all $X_i \in \xset: \size{X_i} \geq \delta \size{N}$, we have $H \cap N \neq \emptyset$.
%\end{theorem}
%
%Using the theorem with $\delta = n^{-2\epsilon/4}$, we can find a hitting set $H \subseteq A_i$ of size at most $\tilde{O}(n^{2\epsilon/4})$, and since we have $|S_{\Consumer} \cap A_i| \geq \delta n$ for all $\Consumer \in \cset_2$, we are guaranteed that $H \cap S_{\Consumer} \neq \emptyset$ for all $\Consumer \in \cset_2$.


%\subsection{Detail of Step 4}\label{sec:detail four}




%\danupon{I redefine the definition}\danupon{I remember that we did this for the general version but it didn't work. I don't remember why though.}
%%
%To be able to formally talk about the reduction of dimensions, we introduce the following notion of {\em equivalence} and {\em consideration-preserving embedding}. For any positive integers $d$ and $d'$, let $(\cC, \cI)$ and $(\cC', \cI')$ be any instances of $d$-{\sf UDP-MIN} and $d'$-{\sf UDP-MIN},  respectively. We say that $(\cC, \cI)$ and $(\cC', \cI')$ are equivalent if there exist one-to-one mappings $f:\cC\rightarrow \cC'$ and $g:\cI\rightarrow\cI'$ such that consumer $\Consumer\in \cC$ considers item $\Item\in \cI$ (i.e., $\Item\geq \Consumer$) if and only if consumer $f(\Consumer)$ considers item $g(\Item)$ (i.e., $g(\Item)\geq {f(\Consumer)}$) and for any $\Consumer\in \cset$, $B_\Consumer=B_{f(\Consumer)}$. In other words, although  $(\cC, \cI)$ and $(\cC', \cI')$ correspond to points on different dimensions, they represent the same pricing problem (i.e., the consumers' consideration sets are exactly the same). We call the pair $(f, g)$ an consideration-preserving embedding.
%%
%The following lemma follows trivially.
%
%\begin{lemma}
%If $(\cC, \cI)$ and $(\cC', \cI')$ are equivalent then
%\[\opt(\pset(\cset, \iset)) = \opt(\pset(\cset', \iset')) \]
%Moreover, a solution for $\pset(\cset', \iset')$ can be transformed into one for $\pset(\cset, \iset)$ that gives the same revenue using the consideration-preserving embedding $(f, g)$.
%\end{lemma}
%
%The transformation in the above lemma is trivial: For any pricing function $p$ for $\pset(\cset', \iset')$, we simply price item $\Item\in \iset$ to $p(g(\Item))$. Observe that we will receive the same revenue from both problems using this pricing strategy.

%\subsubsection{Equivalences of Problems}

\subsection{Consideration-preserving Embedding}\label{sec:detail four}


To formally discuss the reduction of dimensions, we introduce the notion of consideration-preserving embedding. For any $d$, let $(\cC, \cI)$ be any instance of $d$-{\sf UUDP-MIN}. For any $d'$, consider one-to-one functions $f$ and $g$ that map points in $\R^d$ to the ones in $\R^{d'}$. We say that $(f, g)$ is a {\em consideration-preserving embedding} if, for any item $\Item \in \iset$ and consumer $\Consumer \in \cset$, we have that $\Item \geq \Consumer$ if and only if $g(\Item) \geq f(\Consumer)$. That is, the fact that consumer $\Consumer$ is considering or not considering item $\Item$ must be preserved in $f(\Consumer)$ and $g(\Item)$.

%\squishlist
%  \item Function $g: \iset' \rightarrow \iset^0$ is an injective map from $\iset'$ to items $\iset^0 \subseteq \R^{d'}$, and function $f: \cset' \rightarrow \cset^0$ is a mapping of consumers.
%
%  \item For any item $\Item \in \iset'$ and consumer $\Consumer \in \cset'$, we have that $\Item \geq \Consumer$ if and only if $g(\Item) \geq f(\Consumer)$.
%\squishend

Given a consideration-preserving embedding $(f,g)$, we can naturally define a $d'$-{\sf UUDP-MIN} problem $\pset(f(\cset), g(\iset))$ where $f(\cset)=\{f(\Consumer)\mid \Consumer\in \cset\}$, $g(\iset)=\{g(\Item)\mid \Item \in \iset\}$ \danupon{Should we say this? ``(note that we allow the sets to contain identical points)''} and the budget $B_{f(\Consumer)}$ is $B_\Consumer$ for any $\Consumer\in\cset$.
%




Observe that, although  $(\cC, \cI)$ and $(f(\cC), g(\cI))$ correspond to points on different spaces, they represent the same pricing problem (i.e., the consumers' consideration sets and budgets are exactly the same). Thus, we sometimes say that $(\cC, \cI)$ and $(f(\cC), g(\cI))$ are {\em equivalent}. The following observation follows trivially.



\begin{observation}
\label{observation: consideration preserving embedding}
For any instance $(\cset,\iset)$, let $(f,g)$ be a consideration-preserving embedding of $(\cset, \iset)$ into $\R^{d'}$. Then we have that
%\[
$\opt(\cset, \iset) = \opt(f(\cset), g(\iset)).$
%\]
Moreover, if $f$ and $g$ are polynomial-time computable then a solution for $\cP(f(\cset), g(\iset))$ can be efficiently transformed into one for $\cP(\cset, \iset)$  that gives the same revenue.
\end{observation}

The transformation in the above lemma is trivial: For any price function $p$ for $(f(\cset), g(\iset))$, we simply price item $\Item\in \iset$ to $p(g(\Item))$. Observe that we will receive the same revenue from both problems using this pricing strategy.

In Step 1, we claimed that when the items form a chain, our instance would be equivalent to $1$-{\sf UUDP-MIN}. Now we prove this fact formally below.


\begin{lemma}\label{lem:chain to one dim}
Let $(\cset, \iset)$ be a $d$-{\sf UUDP-MIN} instance where $(\iset, \leq)$ is a chain. Then $(\cC, \cI)$ is equivalent to a $1$-{\sf UUDP-MIN} instance. Moreover, the corresponding consideration-preserving embedding $(f, g)$ can be computed in polynomial time.
\end{lemma}
\begin{proof}
Order items in $\cI$ by $\Item_1\leq \Item_2\leq \ldots$. Now map each item into a one-dimensional point: $g(\Item_i)=(i)$. Moreover, map each consumer according to $f(\Consumer)=g(\Item_i)$, where $i$ is the minimum number such that $\Item_i\geq \Consumer$. Observe that $(f, g)$ is a consideration-preserving embedding since $S_\Consumer=\{\Item_i, \Item_{i+1}, \ldots\}$ while $S_{f(\Consumer)}=\{g(\Item_i), g(\Item_{i+1}), \ldots\}$ for any $\Consumer\in \cset$. (Note that this embedding might create redundancy since it is possible that $f(\Consumer)=f(\Consumer')$ for some $\Consumer\neq \Consumer'$. This can be fixed easily by slightly perturbing the points.\danupon{I'm not sure if this is necessary.})
\end{proof}

In Step 4, we also claimed the dimension reduction of sub-instances $(\cset_{\Item^*}, A_i^j)$, and we now prove the claim formally. Recall that the item $\Item^*\in A_i^j$ has the property that $\Item^*\geq \Consumer$ for all $\Consumer \in \cC_{\Item^*}$ and $\Item^*[j]\leq \Item[j]$ for all $\Item\in A_i^j$.

\begin{lemma}\label{lem:dim reduction}
The instance
$(\cC_{\Item^*}, A_i^j)$ is equivalent to a $(d-1)$-{\sf UUDP-MIN} instance. Moreover, the corresponding consideration-preserving embedding $(f, g)$ can be computed in polynomial time.
\end{lemma}
\begin{proof}
Consider ``ignoring'' the $j$-th coordinate as follows. For any $\Consumer\in \cC_{\Item^*}$ and $\Item\in A_i^j$, let $f(\Consumer)=(\Consumer[1], \Consumer[2], \ldots, \Consumer[j-1], \Consumer[j+1], \ldots, \Consumer[d])$
and
$g(\Item)=(\Item[1], \Item[2], \ldots, \Item[j-1], \Item[j+1], \ldots, \Item[d]).$
Observe that for any $\Consumer\in \cC_{\Item^*}$ and $\Item\in A_i^j$,  $\Item\geq \Consumer$ trivially implies that $g(\Item)\geq f(\Consumer)$. Conversely, if $g(\Item)\geq f(\Consumer)$ then $\Item\geq \Consumer$ since $\Item[j]\geq \Item^*[j]\geq \Consumer[j]$. Thus, $(f, g)$ is a consideration-preserving embedding.
\end{proof}

%In Step 4, we use this lemma with $\cC=\cC_{\Item^*}$ and $\cI=A_i$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Below is the old version
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\iffalse
%\section{Algorithm and Proof Idea for $d$-{\sf UDP-MIN}}\label{sec:d udp min}
%
%
%%We sketch an $\tilde O(n^{3/4})$-approximation algorithm for $2$-{\sf UDP-MIN} to illustrate the key ideas used in obtaining our main results. We note that this section is only for illustration and in fact better approximation factors for $2$-{\sf UDP-MIN} can be obtained -- this problem is $\tilde O(n^{1/2})$-approximable and even admits {\sf QPTAS}. Further details on larger $d$ will be shown in later sections.
%
%%We will use Fig.~XXX as an illustration.
%
%We are given sets of consumers $\cset$ and items $\iset$ as $d$-dimensional points where each consumer $\Consumer$ has budget $B_{\Consumer}$ and consideration set $S_{\Consumer}$, which is determined by the coordinates of input points. For any subsets $\cset' \subseteq \cset$ and $\iset' \subseteq \iset$, we denote by $\pset(\cset', \iset')$ the $d$-{\sf UDP-MIN} problem with $(\cset', \iset')$ as input. We use $\opt(\cset', \iset')$ to denote the optimal revenue that can be collected from $\pset(\cset', \iset')$. First it is easy to show that $1$-{\sf UDP-MIN} can be solved optimally in polynomial time (see Appendix~\ref{sec:one udp min}). Our algorithm proceeds in inductive manner, solving $d$-{\sf UDP-MIN} by invoking the algorithm for $(d-1)$-{\sf UDP-MIN} and $1$-{\sf UDP-MIN} as a sub-routine. The following theorem summarizes our main result.
%
%\begin{theorem}
%\label{thm: dimension reduction for UDP}
%For any $\epsilon \in [0,1)$, if there is a $\tilde O(n^{1-\epsilon})$-approximation algorithm for $(d-1)$-{\sf UDP-MIN} then there is a $\tilde O(n^{1-\epsilon/4})$-approximation algorithm for $d$-{\sf UDP-MIN} as well.
%\end{theorem}
%
%
%%For any sets $\cset$ and $\iset$ of consumers and items, let $\opt(\cset, \iset)$ be the optimal revenue of $1$-{\sf UDP-MIN} when $(\cset, \iset)$ is an input. Let $\cset$ and $\iset$ be the input sets and $\{S_\Consumer\}_{\Consumer\in \cset}$ be the corresponding consideration sets. C
%
%\begin{corollary}
%For any constant $d$, there is an approximation algorithm that gives a sub-linear approximation guarantee for $d$-{\sf UDP-MIN}.
%\end{corollary}
%
%
%Now we prove Theorem~\ref{thm: dimension reduction for UDP}. We first make the following simple observation. We say that a collection $\set{(\cset'_1,\iset'_1),\ldots, (\cset'_k, \iset'_k)}$ is a {\em decomposition} of the original problem if and only if for any $\Consumer \in \cset$ and $\Item \in S_{\Consumer}$, there exists (not necessarily unique) $i$ such that $\Consumer \in \cset_i$ and $\Item \in \iset_i$. In other words, the fact that consumer $\Consumer$ is interested in item $\Item$ must be ``realized'' in at least one sub-instance $(\cset_i, \iset_i)$. The following lemma allows us to decompose the problem into many sub-problems and focus on collecting revenue from the most profitable sub-problem.
%
%\begin{lemma}
%\label{lemma: UDP decomposition}
%For any decomposition $\{(\cset'_1,\iset'_1)$, $\ldots$, $(\cset'_k, \iset'_k)\}$ of $(\cset, \iset)$,
%\[\sum_{i=1}^k \opt(\cset'_i, \iset'_i)\geq \opt(\cset, \iset)
%,.\]
%Moreover, any price function for $\pset(\cset'_i, \iset'_i)$ can be extended to a price function for the original problem $\pset(\cset, \iset)$ that gives revenue $\opt(\cset'_i, \iset'_i)$
%\end{lemma}
%
%We only sketch the proof here and defer the full proof to Appendix~XXX: For the first claim, if $p^*$ is the optimal price function for $\pset(\cset, \iset)$, the combined revenue we get from restricting $p^*$ to each of the sub-problems $\pset(\cset_i, \iset_i)$ would be at least $\opt(\cset, \iset)$. For the second claim, if we are given a price function $p$ for $\pset(\cset_i, \iset_i)$, we can extend the function to $p': \iset \rightarrow \R$ by pricing items in $\iset\setminus\iset'_i$ to infinity. See Appendix~XXX for the full proof\danupon{To do: Add proof}.
%
%
%
%%The first claim in the lemma above can be shown simply by pricing $p^*$ on each problem $\pset(\cset'_i, \iset'_i)$ where $p^*$ is the optimal price function for $\pset(\cset, \iset)$. The second claim can be shown by pricing items in $\iset\setminus\iset'_i$ to infinity.
%
%%
%This notion of decomposition allows us to focus only on solving specific parts of the input and forget about other parts.
%
%
%%Our second observation is that $1$-{\sf UDP-MIN} can be solved optimally in polynomial time by a simple dynamic program. \\
%%
%%\begin{observation}
%%$1$-{\sf UDP-MIN} can be solved optimally in polynomial time by a simple dynamic program.
%%\end{observation}
%
%\danupon{This paragraph has to be changed.} Now our main goal is to find $\cset^*\subseteq \cset$ and $\iset^*\subseteq \iset$ such that $\opt(\cset^*, \iset^*)=\Omega(\opt/n^{3\epsilon/4})$, and the $d$-{\sf UDP-MIN} problem $\pset(\cset^*, \iset^*)$ is equivalent to a $(d-1)$-{\sf UDP-MIN} problem. Once we get this, we can invoke an $\tilde O(n^{1-\epsilon})$ for $(d-1)$-{\sf UDP-MIN} to get an approximation factor of $\tilde O(n^{1-\epsilon}\cdot n^{3\epsilon/4})=\tilde O(n^{1-\epsilon/4})$. Our algorithm proceeds in four steps, as follows.
%
%%Consider any $\cset'_1, \ldots, \cset'_k\subseteq \cset$ and $\iset'_1, \ldots, \iset'_k$ such that, for any $\Consumer$ and $\Item\in S_\Consumer$, there exists $i\leq k$ such that $\Consumer\in \cset'_i$ and $\Item\in \iset'$. Observe that $\sum_{i=1}^k \opt(\cset_i, \iset_i)\geq \opt(\cset, \iset)$. Moreover, we can achieve the revenue of $\opt(\cset_i, \iset_i)$ by pricing all $\iset\setminus \iset_i$ to infinity and all items in $\iset$ to the price we use to achieve $\opt(\cset_i, \iset_i)$ when the input consists of $\cset_i$ and $\iset_i$.
%
%%Secondly, we note that $1$-{\sf UDP-MIN} can be solved optimally by a simple dynamic program.
%
%%Our main goal is to find $\cset'\subseteq \cset$ and $\iset'\subseteq \iset$ such that $\opt(\cset', \iset')=\Omega(\opt(\cset, \iset)/n^{3/4})$ and the $2$-{\sf UDP-MIN} problem on input $(\cset', \iset')$ can be solved optimally by reducing to a $1$-{\sf UDP-MIN} problem. We do this in several steps as follows.
%
%\paragraph{Step 1: Partitioning items into chains and antichains.} We view items as a partially ordered set where we write $\Item_1\leq \Item_2$ if and only if $\Item_1[d']\leq \Item_2[d']$ for all $d'\in [d]$.\danupon{QUESTION: Can we partition POSET into ``2-dimensional'' chains and anti-chains? That is, instead of a chain, we want a poset of dimension at most two (``2-dimensional chain'') and, instead of an anti-chain, we want a set of elements that intersect all 2-dimensional chains.}
%
%%First, we use Dilworth's theorem to decompose items into $O(\sqrt{n})$ chains and antichains.
%%(We refer the readers to Section~\ref{thm: dimension reduction} for more details.)
%%(We refer the reader to graph theory textbook for details of Dil.)
%%
%%\begin{lemma}
%%In polynomial time, we can partition $\iset$ into $A_1, \ldots, A_s$ and $B_1, \ldots, B_t$ such that $s \leq n^{1/4}$, $t\leq n^{3/4}$ and, for all $i$, $A_i$ and $B_i$ are an antichain and a chain, respectively.
%%\end{lemma}
%
%
%\begin{lemma}
%\label{lemma: chain decomposition}
%In polynomial time, we can partition $\iset$ into $A_1, \ldots, A_s$ and $B_1, \ldots, B_t$ such that $s \leq n^{\epsilon/4}$ and $t\leq n^{1-\epsilon/4}$. Moreover, each $A_i$ is an antichain, and each $B_i$ is a chain.
%\end{lemma}
%
%The proof of this lemma is a simple application of Dilworth's theorem \cite{Dilworth,Fulkerson-Dilworth} which states that the minimum chain decomposition equals to the maximum antichain size and the fact that these two objects can be computed in polynomial time: As long as the minimum antichain is bigger than $n^{\epsilon/4}$, we repeatedly extract such an anti-chain out of the input; otherwise, we would have the decomposition into at most $n^{\epsilon/4}$ chains, so we stop. We refer to Section~XXX for more detail.
%
%
%
%It then follows, from Lemma~\ref{lemma: UDP decomposition}, that
%$$\sum_{i=1}^s\opt(\cset, A_i)+\sum_{j=1}^t \opt(\cset, B_i) \geq \opt(\cset, \iset)$$
%because the collection $\{(\cset, A_1)$, $\ldots$, $(\cset, A_s)$, $(\cset, B_1)$, $\ldots$, $(\cset, B_t)\}$ is a decomposition of $(\cset, \iset)$. Further, observe that if there exists $j$ such that $\opt(\cset, B_j)\geq\opt(\cset, \iset)/2n^{1-\epsilon/4}$, then we would be done: the $d$-{\sf UDP-MIN} problem $\pset(\cset, B_j)$ can be seen as a $1$-{\sf UDP-MIN} problem (since $B_j$ is a chain) and hence can be solved optimally! (NEED DETAIL) If this is not the case then we know that there must be an antichain $A_i$ such that $\opt(\cset, A_i)\geq \opt(\cset,\iset)/2n^{\epsilon/4}$. We now proceed to the next step.
%
%%Our goal now is to $O(n^{1/2})$-approximate the problem on such $A_i$.
%
%
%
%
%\paragraph{Step 2: Dealing with small consideration sets.} For simplicity, let us assume that we know $i$ such that $\opt(\cset, A_i)\geq \opt(\cset, \iset)/2n^{\epsilon/4}$. Now we can just focus on collecting revenue from the subproblem $\pset(\cset, A_i)$. Let $\cset_1$ be the set of consumers who are interested in at most $n^{1-2\epsilon/4}$ items in $A_i$, i.e. $\cset_1=\{\Consumer\in \cset: |S_\Consumer\cap A_{i}|\leq n^{1-2\epsilon/4}\}$, and define $\cset_2=\cset\setminus \cset_1$. Observe that $\opt(\cset_1, A_i)+\opt(\cset_2, A_i)\geq \opt(\cset, A_i)\geq \opt(\cset, \iset)/2n^{\epsilon/4}$ because $\{(\cset_1, A_i), (\cset_2, A_i)\}$ is a decomposition of $(\cset, A_i)$.
%
%Now we need an algorithm of \cite{BalcanB07,BriestK06} which bounds an approximation ratio in terms of $k = \max_{\Consumer \in \cset} \size{S_{\Consumer}}$, as stated in the following theorem.
%
%\begin{theorem}
%Let $k = \max_{\Consumer \in \cset} \size{S_{\Consumer}}$. Then there is an $O(k)$-approximation algorithm for {\sf UDP-MIN}.
%\end{theorem}
%
%We note that in fact the algorithm in~\cite{BalcanB07} is for {\sf SMP}, but it is easy to see that their algorithm gives the same guarantee for {\sf UDP-MIN}. For completeness, we provide the proof in Appendix.
%
%Using the theorem, if $\opt(\cset_1, A_i)\geq \opt(\cset, \iset)/4n^{\epsilon/4}$, then we could invoke the algorithm, yielding a solution that gives revenue of $\Omega(\opt(\cset_1, A_i)/n^{1-2\epsilon/4})=\Omega(\opt(\cset, \iset)/n^{1-\epsilon/4})$ as desired. Otherwise, it must be the case that $\opt(\cset_2, A_i)=\Omega(\opt(\cset, \iset)/n^{\epsilon/4}).$ We will deal with this case in the next steps.
%
%%... Note that $|A_i|$ could be as large as $\Omega(n)$....
%
%\paragraph{Step 3: Finding a small hitting set via epsilon net.} Let $N$ be a set of ground elements, and $\xset= \{X_1,\ldots, X_m \}$ where $X_i \subseteq N$, be a collection of sets. We say that $\xset$ {\em shatters} a subset $N' \subseteq N$ if and only if $\size{\set{N' \cap X_i: X_i \in \xset}} = 2^{\size{N'}}$. The VC-dimension of set system $(N,\xset)$ is the size of maximum-size subset $N' \subseteq N$ that is shattered by $\xset$.
%
%We will be working with the set system $(A_i, \set{S_{\Consumer}}_{\Consumer \in \cset_2})$. Notice that each set $S_{\Consumer}$ can be viewed as a $d$-dimensional box, so the VC-dimension of such set system is at most $O(d)$. We will need the following theorem.
%
%\begin{theorem}[Epsilon net theorem]
%Let $(N, \xset)$ be a set system of VC-dimension at most $d'$. Then for any $\delta \in (0,1)$, we can, in randomized polynomial time, find a ``hitting set'' $H \subseteq N$ with $\size{H} = O(\frac{d'}{\delta}\log \frac{d'}{\delta})$ such that, for all $X_i \in \xset: \size{X_i} \geq \delta \size{N}$, we have $H \cap N \neq \emptyset$.
%\end{theorem}
%
%Using the theorem with $\delta = n^{-2\epsilon/4}$, we can find a hitting set $H \subseteq A_i$ of size at most $\tilde{O}(n^{2\epsilon/4})$, and since we have $|S_{\Consumer} \cap A_i| \geq \delta n$ for all $\Consumer \in \cset_2$, we are guaranteed that $H \cap S_{\Consumer} \neq \emptyset$ for all $\Consumer \in \cset_2$.
%
%%We claim that we can find a hitting set $H\subseteq A_i$ of size $\tilde O(n^{2\epsilon})$, i.e., $S_\Consumer\cap H\neq \emptyset$ for all $\Consumer\in \cset_2$. This follows from the epsilon net theorem~\cite{Chazelle-book,Epsilon-net} which roughly states that, for any $\delta>0$, if the set system has low VC dimension and all sets have size at least $n^\delta$ then there is a hitting set of size $\tilde O(n^{1-\delta})$; here, we use $\delta=1-2\epsilon$, and our sets $S_\Consumer$ have $O(1)$ VC dimension because they can be seen as $d$-dimensional boxes.
%
%
%\paragraph{Step 4: Reducing the dimension.} We have now reached the most crucial step. We will use the hitting set to decompose the problem into a few $(d-1)$-{\sf UDP-MIN} problems. For each $\Item\in H$, let $\cset_\Item=\{\Consumer\in \cset_2\mid \Item \in S_\Consumer\}$, i.e., $\cset_\Item$ is the set of all consumers in $\cset_2$ that considers item $\Item$. Observe that
%%
%\[\sum_{\Item \in H} \opt(\cset_\Item, A_i)\geq \opt(\cset_2, A_i) \geq \Omega(\opt(\cset, \iset)/n^{1/4^{d-d'}}).\]
%%
%This is because $\{(\cset_\Item, A_i)\}_{\Item\in H}$ is a decomposition of $(\cset_2, A_i)$. Since $\size{H}=\tilde O(n^{2\epsilon/4})$, there exists $\Item^*\in H$ such that $\opt(\cset_{\Item^*}, A_i) =\tilde\Omega(\opt n^{-\epsilon/4}/|H|)=\tilde\Omega(\opt/n^{3\epsilon/4})$. Now we, again, turn our focus to the subproblem $\pset(\cset_{\Item^*}, A_i)$. For notational convenience, we abbreviate $\cset_{\Item^*}$ by $\tilde{\cset}$ and $A_i$ by $\tilde{\iset}$. We will (crucially) rely on the fact that all consumers in $\tilde{\cset}$ consider item $\Item^*$, and that $\tilde{\iset}$ is an antichain.
%
%%We now decompose the problem on $C_{\Item^*}$ and $A_i$ into two problems that are equivalent to {\sf $1$-UDP-MIN}.
%%
%
%For each $j \leq d$, we define $\tilde{\iset}_j$ as the set of items that are at least as good as $\Item^*$ in the $j^{th}$ coordinate. That is, let $\tilde{\iset}_j=\{\Item\in \tilde{\iset} \mid \Item[j]\geq \Item^*[j]\}$.
%
%%
%%That is, for $j=1, 2$, let $\cset_{\Item^*}^j=\{\Consumer\in \cset_{\Item^*} \mid \Consumer[j]\leq \Item^*[j]\}$ and $A_i^j=\{\Item\in A_i \mid \Item[j]\geq \Item^*[j]\}$.
%%
%Observe that
%$$\tilde{\iset} = \bigcup_{j=1}^d \tilde{\iset}_j$$
%since $\tilde{\iset}$ is an antichain (in any antichain, no item can completely dominate others, so at least one coordinate of $\Item$ has to be at least as good as $\Item^*$.) Then we have
%$$\sum_{j=1}^d \opt(\tilde{\cset}, \tilde{\iset}_j) \geq \opt(\tilde{\cset}, \tilde{\iset}) = \tilde\Omega(\opt/n^{1-\epsilon/4})\,.$$
%
%%For $j=1, 2$, let $\cset_{\Item^*}^j=\{\Consumer\in \cset_{\Item^*} \mid \Consumer[j]\leq \Item^*[j]\}$ and $A_i^j=\{\Item\in A_i \mid \Item[j]\geq \Item^*[j]\}$.
%%
%%In other words, we guarantee that all consumers in $\cset_{\Item^*}^j$ are satisfied by all items in $A_i^j$ in the $j$th attribute.
%%
%%Consider the problem induced from $\cset_{\Item^*}^j$ and $A_i^j$ where we set price of all items outside $A_i^j$ to infinity and want to maximize the revenue we collect from $\cset_{\Item^*}^j$ and let $\opt^j$ be the corresponding optimal solution. Observe that $\opt^1+\opt^2\geq \opt'''_{\Item^*} =\tilde\Omega(\opt/n^{3/4})$.
%%
%%Observe that $\opt(\cset_{\Item^*}^1, A_i^1)+\opt(\cset_{\Item^*}^2, A_i^1)\geq \opt(\cset_{\Item^*}, A_i) =\tilde\Omega(\opt(\cset, \iset)/n^{3/4})$. (This is because $A_i$ is an antichain.)
%
%
%For any $j\leq d$, since for all $\Consumer\in \tilde\cset$ and $\Item \in \tilde\iset_j$, $\Consumer[j]\leq \Item^*[j]\leq \Item[j]$, we can ignore the $j^{th}$ coordinate when we solve the $d$-{\sf UDP-MIN} problem $\pset(\tilde\cset,\tilde\iset_j)$. In other words, the problem can be viewed as a $(d-1)$-{\sf UDP-MIN} problem. Thus, we can invoke the $\tilde O(n^{1-\epsilon})$-approximation algorithm for $(d-1)$-{\sf UDP-MIN} to collect the revenue of
%
%\begin{align*}
%&\max\set{\opt(\tilde\cset, \tilde\iset_1), \ldots, \opt(\tilde\cset, \tilde\iset_d)}/n^{1-\epsilon}\\
%&=\tilde\Omega_d(\opt n^{-3\epsilon/4}/n^{1-\epsilon})\\
%&=\tilde\Omega_d(\opt/n^{1-\epsilon/4})\,.
%\end{align*}
%
%\fi 

==> arxiv 7.24.2012/proof_algo_ec.tex <==
\section{Proof Omitted from Section~\ref{sec:d udp min}}


\subsection{Proof of Lemma~\ref{lemma: UDP decomposition}}
\label{sec: proof of UDP decomposition lemma}

Let $p^*$ be the optimal price function for $\pset(\cset, \iset)$. For each $i=1,\ldots, k$, we define $p^*_i: \iset'_i \rightarrow \R$ by
$$p^*_i(\Item) = p^*(\Item)~~\mbox{if $\Item \in \iset'_i$, and $p^*_i(\Item) = \infty$ otherwise.}$$
Let $r_i$ be the total revenue made by $p^*_i$ in $\pset(\cset'_i, \iset'_i)$. We argue below that
\begin{align}\label{eq:one}
\sum_{i=1}^k r_i \geq \opt(\cset, \iset).
\end{align}
Let $\cset^* \subseteq \cset$ be the set of consumers who make a positive payment with respect to $p^*$. For each consumer $\Consumer \in \cset^*$, denote by $\phi(\Consumer) \in \iset$ the item that consumer $\Consumer$ buys with respect to the price $p^*$.
%(For a technical reason, we also define $\perp$ to be a special symbol such that $\phi(\Consumer)=\perp$ if consumer $\Consumer$ buys nothing and $p^*(\perp)=0$.)
So we can write $\opt(\cset, \iset)$ as
\begin{align}\label{eq:two}
\opt(\cset, \iset) = \sum_{\Consumer \in \cset^*} p^*(\phi(\Consumer)).
\end{align}
For each $i=1,\ldots, k$, let $\cset^*_i \subseteq \cset'_i$ be the set of consumers $\Consumer \in \cset'_i$ such that $\phi(\Consumer) \in \iset'_i$. That is, $\cset^*_i$ is a set of consumers whose item she bought in $\opt(\cset, \iset)$ is in $\iset'_i$.
%
Notice that
\begin{align}\label{eq:three}
r_i \geq \sum_{\Consumer \in \cset^*_i} p^*(\phi(\Consumer)).
\end{align}
%
Since $\set{(\cset'_i, \iset'_i)}_{i=1}^k$ is a consideration-preserving decomposition, we have that
\begin{align}\label{eq:four}
\bigcup_{i=1}^k \cset^*_i \supseteq \cset^*,
\end{align}
%
since for any $\Consumer \in \cset^*$, we must have $\phi(\Consumer)\in \iset_i$ for some $i$. By summing Eq.\eqref{eq:three} over all $i=1,\ldots, k$, we have
%
\begin{align*}
\sum_{i=1}^k r_i &\geq \sum_{i=1}^k \sum_{\Consumer\in \cset^*_i} p^*(\phi(\Consumer)) &\mbox{(by Eq.\eqref{eq:three})}\\
&\geq \sum_{\Consumer\in \cset^*} p^*(\phi(\Consumer)) &\mbox{(by Eq.\eqref{eq:four})}\\
&=\opt(\cset, \iset)&\mbox{(by Eq.\eqref{eq:two})}
\end{align*}
%
%$\sum_{i=1}^k r_i \geq \opt(\cset, \iset)$.
%
This proves Eq.\eqref{eq:one} and thus the first claim.

Now suppose we have a price $p': \iset_i \rightarrow \R$ that collects revenue $r'$ in $\pset(\cset'_i, \iset'_i)$. We define a function $p: \iset \rightarrow \R$ by $p(\Item) = p'(\Item)$ for $\Item \in \iset'_i$ and $p(\Item) = \infty$ otherwise. We can use $p'$ to obtain a revenue of $r'$ from $\cP(\cset, \iset)$. This proves the second claim.


%\subsection{Detail of Step 1}
\subsection{Decomposing items into small number of chains and antichains}\label{sec:detail one}

%Given a partial order $P=(S,\leq)$, we can define the chain number of $P$ as ${\sf chain}(P)$ which denotes the minimum positive integer $w$ such that $S$ can be partitioned into disjoint sets $S_1,\ldots, S_w$ where each $S_j$ is a chain.
We will use the following theorem, first proved by Dilworth \cite{Dilworth}, and its polynomial computability follows from the equivalence between Dilworth's theorem and K\"onig's theorem~\cite{Fulkerson-Dilworth}.

\begin{theorem}\label{theorem:dilworth}
Let $(S, \leq)$ be a partially ordered set, and $Z$ be the maximum number of elements in any antichain of $S$. Then there is a polynomial-time algorithm that produces a partition of $S$ into $Z$ chains $S_1,\ldots, S_Z$.
\end{theorem}

We now use the theorem to prove Lemma~\ref{lemma: chain decomposition}.

\begin{proof}[of Lemma~\ref{lemma: chain decomposition}]
Initially, let $i=1$. In iteration $i$, we check if the size of maximum antichain in $\iset$ is at least $t=n^{1-\epsilon/4}$. If so, we find the maximum antichain $A_i$, update $\iset = \iset \setminus A_i$, and proceed to the next iteration; otherwise, we stop the iterations. Notice that the number of iterations is at most $s = n^{\epsilon/4}$, and when the iteration stops, the size of maximum-size antichain is at most $t\leq n^{1-\epsilon/4}$. We apply the above theorem to compute a decomposition of $\iset$ into $t$ chains, denoted by $B_1,\ldots, B_t$. This concludes the proof of Lemma~\ref{lemma: chain decomposition}.
\end{proof}


\subsection{Proof of Balcan-Blum Theorem for {\sf UUDP-MIN} (cf. Theorem~\ref{theorem:BalcanBlum})}\label{sec:balcanblum for udp min}

%\danupon{To do: If $k=O(\log m)$ if we can use Balcan-Blum and derandomized (running time will be $2^O(k)$). Case 2: If $k=\Omega(\log m)$ then we will use Guruswami to get $O(\log m)=O(k)$}
%
We first explain a randomized algorithm, and then we discuss how to derandomize it. This part is essentially the same as \cite{BalcanB07,BriestK11}. First, we randomly construct a set $\iset^* \subseteq \iset'$ where each item ${\bf I}$ is independently added to $\iset^*$ with probability $1/k$ (recall that $k=\max_{\Consumer\in \cset} |S_\Consumer|$). Then let $\cset^*$ be a set of consumer $\Consumer$ such that $\size{S_\Consumer\cap \iset^*}=1$ %$\size{\iset^*_{\succeq \Consumer}}=1$
(i.e. consumers who care about exactly one item in $\iset^*$). We show that the problem $\cP(\cset^*, \iset^*)$ has expected revenue at least $\Omega(\opt(\cset, \iset)/k)$.

Let $p$ be the optimal price function for $(\cset, \iset)$ and $\phi: \cset \rightarrow \iset\cup \{\perp\}$ be a function that maps each consumer to the item she buys with respect to $p$ (let $\phi(\Consumer)=\perp$ if consumer $\Consumer$ buys nothing and $p(\perp)=0$). Therefore, we have that $\opt(\cset, \iset) = \sum_{\Consumer} p(\phi(\Consumer))$. We denote by $p^*$ the price function $p$ restricted to $\iset^*$. For each $\Consumer$, if $\Consumer \in \cset^*$ and $\phi(\Consumer) \in \iset^*$, the revenue created by $p^*$ in $(\cset^*, \iset^*)$ would be at least $p(\phi(\Consumer))$. Therefore,
$$\expect{}{\opt(\cset^*, \iset^*)} \geq \sum_{\Consumer \in \cset} \Pr[\mbox{$\phi(\Consumer)\in \iset^*$ and $\Consumer\in \cset^*$}] \times p(\phi(\Consumer))\,.$$
%
Notice that, for any $\Consumer\in\cset$ and $\Item\in S_{\Consumer }$,
\[\Pr[\mbox{$\Item\in \iset^*$ and $\Consumer\in \cset^*$}] \geq \frac{1}{k}\left(1-\frac{1}{k}\right)^{k-1}\geq \frac{1}{k\mathrm{e}},\]
which implies that $\expect{}{\opt(\cset^*, \iset^*)} \geq \frac{1}{k \mathrm{e}}\cdot \opt(\cset, \iset)$.


{\bf Derandomization:} First, note that we can assume that $k=O(\log m+\log n)$. Otherwise, we can use the result of \cite{AggarwalFMZ04,GuruswamiHKKKM05,BalcanBM08} (see \cite[Section 4]{BalcanBM08} for the result in a general setting) to obtain $O(\log m+ \log n)$ approximation algorithm for {\sf UUDP-MIN}, which will also be $O(k)$-approximation.

Now, assuming that $k=O(\log m+\log n)$, we follow the argument of Balcan and Blum~\cite{BalcanB07}. In particular, we observe that we need only $k$-wise independence among the events of the form ``$\Item\in \iset^*$ and $\Consumer\in \cset^*$'', for any $\Item$ and $\Consumer$,  in order to get the above expectation result. In this case, we can use the tools from Even et al \cite{EvenGLNV98} to derandomize the above algorithm while blowing up the running time by a factor of $2^{O(k)}=\poly(m, n)$. For more details, we refer the readers to \cite{BalcanB07}.



%\subsection{Proof of Lemma~\ref{lemma: chain decomposition}}
%
%
%We will use the following theorem, first proved by Dilworth \cite{Dilworth}, and its polynomial computability follows from the equivalence between Dilworth's theorem and K\"onig's theorem \cite{Fulkerson-Dilworth}. We say that $X$ is an anti-chain of $S$ if $X\subseteq S$ and $X$ is an antichain.
%
%\begin{theorem}(\cite{Dilworth, Fulkerson-Dilworth})
%Let $z$ be the maximum number of elements in any antichain of $S$. Then there is a polynomial time algorithm that partitions $S$ into $z$ chains (i.e., it outputs a collection of $z$ chains $S_1, \ldots, S_z$ of $S$ where $S=\bigcup_{i=1}^z S_i$).
%\end{theorem}
%
%Now we prove the lemma. We repeatedly extract maximum antichain out of $S$ (i.e., we delete all elements of the maximum antichain) until the size of maximum antichain is at most $\size{S}^\delta$. This process gives at most $\size{S}^{1-\delta}$ antichains. Then, since the collection of the remaining elements in $S$ has maximum antichain of size at most $\size{S}^\delta$, it can be decomposed into $\size{S}^{\delta}$ chains (by Dilworth's theorem).


\subsection{Proof of Lemma \ref{lem:union of d dimensions}}\label{proof:union of d dimensions}
%First, we prove Lemma~\ref{lem:union of d dimensions}.
Recall that each $A_i$ is an antichain, i.e., for any distinct $\Item_1, \Item_2\in A_i$, there exists $1\leq d_1, d_2\leq d$ such that $\Item_1[d_1]<\Item_2[d_1]$ and $\Item_1[d_2]>\Item_2[d_2]$. In particular, if $\Item_1=\Item^*$, then we have that for any $\Item\in A_i$, there exists coordinate $j$ such that $\Item[j]\geq \Item^*$. This means that $\Item\in A_i^j$. The lemma follows.


\subsection{Polynomial-Time Algorithm for $1$-{\sf UUDP-MIN}}\label{sec:one udp min}

We provide a polynomial-time algorithm for solving $1$-{\sf UUDP-MIN}. Let $\Item_1,\ldots, \Item_n$ be a sequence of items ordered non-increasingly by their coordinates. We can assume without loss of generality that their coordinates are different (by slightly perturbing their values), and we say that consumer $\Consumer$ is at {\em level $j$} if her coordinate lies between $\Item_{j-1}$ and $\Item_j$. Notice that, for any consumer $\Consumer$ at level $j$, we have $S_{\Consumer} = \set{\Item_1,\ldots, \Item_j}$.

\begin{claim}
Let $p^*$ be an optimal price. Then we can assume that $p^*(\Item_1) \geq p^*(\Item_2) \geq \ldots \geq p^*(\Item_n)$.
\end{claim}
\begin{proof}
Suppose that $p^*(\Item_i) < p^*(\Item_j)$ for some $i <j$. Recall that $\Item_i \geq \Item_j$, so for each consumer $\Consumer$ such that $\Consumer \leq \Item_j$, we know that $\Consumer$ does not buy item $\Item_j$ with respect to this solution. Thus, we can reduce $p^*(\Item_i)$ slightly, while maintaining the same revenue.
\end{proof}

The claim will ensure that consumers at level $j$ only buy item $\Item_j$ but not any other items in $\set{\Item_1,\ldots, \Item_{j-1}}$, and this allows us to solve the problem by dynamic programming. For each $j=1,\ldots, n$, for each price $P \in \R$ we have a table entry $T[j,P]$ that keeps the maximum revenue achievable from consumers at levels $1,\ldots, j$ and items $\set{\Item_1,\ldots, \Item_j}$ where the price of $\Item_j$ is set to $P$. Notice that it is easy to compute the profit from consumers at level $j$ if we know $p(\Item_j) = P$. Denote such value by $\gamma$. Then we have that $T[j,P] = \gamma + \max_{P' \geq P} T[j-1,P']$. Finally, we note that there are at most $|\cset|$ possibilities of prices $P$ because one can assume without loss of generality that, for {\sf UUDP-MIN}, the prices always belong to $\set{B_{\Consumer}}_{\Consumer \in \cset}$.



==> arxiv 7.24.2012/single-minded-3.tex <==
\section{{\sf QPTAS} for $2$-{\sf SMP}}\label{sec:2-SMP}

In this section, we show that {\sf QPTAS} for $2$-{\sf SMP}. %Recall that, by Lemma~\ref{lemma:discretization}, 
%Note that, similar to Lemma~\ref{lem:uudp-discretize}, we may assume that optimal prices only assign prices in $\Gamma$ where $\size{\Gamma} = O(\log m)$.


\subsection{Overview}

\danupon{This problem is harder than the highway pricing problem since it doesn't have a separator. For example, the log n approx of Balcan-Bum for Highway heavily relies on the separator. Similarly, Khaled's QPTAS also relies on the separator (once you remember the profile in the middle, you can solve two sides separately).}

We sketch the key ideas here and leave the details in next sections. First, consider the special case where each consumer has
budget $1$ or $2$ and each item must be priced either $0$ or $1$.
The exact optimal solution of this case can be found in
$n^{O(\log^2 m n)}$ time. We later
show how to extend the idea to the general cases, which turns out to
be easy for the case of highway problem but need a few more ideas
for the case of $2$-{\sf SMP}.

\paragraph{Algorithm for highway pricing problem reviewed:}
Let us first start with the highway pricing problem which can be
casted as a special case of $2$-{\sf SMP} where items are in the
form $(1,n), (2,n-1), \ldots, (n,1)$.
The main idea used in \cite{ElbassioniSZ07}, casted in our language
of ``partition tree'' (for convenience in explaining our $2$-{\sf SMP} algorithm later) is the following.\danupon{I removed [htb!] from the figure.}


\begin{figure}%[htb!]
\centering \scalebox{1.2}[1.2]{\includegraphics{pic1}}
\caption{A partition tree}\label{fig:Partition_Tree}
\end{figure}


%
%\begin{figure}
%\psfrag{A}{$V_r$}
%
%\psfrag{B}{$V_u$}
%
%\psfrag{C}{$V_v$}
%
%\psfrag{r}{$r$}
%
%\psfrag{u}{$u$}
%
%\psfrag{v}{$v$}
%
%%\begin{wrapfigure}{r}{.3\textwidth}
%%\vspace{-5mm}
%  \centering
%      \epsfig{file=tree-highway.eps,width=0.4\textwidth}
%  \caption{A partition tree}\label{fig:Partition_Tree} \vspace{-5mm}
%%\end{wrapfigure}
%\end{figure}


We first construct a balanced binary tree called a {\em partition tree} and denoted by
${\cal T}$. We define the vertical gridline in the middle to be a level-$0$ line, denoted by $\ell_r$, dividing the items equally to left and right sides. This line corresponds to the root node $r$ of the tree. We also assign the consumers whose consideration set contains items on both sides to the root node. Then we recursively define the subtrees on the subproblems on the two sides of line $\ell_r$ as shown in Figure~\ref{fig:Partition_Tree} until we reach the subproblem containing only one item. For any node $v \in \tset$, let $\cset_v$ be the set of consumers assigned to $v$, and $\ell_v$ be the line associated with node $v$.

%We first construct a balanced binary tree called a {\em partition
%tree} and denoted by ${\cal T}$. This is done by drawing a vertical
%line through the middle item (i.e., the item at $(\lceil |{\cal
%I}|/2 \rceil, \lceil |{\cal I}|/2 \rceil)$). This item is assigned
%to the root node of the tree. Moreover, we assign all consumers
%whose consideration sets contain this item to the root node and
%delete them from the problem. We then recursively define the
%subtrees on the items on two sides of the vertical line as shown in
%Figure~\ref{fig:Partition_Tree}. For any node $v\in {\cal T}$, let
%$\Item_v$ and ${\cal C}_v$ be the item and the set of consumers
%assigned to $v$, respectively.



Now we show a top-down recursive algorithm to solve this problem.
This algorithm can be converted to a dynamic program by working
bottom-up instead. At the root node $r$ of ${\cal T}$, we would like
to compute $f_r(\Item_{L, 1}, \Item_{L, 2}, \Item_{L, 3}, \Item_{R,
1}, \Item_{R, 2}, \Item_{R, 3})$ which is defined to be the optimal
revenue that we can collect from consumers in ${\cal C}\setminus
{\cal C}_r$ when we price the items in such a way that $\Item_{L,
1}$, $\Item_{L, 2}$ and $\Item_{L, 3}$ ($\Item_{R, 1}$, $\Item_{R,
2}$ and $\Item_{R, 3}$, respectively) are the first, second, and
third closest items on the left (respectively, right) of $\ell_r$
that have price $1$. To avoid long notation, let us denote
$\{\Item_{L, 1}, \Item_{L, 2}, \Item_{L, 3}, \Item_{R, 1}, \Item_{R,
2}, \Item_{R, 3}\}$ by $\Gamma_r$ and $f_r(\Item_{L, 1}, \Item_{L,
2}, \Item_{L, 3}, \Item_{R, 1}, \Item_{R, 2}, \Item_{R, 3})$ by
$f_r(\Gamma_r)$.
%
%
%define a {\em
%guess of $r$}, denoted by $\Gamma_r$, to be any set of items
%$\{\Item_{L, 1}, \Item_{L, 2}, \Item_{L, 3}, \Item_{R, 1}, \Item_{R,
%2}, \Item_{R, 3}\}$ such that $\Item_{L, 3}[1]\leq \Item_{L,
%2}[1]\leq \Item_{L, 1}[1] \leq \Item_r[1] \leq \Item_{R, 1}[1] \leq
%\Item_{R, 2}[1]\leq \Item_{R, 3}[1]$. We then denote $f_r(\Item_{L,
%1}, \Item_{L, 2}, \Item_{L, 3}, \Item_{R, 1}, \Item_{R, 2},
%\Item_{R, 3})$ by $f_r(\Gamma_r)$.
%
If we can compute $f_r(\Gamma_r)$ for all $\Gamma_r$ then the
optimal revenue can be obtained via the following formula.
%
\begin{align}
\text{Optimal revenue} &=
\max_{\Gamma_r} f_r(\Gamma_r) + m_1(\Gamma_r) + 2m_2(\Gamma_r)\label{eq:highway}
\end{align}
%
where, for any node $v$, $m_1(\Gamma_v)$ is the number of consumers
in ${\cal C}_v$ whose consideration sets contain exactly one item in
$\Gamma_v$, and $m_2(\Gamma_v)$ is the number of consumers in ${\cal
C}_v$ with budget $2$ whose consideration sets contain exactly two
items in $\Gamma_v$. The point is that we can calculate the revenue
from consumers in ${\cal C}_r$ as $m_1(\Gamma_r) + 2m_2(\Gamma_r)$
and use $f_r(\Gamma_r)$ to compute the revenue obtained from the
rest of the consumers.

It is left to compute $f_r(\Gamma_r)$. Let $u$ and $v$ be the left
and right children of $r$, respectively. In order to compute
$f_r(\Gamma_r)$, we will compute $f_u(\Gamma_r, \Gamma_u)$ which is
the maximum revenue we can collect from consumers assigned to the
descendants of $u$ (excluding $u$) where $\Gamma_r$ is the set of
six items of price $1$ that are closest to $\ell_r$ as defined
earlier. And, similarly, $\Gamma_u=\{\Item'_{L, 1}, \Item'_{L, 2},
\Item'_{L, 3}, \Item'_{R, 1}, \Item'_{R, 2}, \Item'_{R, 3}\}$ is the
set of six items of price $1$ that are closest to $\ell_u$.
Moreover, we require that $\Gamma_u$ must be {\em consistent} with
$\Gamma_r$ in the sense that there is some price assignment such
that items in $\Gamma_u$ are the items closest to $\ell_u$ of price $1$
and items in $\Gamma_r$ are the items closest to $\ell_u$ of price $1$ as
well.
%
%once we assign the price to some items to make
%items in $\Gamma_u$ be the items closest to $u$ of price $1$, then
%items in $\Gamma_r$ is still the items closest to $r$ of price $1$.
%
(For example, if we let $\Gamma_r=\{\Item_{L, 1}, \Item_{L, 2},
\Item_{L, 3}, \Item_{R, 1}, \Item_{R, 2}, \Item_{R, 3}\}$ then an
item $\Item$ with property $\Item_{L, 3}[1]<\Item[1]<\Item_{L,
2}[1]$ cannot be in $\Gamma_u$ since this item must have price $0$.)
We use $\Gamma_u\bowtie\Gamma_r$ to denote ``$\Gamma_u$ is
consistent with $\Gamma_r$''. We define $f_v(\Gamma_r, \Gamma_v)$ in
a similar way.

Once we have $f_u(\Gamma_r, \Gamma_u)$ and $f_v(\Gamma_r, \Gamma_v)$
for all $\Gamma_u\bowtie\Gamma_r$ and $\Gamma_v\bowtie\Gamma_r$, we
can compute $f_r(\Gamma_r)$:
%
\begin{align}
 f_r(\Gamma_r) & = \max_{\Gamma_u\bowtie\Gamma_r} \left\{f_u(\Gamma_r, \Gamma_u) + m_1(\Gamma_u) + 2m_2(\Gamma_u)\right\} + \max_{\Gamma_v\bowtie\Gamma_r} \left\{f_v(\Gamma_r, \Gamma_v) + m_1(\Gamma_v) + 2m_2(\Gamma_v)\right\} \,.\label{eq:highway_recurse}
\end{align}
%
The main point here is that there is no consistency requirement between $\Gamma_u$ and $\Gamma_v$ so we have two independent subproblems. We define the function $f_z$, for all nodes $z$ in ${\cal T}$ similarly: Let $r=v_0$, $v_1$, $v_2$, ..., $v_{q-1}$ be the ancestors of $z$ and $v_q=z$. We have to compute $f_z(\Gamma_{v_0}, \Gamma_{v_1}, \ldots, \Gamma_{v_q})$ for all $\Gamma_{v_0}, \Gamma_{v_1}, \ldots, \Gamma_{v_q}$ such that $\Gamma_{v_i}\bowtie \Gamma_{v_j}$ for all $i\neq j$.

The computation of $f_z(\Gamma_{v_0}, \Gamma_{v_1}, \ldots,
\Gamma_{v_q})$ is done in the same way as Eq.\eqref{eq:highway_recurse} for every non-leaf node $z$.  At leaf node $z$, $f_z(\Gamma_{v_0}, \Gamma_{v_1}, \ldots,
\Gamma_{v_q})$ can also be easily computed: $f_z(\Gamma_{v_0},
\Gamma_{v_1}, \ldots, \Gamma_{v_q})=m_1(\Gamma_z)+2m_2(\Gamma_z)$.


Observe that $q=O(\log m + \log n)$ and there are $n^{6}$
choices for each $\Gamma_{v_i}$. Therefore, we can precompute
$f_z(\Gamma_{v_0}, \Gamma_{v_1}, \ldots, \Gamma_{v_q})$ for all
$n^{O(\log m + \log n)}$ combinations of $\Gamma_{v_0},
\Gamma_{v_1}, \ldots, \Gamma_{v_q}$. By working bottom-up from the
leaf nodes, the running time becomes $\poly(m)n^{O(\log m + \log n)}$.


\paragraph{Algorithm for $2$-{\sf SMP} (special case):} To solve the special case of $2$-{\sf SMP} defined above, we need to modify a few definitions in a right way.
%In particular, we cannot completely create two independent subproblems, we need to define the functions $f_v$ on two subproblems carefully so that we can find the solutions of these subproblems independently and be able to combine them without having one solution interfering the other.
%
%
Let us again consider the top-down algorithm and start at the root node $r$ of the partition tree ${\cal T}$. (Recall that we can assume that there is at most one item in each row and column so we can still define the paritition tree by drawing the vertical line through the point in the middle when sorted by the first dimension.)

One problem immediately appears: $f_r(\Gamma_r)$ cannot be used to compute the optimal revenue as we did in Eq.\eqref{eq:highway}. The reason is that we cannot compute the revenue from ${\cal C}_r$ using $m_1(\Gamma_r) + 2m_2(\Gamma_r)$ anymore.
%In fact, there seems to be no way to compute such a revenue unless $\Gamma_r$ is very big -- too big to try all possibilities efficiently. For this reason,
To fix this, we have to redefine ${\cal C}_r$ in the following way:
We assign all consumers lying on the left (respectively, right) of
$\Item_r$ to the left (respective, right) child and keep only those
consumers lying exactly on the vertical line going through $\Item_r$
in ${\cal C}_r$.

Now we can compute the revenue from the newly defined ${\cal C}_r$
and a function that computes the total revenue. To do this, we
define $f_r(\Item_1, \Item_2, \Item_3)$ to be the total revenue we
can get from consumers in ${\cal C}\setminus{\cal C}_r$ by pricing
the items in such a way that, among the items on the right side of
$\Item_r$, items $\Item_1$, $\Item_2$, and $\Item_3$ are the items
with price $1$ that have the highest, second highest, and third
highest values in the second dimension, respectively. Again, let
$\Gamma_r$ denote a possible choice of $\{\Item_1, \Item_2,
\Item_3\}$ and write $f_r(\Gamma_r)$ instead of $f_r(\Item_1,
\Item_2, \Item_3)$. If we can compute $f_r(\Gamma_r)$ then we can
get the optimal revenue by Eq.\eqref{eq:highway},
%, $\text{optimal
%revenue} = \max_{\Gamma_r} f_r(\Gamma_r) + m_1(\Gamma_r) +
%2m_2(\Gamma_r)$,
%
%\begin{align*}
%\text{Optimal revenue} &=
%\max_{\Gamma_r} f_r(\Gamma_r) + m_1(\Gamma_r) + 2m_2(\Gamma_r)\label{eq:2-smp-revenue}
%\end{align*}
%
where $m_1(\Gamma_r)$ and $m_2(\Gamma_r)$ is as defined earlier (with the new definition of ${\cal C}_r$).

Some more complications lie in computing $f_r(\Gamma_r)$, for any
$\Gamma_r$. As before, we will compute $f_u(\Gamma_r, \Gamma_u)$ and
$f_v(\Gamma_r, \Gamma_v)$ where $u$ and $v$ are the left and right
children of $r$, respectively. Howerver, we have to carefully define
$f_u(\Gamma_r, \Gamma_u)$ and $f_v(\Gamma_r, \Gamma_v)$, in a
different way.

We define $f_u(\Gamma_r, \Gamma_u)$, for any $\Gamma_u=\{\Item_1,
\Item_2, \Item_3\}$, to be the maximum revenue from the consumers
assigned to the descendants of $u$ when we price the items in such a
way that, among the items lying on the right side of $\Item_u$ and
left side of $\Item_r$, items $\Item_1$, $\Item_2$, and $\Item_3$
are the items with price $1$ that have the highest, second highest,
and third highest values in the second dimension, respectively. Note
that we do not need to check any consistency between $\Gamma_r$ and
$\Gamma_u$: For any choice of $\Gamma_r$ and $\Gamma_u$, there is
always a price assignment such that items in $\Gamma_r$ and
$\Gamma_u$ are the items of price $1$ that have the highest values
in the second dimension in their respective regions. In this case,
we say that $\Gamma_r\bowtie \Gamma_u$ is always true for any
$\Gamma_r$ and $\Gamma_u$.

On the other hand, we define $f_v(\Gamma_r, \Gamma_v)$, for any
$\Gamma_v=\{\Item_1, \Item_2, \Item_3\}$, to be the maximum revenue
from the consumers assigned to the descendants of $v$ when we price
the items in such a way that, among the items lying on the right
side of $\Item_v$, items $\Item_1$, $\Item_2$, and $\Item_3$ are the
items with price $1$ that have the highest, second highest, and
third highest values in the second dimension, respectively. In this
case, we have to make sure that $\Gamma_v$ is consistent with
$\Gamma_r$, i.e., there is some price assignment such that items in
$\Gamma_r$ and $\Gamma_u$ are the items of price $1$ that have the
highest values in the second dimension in their respective regions.


Now we have defined $f_u(\Gamma_r, \Gamma_u)$ and $f_v(\Gamma_r,
\Gamma_v)$, we compute $f_r(\Gamma_r)$ using
Eq.\eqref{eq:highway_recurse}.
%
%\begin{align*}
% f_r(\Gamma_r) & = \max_{\Gamma_u\bowtie\Gamma_r} \left\{f_u(\Gamma_r, \Gamma_u) + m_1(\Gamma_u) + 2m_2(\Gamma_u)\right\} + %\max_{\Gamma_v\bowtie\Gamma_r} \left\{f_v(\Gamma_r, \Gamma_v) + m_1(\Gamma_v) + 2m_2(\Gamma_v)\right\} \,.
%\end{align*}
%
As in the case of the highway pricing problem, we can extend the
definition to other nodes. In particular, at a leaf node $z$ we have
to compute $f_z(\Gamma_{v_0}, \Gamma_{v_1}, \ldots, \Gamma_{v_q})$
where $q=O(\log m + \log n)$. Hence, this case can be solved in
$\poly(|{\cal C}|)\cdot\size{\cal I}^{\polylog{|{\cal I}|}}$ time.

\danupon{To do: try not to use $m$ and $n$.}

\paragraph{Algorithm for general $2$-{\sf SMP}:}
We now remove the restrictions that each item must be priced $0$ or
$1$ and each budget must be $1$ or $2$. The removal of the
restriction on item price does not affect the case of highway
pricing problem since this can be easily assumed (see, e.g.,
\cite{GrandoniR10}).\danupon{Actually, can we assume this? In
\cite{GrandoniR10}, they also assume this for tollbooth problem on
trees (Section 4.1).}
%
Moreover, we can still assume that the maximum budget is $O(m n)$. Now we can deal with the general highway problem by
redefining $f_r(\Gamma_r)$: Let $\Gamma_r=\{\Item_{L,0}, \Item_{L,
1}, \ldots, \Item_{L, q}, \Item_{R,0}, \Item_{R, 1},
\ldots,\Item_{R, q}\}$ where $q=O(\log m n)$.
For any $i\leq q$, we want to price in such a way that $\Item_{L,
i}$ is the item closest to $\Item_r$ on the left such that the sum
of the price of all items between $\Item_r$ and $\Item_{L, i}$ is at
least $(1+\epsilon)^i$. Computing $f_r(\Gamma_r)$ can be done in the
same manner as before and consistency checking is easy to deal with.
Function $f_{v_q}(\Gamma_{v_0}, \Gamma_{v_1}, ..., \Gamma_{v_q})$,
for any node $v_q$ at level $q$ in $\cal T$, can be defined in a
similar manner.

For $2$-{\sf SMP}, we may not in general assume the item prices to
be $0/1$. Instead, we show that it can be assumed that each item
must have price $0$, or $(1+\epsilon)^j$, for any $j=0, 1, \ldots,
O(\log m)$. A natural extension of the above idea is to
define the notion of ``volume of regions'': For each item $\Item$,
let $H_{\Item}$ and $V_{\Item}$ denote the horizontal and vertical
line cutting through item $\Item$, respectively. Any rectangle
resulting from drawing some horizontal and vertical lines through
some items are called {\em regions} and the regions that do not
contain other regions are called {\em minimal regions}. For any
price assignment, we define the {\em volume} of a region to be the
sum of the price of all items within the region.



\begin{figure}%[htb!]
\centering \scalebox{0.7}[0.7]{\includegraphics{pic2}}
\caption{Approximating the revenue from consumer $\Consumer$ assigned to node  $z$ in $\mathcal{T}$.}\label{fig:area-idea}
\end{figure}


%\psfrag{A}{$V_z$}
%
%\psfrag{C}{$\Consumer$}
%
%%\begin{wrapfigure}{r}{.3\textwidth}
%\begin{figure}
%%\vspace{-5mm}
%  \centering
%      \epsfig{file=area-idea.eps,width=0.4\textwidth}
%  \caption{Approximating the revenue from consumer $\Consumer$ assigned to node $z$ in $\cal T$.}
%  \label{fig:area-idea} %\vspace{-5mm}
%%\end{wrapfigure}
%\end{figure}

Now, similar to the highway problem, we define $\Gamma_r=\{\Item_0,
\Item_1, ..., \Item_k\}$ (note that $k=O(\log m)$) as the
``region guess'': We define $f_r(\Gamma_r)$ to be the maximum
revenue from ${\cal C}\setminus {\cal C}_r$ when we price in such a
way that, for any $i$, item $\Item_i$ is the highest item (in the
second dimension) such that the volume of the region on the right of
the vertical line $V_{\Item_r}$ and above the horizontal line
$H_{\Item_i}$ (including $\Item_i$) is at least $(1+\epsilon)^i$.
Using these volume guesses, we can approximate the upper and lower
bounds of the revenue from each consumer $\Consumer$ at node $z$ by
looking at $\Gamma_v$ for all ancestors $v$ of $z$. This is because
each consumer's consideration set will contain some set of regions
$B_1, B_2, ...$ with volume guesses $(1+\epsilon)^{i_1},
(1+\epsilon)^{i_2}, ...$, respectively (such as the blue regions in
Figure~\ref{fig:area-idea}). Also, this consideration set will also
be contained in some set of regions $R_1, R_2, ...$ with volume
guesses $(1+\epsilon)^{i_1+1}, (1+\epsilon)^{i_2+1}, ...$ (such as
the blue and red regions together in Figure~\ref{fig:area-idea}).






However, in contrast to the case of highway problem, the consistency
between the guesses (e.g., between $\Gamma_r$ and its children
$\Gamma_u$ and $\Gamma_v$) is harder to guarantee. In order to
guarantee the consistency, we add another parameter, denoted by
$\Delta_r=\{\delta_0, \delta_1, \ldots, \delta_{O(k^2)}\}\subseteq
R_{\geq 0}^{O(k^2)}$ (recall that $|\Gamma_r|=k+1$). $\Delta_r$ is
used as a ``volume guess''. That is, we define $f_r(\Gamma_r,
\Delta_r)$ to be the maximum revenue from ${\cal C}\setminus {\cal
C}_r$ when we price in such a way that the restriction on $\Gamma_r$
is as before and, additionally, the volumn of the $i$-th minimal
region is exactly $\delta_i$ (where we make any order of the minimal
regions). We can now guarantee the consistency by making sure that
the sum of the volume guesses in smaller regions defined by
$\Gamma_u$ and $\Delta_u$ (as well as $\Gamma_v$ and $\Delta_v$) is
exactly the volume guesses in the bigger regions defined by
$\Gamma_r$ and $\Delta_r$. \danupon{Need to make this part much more
precise later. Also, we have to make it very clear why we need the
volume guesses, not region guesses alone.}

For any node $z$, we also define a function $f_z(\Gamma_{v_0},
\Gamma_{v_1}, \ldots, \Gamma_{v_q}, \Delta_z)$ where $v_0, v_1,
\ldots, v_{i-1}$ are ancestors of $z$ and $v_q=z$. In this case, we
consider the minimal regions obtained by drawing vertical lines
$V_{\Item_{v_0}}, V_{\Item_{v_1}}, \ldots, V_{\Item_{v_q}}$ and
horizontal lines $H_{\Item}$ for $\Item\in \Gamma_{v_i}$, for all
$i$. We use $\Delta_z$ to store the numbers that are the ``volume
guesses'' of all these regions. We also check the consistency in
terms of volume, i.e., $\Pi=\{\Gamma_{v_0}, \Gamma_{v_1}, \ldots,
\Gamma_{v_q}, \Delta_{v_q}\}$ is consistent with
$\Pi'=\{\Gamma_{v_0}, \Gamma_{v_1}, \ldots, \Gamma_{v_{q-1}},
\Delta_{v_{q-1}}\}$ if the volume guesses of the smaller regions
defined by lines in $\Pi$ add up to the volume guesses of the bigger
regions defined by lines in $\Pi'$.




%\iffalse
\subsection{Preprocessing}
Fix some $\epsilon >0$. Given an instance $(\iset, \cset)$, our goal
is to compute a price that collects a revenue of at least
$(1-O(\epsilon)) \opt$. Recall that we can assume that the consumers
are on the intersection of grid lines, and the items are in the grid
cells (cf. Lemma~\ref{lem:perturb}). First we process the input so
that the budgets and prices are polynomially bounded. Moreover, the
optimal solution only assigns prices of the form $(1+\epsilon)^j$
for some $j \leq O(\log m)$. The proof of this fact only uses
standard arguments (along the same line as in \cite{BalcanB07}).

%\begin{lemma}\label{lem:preprocess}
%Let $M= O(mn /\epsilon)$. We can transform, in polynomial time, the
%input $\pset$ into $\pset'$ such that
%%\begin{itemize}
%\squishlist
%  \item For each consumer ${\bf C}$, the budget of ${\bf C}$ is between $1$ and $M$.
%  \item Any price $p'$ that $\alpha$-approximates the optimal pricing of $\pset'$ can be transformed in polynomial time into another price $p$ that gives $(1+3\epsilon) \alpha$-approximation for $\pset$.
%  \item There is a near-optimal\parinya{To be changed} solution $\tilde{p}$ satisfying the following: For all ${\bf I} \in \iset$, $1 \leq \tilde{p}({\bf I}) \leq M$, and $\tilde{p}({\bf I})$ is in the form $(1+\epsilon)^j$ for some $j \leq O(\log m)$.
%\squishend
%%\end{itemize}
%\end{lemma}

\begin{lemma}\label{lem:preprocess}
Let $M= O(mn /\epsilon)$. The input instance ${\cal P}$ can be
reduced to ${\cal P'}$ with the following properties.

\squishlist
  \item For each consumer ${\bf C}$, the budget of ${\bf C}$ in ${\cal P}'$ is between $1$ and $M$.
  \item Any price $p'$ that $\alpha$-approximates the optimal pricing of $\pset'$ can be transformed in polynomial time into another price $p$ that gives $(1+3\epsilon) \alpha$-approximation for $\pset$.
  \item There is a $(1+\epsilon)$-approximate solution $\tilde{p}$ satisfying the following: For all ${\bf I} \in \iset$, $1 \leq \tilde{p}({\bf I}) \leq M$, and $\tilde{p}({\bf I})$ is in the form $(1+\epsilon)^j$ for some $j \leq O(\log m)$.
  %\item There is a solution $\tilde{p}$ for ${\cal P}'$ that $(1+\epsilon)$-approximates the optimal solution of $\cal P$ and
  %satisfies the following: For all ${\bf I} \in \iset$, $1 \leq \tilde{p}({\bf I}) \leq M$, and $\tilde{p}({\bf I})$ is in the form $(1+\epsilon)^j$ for some $j \leq O(\log m)$.
\squishend
%\end{itemize}
\end{lemma}
\begin{proof}%[Proof of Lemma~\ref{lem:preprocess}]
Let $B_{\max}$ be the maximum budget among all consumers. We first
remove all consumers whose budgets are less than $\epsilon
B_{\max}/mn$. Notice that we only lose the revenue of at most
$\epsilon B_{\max} \leq \epsilon \opt$ by this removal. We denote
the new set of consumers by $\cset'$. Now look at the optimal price
$p^*$ for the resulting instance. If for some ${\bf I} \in \iset$,
the price $p^*({\bf I})$ is less than $\epsilon B_{\max}/mn$, we
change its price to $p'({\bf I}) = 0$ and remove item ${\bf I}$
completely from the instance. Again, since each such item can only
be sold to at most $m$ consumers, discarding it only decreases the
revenue by $\epsilon B_{\max}/n$. There are at most $n$ such items,
so we lose a revenue of at most $\epsilon \opt$ in total. Let
$\iset'$ denote the resulting set of items.

Next we scale each consumer budget by $M'=mn/\epsilon B_{\max}$ to
get a new budget, i.e. $B'_C = M'B_C$. Now we have a complete
description of the instance $\pset'$ in which consumer budgets are
between $1$ and $M$. Let $\opt'$ be the optimal value of the new
instance. First we try to lower bound the value of $\opt'$. Consider
the same price $p^*: \iset' \rightarrow \R$ scaled up by a factor of
$M'$. The revenue from this price is at least $(1 - 2\epsilon)
M'\opt$, so we have that $\opt' \geq (1-2\epsilon)M'\opt$.

We are now ready to prove the second part. Assume that we have a
price $p'$ that gives $\alpha$-approximation for $\pset'$, so the
revenue collected by $p'$ is at least $\opt'/\alpha$. We construct
the price $p$ by scaling down the price of $p'$ by $M'$. Notice that
for each consumer ${\bf C}$ who can afford his consideration set in
$\pset'$ with price $p'(S_C)$, he can also afford his set in $\pset$
with price $p'(S_C) = p(S_C)/M'$. Therefore, the revenue collected
by $p$ is at least $\opt'/\alpha M' \geq (1-2\epsilon)\opt/ \alpha$.
This argument also implies that $\opt \geq \opt'/M'$.


Finally we show that there is a good solution $\tilde p$ that only
assigns prices in the form $(1+\epsilon)^j$, as follows. We round
down the price of $p^*$ to the nearest scale of $(1+\epsilon)^j$ for
some $j$. For each consumer $\Consumer$ who purchases item ${\bf I}$
w.r.t. price $p^*$, by scaling down every item price, she can still
afford her consideration set $S_{\Consumer}$, whose new price is at
least $p^*(S_{Consumer})/(1+\epsilon) \geq (1-\epsilon)
p^*(S_{\Consumer})$.
\end{proof}


%From now on, we assume that our input instance and its optimal price are in such format. Our goal is to devise a Quasi-PTAS for this instance. We note here that in some special cases of single-minded pricing problems, especially the Highway problem, an even stronger statement can be assumed; namely, that the optimal price is integral. It seems that such nice property may not hold in our case, and we anyway do not need it.

From now on, we assume that our input instance and its optimal price
are in such format. Our goal is to devise a {\sf QPTAS} for this
instance. We note here that in some special cases of single-minded
pricing problems, especially the Highway problem, an even stronger
statement can be assumed; namely, that the optimal price is
integral~\cite{GuruswamiHKKKM05}. It seems that such a nice property
may not hold in our case, and we anyway do not need it.
%\fi

\subsection{Partition tree}

We first construct a (almost balanced) binary tree $\tset$ where
each node in $\tset$ is associated with a rectangular region in the
plane (from now on, whenever we talk about region, we always mean a
rectangular one). We call this tree the {\em partition tree}. It can
be constructed recursively as follows. In the beginning, we have
$\tset=\set{r}$ where $r$ is the root of the tree whose region $A_r$
is the whole grid. We repeat the following process: For each leaf $v
\in \tset$, if the region $A_v$ of $v$ contains at least two items,
we choose a vertical grid line $\ell_v$ dividing the items in a
balanced manner to the left and right side. We then add the left
child $v'$ of $v$ with the region $A_{v'}$ being the region of $A_v$
on the left side of $\ell_v$. We also add the right child $v''$ of
$v$ associated with the region $A_{v''}$ on the right side of
$\ell_v$. We repeat the process until every leaf is associated with
a region containing only one item; see Figure~\ref{figure: tree}.

\danupon{It's better to define ``volume'' later because we need to
define ``region'' with horizontal lines first.} For each node $v \in
\tset$, we define the item set $\iset_v$ to be the set of all items
in the region $A_v$. Fix a price $p: \iset \rightarrow \R$. For any
region $A$, we define the ``volume'' $\vol_p(A)$ to be the total
price among all items in the region, i.e. $\vol_p(A) = \sum_{{\bf I}
\in A} p({\bf I})$. The following simple claim
is crucial in designing our algorithm.

\begin{claim}\label{claim:bound_sum}
Let $p^*$ be an optimal price. Then for any region $A$, there are
only $n^{O(\log m)}$ possible values of $\vol_{p^*}(A)$.
\end{claim}

\begin{proof}%[Proof of Claim~\ref{claim:bound_sum}]
Let $x_j$ denote the number of items ${\bf I}$ in $A$ with price
$p^*({\mathbf I}) = (1+\epsilon)^j$. Notice that we can write the
volume of $A$ as $\sum_{j=1}^{q} x_j (1+\epsilon)^j$ where $x_j$
only takes non-negative integer values at most $n$. So we have at
most $n^{O(\log m)}$ possibilities for the volume.
\end{proof}


\subsection{Horizontal partition and local profile}

From the construction, each node $v$ of the partition tree, is
associated with a vertical line $\ell_v$ which divides the plane
into two region. We further partition the right region using
vertical line, as follows.

Consider a non-leaf node $v \in \tset$ with left child $v'$ and
right child $v''$. A {\em horizontal partition} for node $v$,
denoted by $H_v$, is a collection of (not-necessarily distinct)
horizontal lines $\ell^v_1,\ldots, \ell^v_q$, partitioning the
region of $A_{v''}$ into many pieces; note that the left endpoints
of these lines are on $\ell_v$.\danupon{Need a picture here.} The
line $\ell^v_j$ is supposed to mark the highest $y$-coordinate such
that the volume inside $A_{v''}$ above $\ell^v_j$ is at least
$(1+\epsilon)^j$. Notice that each node $v$ has at most $n^{O(\log
m)}$ feasible partitions since there are at most $n$ possibilities
for the choice of each $\ell^v_j$.

Now if we fix a horizontal partition of every non-leaf node in the
partition tree, we can define {\em minimal} regions for each
non-leaf node $v$ as follows. For each node $v$, we consider all
vertical and horizontal lines associated with $v$ and all its
ancestors (i.e., all lines in $\ell_u$ and $H_u$ where $u=v$ or $u$
is an ancestor of $v$). Let $\lset_v$ denote the set of these lines.
%
$\lset_v$ naturally defines minimal regions: We say that a region
$A$ is minimal with respect to $\lset_v$ if and only if $A$ is a
rectangle whose four boundaries are the lines in $\lset_v$, and
there is no line in $\lset_v$ that intersects with the interior of
$A$.

%Now, in addition to fixing vertical partition of every non-leaf
%node, also fix some price a $p: \iset \rightarrow \R$. Consider
%again any non-leaf node $v$ whose minimal regions are defined as
%above.


Now, we define a {\em local profile} of a node $v$. It consists of
(i) horizontal partitions for $v$ and for all its ancestors, and
(ii) numbers on every minimal region resulting from vertical and
horizonal lines. The numbers are supposedly the ``volume guesses''
of every minimal region of $v$.


Now we try to guess the ``right'' local profile of every node in the
partition tree. We show that if this guess is right, then we get a
good approximation of the optimal solution. Moreover, we can use
dynamic programming to make the right guess.


\subsection{Dynamic Programming Solution}
%
%We need to define the follow terms first: Horizontal partition,
%minimal region, volume guess, and profile.


%For any region $A$, we define the ``volume'' $\vol_p(A)$ to be the
%total price among all items in the region, i.e. $\vol_p(A) =
%\sum_{{\bf I} \in A} p({\bf I})$. The following simple claim (proved
%in Appendix) is crucial in designing our algorithm.
%
%\begin{claim}\label{claim:bound_sum}
%Let $p^*$ be an optimal price. Then for any region $A$, there are
%only $n^{O(\log m)}$ possible values of $\vol_{p^*}(A)$.
%\end{claim}


%Observe that for any node $v$ and its ancestor $v'$, any minimal
%region of $v'$ is partitioned by vertical and horizontal lines into
%minimal regions of $v$.

A {\em global profile} (or just {\em profile} in short) of a node
$v$ consists of the local profile of $v$ and all its ancestors in
such a way that the volumes of minimal regions of $v$ is consistent
with its ancestors. More formally, fix a node $v$. A profile $\Pi_v$
for $v$ consists of, for any ancestor $v'$ of $v$, $\Pi_{v, v'}$
which is the local profile that node $v$ wants its ancestor $v'$ to
have (we also think of $v$ has an ancestor of itself for
convenience).
%
As a reminder, for each ancestor $v'$ of $v$, local profile $\Pi_{v,
v'}$ some horizontal partition $H_{v'}$ and the ``volume guess''of
each minimal region of $v$.
%
%\squishlist
%\item A horizontal partition $H_{v'}$
%  %lines $\set{\ell^{v'}_{j'}}_{j' \leq q}$.\danupon{This is very confusing.}
%
%\item
%%Let $\lset_{v'}$ be the set of all lines
%%$\set{\ell^{v''}_{j'}}_{j'\leq q}$ and $\ell_{v''}$ for ancestor
%%$v''$ of $v'$. Then $\Pi_{v, v'}$ stores the volume of minimal
%%regions $A$ w.r.t. set $\lset_{v'}$, i.e. a number $z_A$ associated
%%with every minimal region $A$.
%
%\squishend
%
In addition, we restrict that these local profiles $\Pi_{v, v'}$
have to be consistent in themselves in the following sense. For each
vertex $v'$, for any minimal region $A'$ of $\Pi_{v,v'}$ that is
further partitioned into minimal regions $A'_1, A'_2,\ldots,
A'_{\gamma}$ of $\Pi_{v,v''}$ for some descendant $v''$ of $v'$, the
number $z_{A'}$ at $\Pi_{v,v'}$ is equal to the sum of the numbers
$z'_{A_j}$ of $\Pi_{v,v''}$.\danupon{This is still not clear and a
bit informal.}

We argue that the number of global profiles for each node is not too
large, i.e. only $n^{\operatorname{poly} \log m}$. There are
$n^{O(\log m)}$ horizontal partitions for each ancestor $v'$ of $v$,
making a total of $n^{O(\log m \log n)}$ possibilities of the lines
$\ell^{v'}_j$. Now fix a choice of such horizontal partitions. If we
draw all lines $\ell^{v'}_j$ involved in the global profiles, we
will see a number of regions formed by intersections between these
lines and the vertical lines $\ell_{v''}$. Since there are $O(\log m
\log n)$ such horizontal lines and $O(\log n)$ vertical lines
involved, we have at most $O(\log m \log^2 n)$ minimal rectangular
regions. Each region has at most $n^{O(\log m)}$ possible volumes,
so there are at most $n^{O(\log^2 m \log^2 n)}$ global profiles for
each node $v$\parinya{We implicitly used the fact that $m \leq O(n)$. Have to say
it somewhere}.

Now we define a {\em valid tree profile} $\Pi$ for $\tset$ as the
set of global profiles $\set{\Pi_v}_{v \in \tset}$ such that $\Pi_v$
is a global profile for node $v$. Moreover, for every parent-child
pair $v, v'$ where $v$ is a parent of $v'$ in $\tset$, the profile
$\Pi_{v'}$ agrees with $\Pi_v$. That is, all profiles about
ancestors of $v$ in $\Pi_v$ and $\Pi_{v'}$ are exactly the same.

Given a valid tree profile $\Pi$, we have the notion of cost of the
profile $\Pi$ (denoted by $\mbox{\sf Cost}(\Pi)$) which is supposed
to approximate the total revenue we can collect by a price function
consistent with $\Pi$. The cost of a profile can be computed as
follows. For each node $v \in \tset$, let $\cset_v$ be the set of
all consumers on line $\ell_v$. For each consumer ${\bf C} \in
\cset_v$, the rectangular region enclosed by horizontal line ${\bf
C}[2]$ and vertical line $\ell_v$ %(see Figure)
is the actual amount the consumer needs to pay. This is the amount
we do not know, but we can approximate: We let $v_0, v_1,\ldots,
v_{\alpha}$ be a sequence of ancestors of $v$ such that $v$ is on
the left subtree of $v_i$ (in the order from $v$ to the root), where
$v_0= v$. And we let for each $i$, $j_i$ be the maximum number such
that $\ell^{v_i}_{j_i}$ does not lie below ${\bf C}[2]$. The cost of
consumer ${\bf C}$ is just the sum $\sum_{i=0}^{\alpha}
(1+\epsilon)^{j_i}$ if $B_C \leq \sum_{i=0}^{\alpha}
(1+\epsilon)^{j_i}$ and zero otherwise. The cost at node $v$ is just
the total cost of all consumers in $\cset_v$, and the cost of the
profile is the sum of the cost over all nodes $v \in \tset$.


\begin{figure}
\centering
%
\subfigure[Tree Decomposition up to depth $2$ where the shaded
region denotes $A_v$]{
\includegraphics[height=5cm]{pic3}\label{figure:
tree} }
%
\hspace{.05\textwidth}
%
\subfigure[The actual volume]{
\includegraphics[height=5cm]{pic4}
\label{fig:area1} }
%
\hspace{.05\textwidth}
%
\subfigure[The approximate volume]{
\includegraphics[height=5cm]{pic5}
\label{fig:area2}}
%
\caption{Computing the cost of consumer ${\bf C}$}\label{fig:area}
\end{figure}



\begin{lemma}\label{lem:exist_good_tree}
There is a valid tree profile $\Pi^*$ such that the cost is at least
$(1-\epsilon)\opt$.
\end{lemma}

\begin{proof}%[Proof of Lemma~\ref{lem:exist_good_tree}]
We start from the optimal price $p^*$ and construct the valid
profile as follows. For each node $v$, we define a feasible
partition of $v$ by choosing the line $\ell^v_j$ to be at the
highest $y$-coordinate such that the total volume enclosed is at
least $(1+\epsilon)^j$. Then we create a profile $\Pi^*_v$ for each
node $v$ according to the actual volume of each minimal region.
Notice that this gives a valid tree profile.
\end{proof}



Our goal now is to compute the valid profile $\Pi$ of maximum cost
by dynamic programming, and the profile will automatically suggest a
near-optimal pricing.

\paragraph{Computing the Solution:} Let $v \in \tset$.
We say that a price $p: \iset_v \rightarrow \R$ is consistent with
global profile $\Pi_v$ if and only if for every minimal region $A$
of $\Pi_v$ that is completely contained in $A_v$, we have $\vol_p(A)
= z_A$. The minimum cost profile can be computed in a bottom-up
fashion, as follows. For a leaf node $v$, a global profile for $v$
automatically determines the price of the only item in $A_v$;
discard a profile which does not have consistent price.

The following lemma shows that a price $p$ consistent with a valid
tree profile $\Pi$ can be computed from $\Pi$.

\begin{lemma}\label{lem:consistent}
For each node $v$ with left child $v'$ and right child $v''$, let
$p':\iset_{v'}\rightarrow \R$ and $p'':\iset_{v''}\rightarrow \R$ be
the prices that are consistent with the profile $\Pi_{v'}$ and
$\Pi_{v''}$ respectively. Then the price $p: \iset_v \rightarrow \R$
defined to agree with $p'$ on $\iset_{v'}$ and with $p''$ on
$\iset_{v''}$, is consistent with $\Pi_v$.
\end{lemma}

\begin{proof}%[Proof of Lemma~\ref{lem:consistent}]
Consider a minimal region $A \sse A_v$ and a volume guess $z_A$ in
$\Pi_v$. If $A \sse A_{v'}$ where $A$ is the union of minimal
regions $A'_1,\ldots A'_{\gamma}$ of $\Pi_{v'}$ (similar argument
can be made in case $A \sse A_{v''}$), then by assumption that
$\Pi_v$ is consistent with $\Pi_{v'}$, we know that the total value
$z_A = \sum_{j=1}^{\gamma} z'_{A'_j}$. Since $p'$ is consistent with
the profile $\Pi_{v'}$, we have that $\vol_{p}(A) = \vol_{p'}(A) =
\sum_{j} \vol_{p'}(A'_j) = \sum_j z'_{A'_j} = z_A$ as desired.
\end{proof}


We have shown that a valid tree profile $\Pi$ always has a price $p$
consistent with it. The following lemma %(proved in Appendix)
basically says that this price $p$ gives a revenue close to the cost
of the profile, which will in turn imply that the maximum cost
profile gives the revenue of at least $(1-O(\epsilon)) \opt$.

\begin{lemma}\label{lem:tree-revenue}
For any valid tree profile $\Pi$, let $p$ be a price consistent with
$\Pi$ and let $p' = p/(1+\epsilon)$. Then $p'$ collects revenue at
least $(1-\epsilon)$ fraction of the profile cost.
\end{lemma}

\danupon{Still need to prove this lemma.}


%\begin{proof}%[Proof of Lemma~\ref{lem:tree-revenue}]
%Fix a node $v \in \tset$. We argue that for each consumer ${\bf C}
%\in \cset_v$, we can collect revenue of at least $(1-\epsilon)$
%fraction of the cost of ${\bf C}$.\parinya{This is not done yet.}
%\end{proof}




%\paragraph{Remarks:} We note that our algorithm in this section also gives {\sf QPTAS} for $2$-{\sf UDP-MIN}. In fact (in a sense that we do not make precise here), our technique always works if consumers' functions are monotone; consumers' function is ``min'' in {\sf UDP-MIN} and ``sum'' in {\sf SMP}. Since $4$-{\sf UDP-MIN} is \APX-hard, one cannot hope to generalize this technique to higher dimensions. Some new ideas are required.



%\subsection{Proofs omitted from Section~\ref{sec:2-SMP}}


==> arxiv 7.24.2012/udp.tex <==
\section{{\sf QPTAS} for $2$-{\sf UUDP-MIN}}
\label{sec: bicriteria}\label{sec: qptas 2 udp}

%We first provide the proof sketch for Theorem~\ref{thm: bicriteria}. The full proof can be found in Appendix~\ref{sec:omitted-algorithms}.

%\subsection{$O(\sqrt{n})$-Approximation Algorithms for $2$-{\sf UUDP-MIN}}
%
%We provide a sketch of $O(\sqrt{n})$ approximation algorithm for $2$-{\sf UUDP-MIN}. First we invoke Lemma~\ref{lem:chain antichain} to partition the items into at most $O(\sqrt{n})$ chains and $O(\sqrt{n})$ antichains. Since each chain is equivalent to $1$-{\sf UUDP-MIN} instance, we would be able to solve it in polynomial time. Each $2$-dimensional antichain is equivalent to the Highway problem, which either admits a {\sf PTAS} (for {\sf SMP}) or has polynomial time algorithm (for {\sf UUDP-MIN}).
%
%
%\subsection{{\sf QPTAS}}
%%\label{subsection: qptas minbuying}

We note that we will write $O(\log m)$ instead of $O(\log n+\log m)$ since we assume that $n\leq m$ in this paper. (Otherwise, we already have approximation ratio of $O(\log m)=O(\log n)$.)

\sodaonly{

We explain the main idea first. The intuition can be realized by solving the following simple case: Assume for now that we have $\Theta(n^2)$ items, which form a set $\set{(2i-1,2j-1): 1 \leq i,j \leq n}$. In this case it is
possible to have two different consumers at the same coordinate, i.e. $\Consumer=\Consumer'$, while there is exactly one item at each point $(2i-1,2j-1)$. Assume further that each consumer has budget either $1$
or $2$. We show below how to solve this case in polynomial time.

Note that there is an optimal solution such that each item is
priced either $1$ or $2$: otherwise we could increase the price by small amount to collect more revenue.
%
Now, for any item point $(2i-1, 2j-1)$ and any price assignment
$p$, define\danupon{(to polish after submission) $r_p(i, j)$ may be confused with $r_\Consumer(p)$.}
\[r_p(i, j):=\min_{\substack{\Item[1]\ge 2i-1, \Item[2]\geq 2j-1 \\ \Item\in\iset}}\{p(\Item)\}
\]
 to be the minimum price among the items
dominating $(2i-1, 2j-1)$. This quantity immediately tells us how much
revenue we will get from consumers at point $(2i-2, 2j-2)$: each consumer
will buy an item at price $r_p(i, j)$ if and only if she has budget
at least $r_p(i, j)$.


By the definition of $r_p$, we know that for any fixed value $j$, $r_p(i,j)$ is non-decreasing in terms of $i$.
In other words, for any pricing $p$ and integer $j$, there exists
a ``threshold'' $\gamma(p, j)$ such that $r_p(i', j)=1$ for all $i'\leq
\gamma(p, j)$ and $r_p(i',j)=2$ for all $i'> \gamma(p, x)$.
%
Additionally, for any $j$, $\gamma(p, j)\geq \gamma(p, j+1)$.
%
Using these observations, we are ready to define the dynamic programming table. The table entry $T[i,j]$ is defined to be the maximum revenue we can get among the price assignment $p$ such that $r_p(i', j)=1$ for all
$i'\leq i$ and $r_p(i', j)=2$ for all $i'>i$. The table $T$ can be
computed as follows.
%
\begin{align}
T[i, j]&=\max_{i'\leq i} \{T[i',j+1]+m_1(i',j) + 2m_2(i',j)\}
\label{eq:udp-min-table}
\end{align}
%
where $m_1(i',j)$ is the number of consumers of the form
$(2i''-2,2j-2)$ for $i''\leq i'$ with budget $1$ and $m_2(i',j)$ is the number of
consumers of the form $(2i''-2,2j-2)$ for $i'' > i'$ with budget $2$. Moreover, let $T[i,n+1]=0$ for all $i$.
%
The optimal solution is then $\max_i T[i,1]$.

The above discussion captures almost all the key ideas for solving the general $2$-{\sf UUDP-MIN} problem. To get a {\sf QPTAS} in the general case,
we extend these ideas in the following way.

\squishlist

\item Consider a slight generalization when there is only one item in each column and row of grid cells (cf.
Lemma~\ref{lem:perturb}) while each budget is still $1$ and $2$. In
this case, we cannot pick arbitrary value of $i'$ when we compute
$T[i, j]$ as in Eq.\eqref{eq:udp-min-table} since it might not
correspond to any pricing. Through some additional observations,
table $T$ can be computed as follows: Let $\Item_j$ be the item whose $y$-coordinate is $j$. If $i=\Item_j[1]$ then we can use Eq.\eqref{eq:udp-min-table}; otherwise, $T[i,j]=T[i,j+1]+m_1(i,j)+2m_2(i,j)$. This algorithm runs in $O(n^3)$ time.


\item When there are $q$ different budgets, say $B_1, B_2, \ldots, B_q$,
we can solve the problem in $n^{O(q)}$ time. This is done
by defining $T[i_1,\ldots, i_{q-1}, j]$ to be the maximum
revenue we can get among the price assignment $p$ such that, for all
$q': 1 \leq q' \leq q$, $r_p(i',j)=B_{q'}$ for all $i_{q'-1}<i'\leq i_{q'}$ (where we let
$i_0=-1$ and $i_q=n$).


\item Finally, we obtain a {\sf QPTAS} by ``discretizing'' the prices so that there are not many choices of item prices (cf. Lemma~\ref{lem:uudp-discretize}). This enables us to assume that the prices are in  $\Gamma=\{0, (1+\epsilon)^0, (1+\epsilon)^1, ..., (1+\epsilon)^q\}$ where $q=O(\log_{1+\epsilon} m)$, and we can get the algorithm running in time $n^{O(\size{\Gamma})}=n^{O(\log m n)}$.\danupon{I changed this slightly: I point to Lemma~\ref{lemma:discretization}.}

\squishend
}

\subsection{Preprocessing}

\fullonly{We need to do a preprocessing, which will be used in the next two sections to design {\sf QPTAS} for $2$-{\sf UUDP-MIN} and $2$-{\sf SMP}.}
%
The following lemma says that we can assume the input lies on the grid where each row and column of the grid contains exactly one item.

\begin{lemma}\label{lem:perturb}
We are given an instance $(\cset,\iset)$ of $2$-{\sf UUDP-MIN}\fullonly{ (or $2$-{\sf SMP})}. Then we can, in polynomial time, transform $(\cset, \iset)$ into an ``equivalent'' instance $(\cset', \iset')$ such that
\begin{itemize}
\item Each consumer ${\bf C}' \in \cset'$ has even coordinates $(2i, 2j)$ for $0 \leq i,j \leq n$.
\item Each item ${\bf I}' \in \iset'$ has odd coordinate $(2i-1, 2j-1)$ for $1 \leq i,j \leq n$.

\item For each odd number $2i-1$, $1 \leq i \leq  n$, there is exactly one item ${\bf I}' \in \iset'$ with ${\bf I}'[1]=2i-1$ and exactly one item ${\bf I}'$ with ${\bf I}'[2]=2i-1$.
\end{itemize}
\end{lemma}
\begin{proof}
We sweep the horizontal line from top to bottom, and whenever the
line meets the items ${\bf I'}_1,\ldots, {\bf I'}_z$ such that ${\bf
I}'_1[1] < {\mathbf I}'_2[1] < \ldots < {\mathbf I}'_z[1]$ with the
same $y$-coordinate $y'$, we break ties as follows. Let $\delta$ be
the vertical distance from the line to the next item point below the
line. We set the new $y$-coordinates of these items to ${\bf
I'}_j[2] = y'-(z-j)\delta/2 z$. Notice that some consumers whose
$y$-coordinates lie in $[y', y'-\delta)$ get affected by this move.
We also change the $y$-coordinates of those consumers to
$y'-\delta/2$. Then we add the horizontal grid lines between the
space of every consecutive items, while making sure that consumer
points are on the line passing $y-\delta/2$. It is easy to see that
this process preserves the consideration set of every consumer. We
repeat the above steps until the sweeping line passes the bottommost
item.

We do a similar sweep of vertical line from right to left, inserting
the grid lines along the way. In the end, each consumer lies on the
intersection of the grid lines and each item in its cell, which guarantees
that no two items appear in the same row or column of the grid.
\end{proof}


\subsection{Detail of {\sf QPTAS} for {\sf UUDP-MIN}}


First, we can make the following simple assumption.

\begin{lemma}%[Lemma~\ref{lem:log_prices}]%\label{lem:log_prices}
\label{lem:uudp-discretize}
We can assume that the prices are in the form $(1+\epsilon)^0,
(1+\epsilon)^1, ..., (1+\epsilon)^q$ or zero where
$q=O(\log_{1+\epsilon} m)$ by sacrificing $(1+\epsilon)$ in the approximation factor.
\end{lemma}

\begin{proof}%[Proof of Lemma~\ref{lem:log_prices}]
We use the following standard arguments. Consider an optimal price
$p^*$. For each item ${\bf I}_j$, if the price is non-zero, we round
down the price $p^*({\bf I}_j)$ to the nearest scale of
$(1+\epsilon)^{q'}$, so the price of each item gets decreased by at
most a factor of $(1+\epsilon)$. Consider a consumer $\Consumer$ who
bought ${\bf I}_{j}$ with price $p^*$. After the rounding, she can
still afford ${\bf I}_j$, so we can still collect at least
$(1-\epsilon)p^*({\bf I}_j)$ from $C$.\danupon{Missing: We have to
first show that we can bound the maximum budget by $O(m)$.}
\end{proof}



Now, assuming that the optimal price $p^*$ has the above structure,
we show how to solve the problem in quasi-polynomial time. First, we
reorder the items based on their $y$-coordinates in descending
order, so we have ${\bf I}_1[2] > {\bf I}_2[2] > \ldots > {\bf
I}_n[2]$. A consumer $\Consumer$ is said to belong to {\em level
$j$} if it lies  between the row\danupon{We didn't define ``row'' before.} of ${\bf I}_j$ and
that of ${\bf I}_{j+1}$, so each consumer belongs to exactly one
level. Moreover, observe that a consumer $\Consumer$ at level $j$ is
only interested in (a subset of) items in $\set{{\bf I}_1,\ldots,
{\bf I}_j}$ (since $\Item_{j'}[2]<\Consumer[2]$ for any $j'>j$).
%
We define a subproblem $\pset_j$ as the pricing problem with items
$\set{{\bf I}_1,\ldots, {\bf I}_j}$ and consumers at levels
$1,\ldots, j$.  We use the dynamic programming technique to solve this
problem.

\paragraph{Profiles} We will remember the profile for each
subproblem $\pset_j$. A profile $\Pi$ of $\pset_j$ consists of
$O(\log m)$ item indices $\pi_1,\ldots, \pi_q \in \set{1,\ldots,
j}$. Each value $\pi_i$ is supposed to tell us the index of the item $\Item$
of price $(1+\epsilon)^i$ with maximum value $\Item[1]$. That is, we say
that a price $p$ for $\pset_j$ is {\em consistent} with profile
$\Pi =(\pi_1,\ldots, \pi_q)$ if, for each $i$, the item ${\bf I}_{\pi_i}$ has the highest value in the first coordinate among the items with price at most $(1+\epsilon)^i$, i.e., for all
$i$,
$$\pi_i=\arg\max_{j'} \{ \Item_{j'}[1]\ |\ p(\Item_{j'})\leq (1+\epsilon)^i\}\,.$$
%
Since $\{ \Item_{j'}\ |\ p(\Item_{j'})\leq (1+\epsilon)^i\}\subseteq
\{ \Item_{j'}\ |\ p(\Item_{j'})\leq (1+\epsilon)^{i+1}\}$ for any
$i$,
$${\bf I}_{\pi_1}[1] \leq {\bf I}_{\pi_2}[1] \leq \ldots \leq {\bf
I}_{\pi_q}[1]\,.$$


Observe that  if two prices $p'$ and $p''$ have the
same $\pset_j$ profile, then consumers at level $j$ see no
difference between these two prices, as shown formally by the
following lemma. We say that an item $\Item_k$ is a profile item for profile $\Pi=(\pi_1,\ldots, \pi_q)$ if and only if $k = \pi_{q'}$ for some $q' \in [q]$.

\begin{lemma}
\label{lemma:reconstruction}
%There are profiles $\Pi_1,\ldots, \Pi_n$ for subproblems $\pset_1,\ldots, \pset_n$ respectively such that (i) each profile is consistent with $p^*$ and (ii) we can assume w.l.o.g. that in $p^*$, each consumer at level $j$ only purchases items in $\Pi_j$.
Let $\Pi$ be a profile for subproblem $\pset_j$, and let $p$ be any
price function for $\pset_j$ that is consistent with profile $\Pi$. Then we
can assume without loss of generality that every consumer at level $j$ only purchases
profile items.
\end{lemma}
%

\begin{proof}%[Proof of Lemma~\ref{lemma:reconstruction}]
Suppose that a consumer $\Consumer$ buys an item ${\bf I}$ in $\iset$
with $p({\bf I}) =(1+\epsilon)^{q'}$ which is not a profile item.
Then consider the profile item ${\bf I}_{\pi_{q'}}$, which satisfies ${\bf I'}[1] \geq {\bf I}[1]$, so we must have $\Item_{\pi_{q'}} \in S_{\Consumer}$. We can
therefore assume that consumer $\Consumer$ buys $\Item_{\pi_{q'}}$ instead
of ${\bf I}$.
\end{proof}


Let $\Pi=(\pi_1,\ldots, \pi_q)$ be a profile for $\pset_{j}$ and
$\Pi'= (\pi'_1,\ldots, \pi'_q)$ be a profile for $\pset_{j-1}$. We
say that $\Pi$ is {\em consistent} with $\Pi'$ if for any price
$p':\set{{\bf I}_1,\ldots, {\bf I}_{j-1}} \rightarrow \R$ that is
consistent with $\Pi'$, we can extend $p'$ to $p$ by assigning value
$p({\bf I}_j)$ such that $p$ is consistent with $\Pi$. Notice that
consistency between any two profiles can be checked in polynomial
time by trying all $q$ possibilities of prices.

We recall that we use $p^*$ to denote the optimal price.

\begin{lemma}\label{lem:udp-consistency}
There are profiles $\Pi^1,\ldots, \Pi^n$ for $\pset_1,\ldots,
\pset_n$ respectively such that for each $j\in\{1,\cdots, n-1\}$,
$\Pi^j$ is consistent with $\Pi^{j+1}$. Moreover, all such profiles
are consistent with price $p^*$.
\end{lemma}
%
\begin{proof}%[Proof of Lemma~\ref{lem:udp-consistency}]
For each subproblem $\pset_j$, we define the profile
$\Pi^j=(\pi^j_1,\ldots, \pi^j_q)$ based on the price $p^*$ (there is
only one possible profile consistent with $p^*$). It is clear that
$\Pi^j$ is always consistent with $\Pi^{j+1}$.
\end{proof}




\paragraph{Dynamic Programming Table} For each $j=1,\ldots, n$ and for each profile $\Pi$ of $\pset_j$, we use a table entry $T(j,\Pi)$ to store the maximum revenue achievable among the price function for $\pset_j$ that is consistent with the profile $\Pi$. Since there are $n^{O(\log m)}$ possibilities for the profile $\Pi$, the table size is $n^{O(\log m)}$. We now show the computation of the table. To compute $T(j,\Pi)$, we recall that given the profile $\Pi$, the revenue from consumers at level $j$ can be computed efficiently. Denote such revenue by $r_j(\Pi)$. The following equation holds:
\[T(j,\Pi) = r_j(\Pi) + \max_{\Pi' \mbox{ consistent with } \Pi} T(j-1, \Pi') \]

\paragraph{Computing the Solution} For each table entry $T(j,\Pi)$, we can keep track of the profile $\Pi'$ such that $T(j-1, \Pi')$ is the entry that is used to compute $T(j,\Pi)$. Let $T(n, \Pi)$ be the entry that contains the maximum value over all $\Pi$. The value in this entry represents the revenue we can get from the optimal pricing $p^*$, so it is enough to reconstruct the price function $p^*$. We first obtain a sequence of profiles $\Pi^1,\ldots, \Pi^n = \Pi$ such that $\Pi^j$ is a profile for $\pset_j$ and that $\Pi^j$ is consistent with $\Pi^{j-1}$ for any $j =1,\ldots, n$. This sequence allows us to reconstruct a price function that is consistent with all the profiles in polynomial time.


